Fundamental Limits on Delivery Time in Cloud- and Cache-Aided Heterogeneous Networks

A Fog radio access network is considered as a network architecture candidate to meet the soaring demand in terms of reliability, spectral efficiency, and latency in next generation wireless networks. This architecture combines the benefits associated with centralized cloud processing and wireless edge caching enabling primarily low-latency transmission under moderate fronthaul capacity requirements. The F-RAN we consider in this paper is composed of a centralized cloud server which is connected through fronthaul links to two edge nodes serving two mobile users through a Z-shaped partially connected wireless network. We define an information-theoretic metric, the delivery time per bit (DTB), that captures the worst-case per-bit delivery latency for conveying any requested content to the users. For the cases when cloud and wireless transmission occur either sequentially or in parallel, we establish coinciding lower and upper bounds on the DTB as a function of cache size, backhaul capacity and wireless channel parameters. Through optimized rate allocation, our achievability scheme determines the best combination of private, common signalling and interference neutralization that matches the converse. Our converse bounds use subsets of wireless, fronthaul and caching resources of the F-RAN as side information that enable a single receiver to decode either one or both users' requested files. We show the optimality on the DTB for all channel regimes. In case of serial transmission, the functional DTB-behavior changes at fronthaul capacity thresholds. In this context, we combine multiple channel regimes to classes of channel regimes which share the same fronthaul capacity thresholds and as such the same DTB-functional. In total, our analysis identifies four classes; in only three of those edge caching and cloud processing can provide nontrivial synergestic and non-synergestic performance gains.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Communications Society subset of the full
IEEEtran package and is intended for use with IEEE Communications Society
publications. The included version of the IEEEtran_HOWTO.pdf has been
specially formatted in IEEE Communications Society (comsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf,
                   bare_jrnl_comsoc.tex.
***************************************************************************


==> content/LDM_tikz/tikz_ldm.tex <==
\input{tikzheader}

%name number of pipes; position (x,y);
\newcommand{\ldmnewuser}[3]{
\begin{scope}[pipedot/.style={draw, circle, inner sep=0pt, minimum size=0.3cm}]
\def\username{#1}
\def\numPipes{#2}
\def\distanceDots{0.6}
\coordinate (position\username) at #3;

\foreach \x in {1,...,\numPipes} {
	\pgfmathparse{-(\x-1)*\distanceDots}
	\node[pipedot] (node\x\username) at ($(0, \pgfmathresult)+(position\username)$) {};
}
\node[draw,fit=(node1\username) (node\numPipes\username)] (group\username) {};
\end{scope}
} 

%name of user1, name of user2, no of pipes, shifted levels 
\newcommand{\ldmconnectusers}[4]{
\foreach \x in {1,...,#3} {
	\pgfmathtruncatemacro\mymacro{(\x+#4)}
	\draw[->, thick] (node\x #1)--(node\mymacro #2) ;
}
} 



\begin{document}

\begin{tikzpicture}

\ldmnewuser{Alice}{6}{(0,0)}
\node[node distance=0.1cm, above=of groupAlice] {Alice};
\node[node distance=0.2cm, left=of node1Alice] {$a\otimes b$};
\node[node distance=0.2cm, left=of node2Alice] {$a\otimes b\otimes b$};

\ldmnewuser{Bob}{6}{(5,0)}
\node[node distance=0.1cm, above=of groupBob] {Bob};

\ldmnewuser{Eve}{6}{(5,-5)}
\node[node distance=0.1cm, above=of groupEve] {Eve};

\ldmconnectusers{Alice}{Bob}{4}{1}
\ldmconnectusers{Alice}{Eve}{2}{3}





\node[right=of node5Bob.south, yshift=-0.2cm] (bobcurly1) {}; 
\node[right=of node2Bob.north, yshift=0.2cm] (bobcurly2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
(bobcurly1) -- (bobcurly2) node [black,midway] {$n_1$};

\node[right=of node5Eve.south, yshift=-0.2cm] (evecurly1) {}; 
\node[right=of node4Eve.north, yshift=0.2cm] (evecurly2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
(evecurly1) -- (evecurly2) node [black,midway] {$n_2$};

\node[right=of node3Eve.south, yshift=-0.2cm] (evecurly3) {}; 
\node[right=of node2Eve.north, yshift=0.2cm] (evecurly4) {}; 
\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
(evecurly3) -- (evecurly4) node [black,midway,xshift=0.4cm] {$n_1-n_2$};



\begin{scope}[on background layer]
\node[fill=blue!10,fit=(node2Bob) (node5Bob)] (groupBobn1) {};
\node[fill=blue!50,fit=(node2Eve) (node3Eve)] (groupEven1n2) {};
%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
\end{scope}


%\draw[->,red] (node5Bob.south)--(node1Eve.north) ;
\end{tikzpicture}


\begin{tikzpicture}
\coordinate (coordSourceupleft1) at (0,0);
\coordinate (coordChannelupleft1) at (10,0);

\node (reliableSourceBitsLeft) at (coordSourceupleft1) {};
\node[right=of reliableSourceBitsLeft] (reliableSourceBitsRight) {};
\node[node distance=1cm, below=of reliableSourceBitsLeft] (secureSourceBitsLeft) {};
\node[node distance=1cm, below=of reliableSourceBitsRight] (secureSourceBitsRight) {};
\node[node distance=0.1cm, left=of secureSourceBitsRight] (secureSourceBitsBlack) {};
\node[node distance=1cm, below=of secureSourceBitsRight] (bottomSourceRight) {};
\node[node distance=0.1cm, left=of secureSourceBitsLeft] {\parbox{2cm}{Secure source bits}};
\node[node distance=0.1cm, right=of secureSourceBitsRight] {$m_2-m_1$};
\node[node distance=0.1cm, left=of reliableSourceBitsLeft] {\parbox{2cm}{Reliable source bits}};
\node[node distance=0.1cm, right=of reliableSourceBitsRight] {$m_1$};

\draw [fill=yellow!20] (reliableSourceBitsLeft) rectangle (bottomSourceRight);
\draw [fill=yellow!50] (secureSourceBitsLeft) rectangle (bottomSourceRight);
\draw [fill=black] (secureSourceBitsBlack) rectangle (bottomSourceRight);


\node (reliableChannelBitsLeft) at (coordChannelupleft1) {};
\node[right=of reliableChannelBitsLeft] (reliableChannelBitsRight) {};
\node[node distance=1cm, below=of reliableChannelBitsLeft] (secureChannelBitsLeft) {};
\node[node distance=1cm, below=of reliableChannelBitsRight] (secureChannelBitsRight) {};
\node[node distance=0.1cm, left=of secureChannelBitsRight] (secureChannelBitsBlack) {};
\node[node distance=1cm, below=of secureChannelBitsRight] (bottomChannelRight) {};
\node[node distance=0.1cm, left=of secureChannelBitsLeft] {\parbox{2cm}{Secure source bits}};
\node[node distance=0.1cm, right=of secureChannelBitsRight] {$m_2-m_1$};
\node[node distance=0.1cm, left=of reliableChannelBitsLeft] {\parbox{2cm}{Reliable source bits}};
\node[node distance=0.1cm, right=of reliableChannelBitsRight] {$m_1$};

\draw [fill=yellow!20] (reliableChannelBitsLeft) rectangle (bottomChannelRight);
\draw [fill=yellow!50] (secureChannelBitsLeft) rectangle (bottomChannelRight);
\draw [fill=black] (secureChannelBitsBlack) rectangle (bottomChannelRight);

\end{tikzpicture}


\tikzstyle{antenna} = [regular polygon,regular polygon sides=3, draw,shape
border rotate=180,minimum size=0.2pt,scale=0.3]
\tikzstyle{waves} = [snake=expanding waves, segment amplitude = 1.5cm, segment length = 0.3 cm,draw ]
\begin{tikzpicture}
	\coordinate (usercoord) at (0,0);
	\node[rectangle,draw, minimum width=1cm, minimum height=1cm] (user) at (usercoord) {Tx};
	\node[antenna] (userant1) at ($(user.west)+(-0.3cm,0.3cm)$) {};
    \path[waves]  (userant1.west) -- ($(userant1.west)+(-1cm,0)$);
    \draw (user) -| (userant1);
          
\end{tikzpicture}

\end{document}

==> content/LDM_tikz/tikz_stacks.tex <==
\input{tikzheader}

\edef\defaultpgflinewidth{\the\pgflinewidth}
%\newlength{\defaultpgflinewidth}
%\setlength{\defaultpgflinewidth}{0.1cm}

%Previous level name, new level name, level height, level description
\newcommand{\placeLevelOnTop}[4]{
\node[draw, fill=white, line width=\defaultpgflinewidth, rectangle, minimum width=1cm,minimum height=#3,inner sep=0pt] (#2) at ($(#1.north)+(0,#3*0.5-\defaultpgflinewidth*0.5)$) {#4}; 
}

%Previous level name, new level name, level height, level description
\newcommand{\placeLevelBelowBottom}[4]{
\node[draw, color=black!20, fill=white, line width=\defaultpgflinewidth, rectangle, minimum width=1cm,minimum height=#3,inner sep=0pt] (#2) at ($(#1.south)+(0,-#3*0.5+\defaultpgflinewidth*0.5)$) {#4}; 
}

\newlength{\mylabelwidth}
%Base coordinate, Level name, level label 
\newcommand{\addLevelLabel}[3]{
\settowidth{\mylabelwidth}{\pgfinterruptpicture #3 \endpgfinterruptpicture}
\node at ($(#2.north west -| #1)+(-0.2cm,-\defaultpgflinewidth*0.5)+(-\mylabelwidth*0.5,0)$) {#3};
\begin{pgfonlayer}{background}
\draw[dashed] ($(#2.north west -| #1)+(-0.1cm,-\defaultpgflinewidth*0.5)$) -- ($(#2.north west)+(0,-\defaultpgflinewidth*0.5)$);
\end{pgfonlayer}
}

%Lower Level name, Upper level name, brace label
\newcommand{\addBraceRight}[3]{
\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
(#1.south east) -- (#2.north east) node [black,midway,xshift=0.8cm,rotate=90] {\footnotesize
#3};
}

%Level name, dim label
\newcommand{\addDimensioningRight}[2]{
\draw[dashed] ($(#1.north east)+(0,-\defaultpgflinewidth*0.5)$) -- ($(#1.north east)+(0.6cm,-\defaultpgflinewidth*0.5)$);
\draw[dashed] ($(#1.south east)+(0,\defaultpgflinewidth*0.5)$) -- ($(#1.south east)+(0.6cm,\defaultpgflinewidth*0.5)$);
\draw[thick,<->] ($(#1.north east)+(0.3cm,-\defaultpgflinewidth*0.5)$) -- node[right,fill=white,inner sep=0pt,xshift=0.1cm] {#2} ($(#1.south east)+(0.3cm,\defaultpgflinewidth*0.5)$);
}

%Level name, dim label
\newcommand{\addDimensioningLeft}[2]{
\draw[dashed] ($(#1.north west)+(0,-\defaultpgflinewidth*0.5)$) -- ($(#1.north west)+(-0.6cm,-\defaultpgflinewidth*0.5)$);
\draw[dashed] ($(#1.south west)+(0,\defaultpgflinewidth*0.5)$) -- ($(#1.south west)+(-0.6cm,\defaultpgflinewidth*0.5)$);
\draw[thick,<->] ($(#1.north west)+(-0.3cm,-\defaultpgflinewidth*0.5)$) -- node[left,fill=white,inner sep=0pt,xshift=-0.1cm] {#2} ($(#1.south west)+(-0.3cm,\defaultpgflinewidth*0.5)$);
}



\begin{document}

\begin{tikzpicture}

[
%
]
\coordinate (txOneY) at (0,0);
\coordinate (txTwoY) at ($(txOneY)+(1.5,0)$);
\coordinate (baseLeft) at ($(txOneY)+(-0.75cm,0)$);
\coordinate (txOneZ) at ($(txTwoY)+(2,0)$);
\coordinate (txTwoZ) at ($(txOneZ)+(1.5,0)$);

\node (ytx1) at ($(txOneY)+(0,-0.5)$) {Tx1};
\node (ytx2) at ($(txTwoY)+(0,-0.5)$) {Tx2};
\node  at ($(txOneY)!0.5!(txTwoY) + (0,-1)$) {$\textbf{Rx2}$};
\node (ztx1) at ($(txOneZ)+(0,-0.5)$) {Tx1};
\node (ztx2) at ($(txTwoZ)+(0,-0.5)$) {Tx2};
\node  at ($(txOneZ)!0.5!(txTwoZ) + (0,-1)$) {$\textbf{Rx1}$};

\placeLevelOnTop{txOneY}{d1}{0.5cm}{${D}_1$}
\placeLevelOnTop{d1}{c1}{1cm}{${C}_1$}
\placeLevelOnTop{c1}{b1}{0.5cm}{${B}_1$}

\placeLevelOnTop{txTwoY}{b2}{0.5cm}{${B}_2$}

\placeLevelOnTop{txOneZ}{d1}{0.5cm}{${B}_1$}

\placeLevelOnTop{txTwoZ}{d2z}{0.5cm}{${D}_2$}
\placeLevelOnTop{d2z}{c2z}{1cm}{${C}_2$}
\placeLevelOnTop{c2z}{b2z}{0.5cm}{${B}_2$}
\addLevelLabel{baseLeft}{c2z}{$2n_d-n_c$}
\addLevelLabel{baseLeft}{d2z}{$n_d$}
\addLevelLabel{baseLeft}{b2z}{$n_c$}

\addDimensioningRight{c2z}{$l_1$}


\draw[thick] ($(baseLeft)+(0,-\defaultpgflinewidth*0.5)$) -- ($(txTwoY)+(0.75cm,-\defaultpgflinewidth*0.5)$);
\draw[thick] ($(txOneZ)+(-0.75,-\defaultpgflinewidth*0.5)$) -- ($(txTwoZ)+(0.75cm,-\defaultpgflinewidth*0.5)$);

\end{tikzpicture}




\end{document}

==> content/LDM_tikz/tikz_stacks_app.tex <==
\input{tikzheader}

\edef\defaultpgflinewidth{\the\pgflinewidth}
%\newlength{\defaultpgflinewidth}
%\setlength{\defaultpgflinewidth}{0.1cm}

%Previous level name, new level name, level height, level description
\newcommand{\placeLevelOnTop}[4]{
\node[draw, fill=white, line width=\defaultpgflinewidth, rectangle, minimum width=1cm,minimum height=#3,inner sep=0pt] (#2) at ($(#1.north)+(0,#3*0.5-\defaultpgflinewidth*0.5)$) {#4}; 
}

%Previous level name, new level name, level height, level description
\newcommand{\placeLevelBelowBottom}[4]{
\node[draw, color=black!20, fill=white, line width=\defaultpgflinewidth, rectangle, minimum width=1cm,minimum height=#3,inner sep=0pt] (#2) at ($(#1.south)+(0,-#3*0.5+\defaultpgflinewidth*0.5)$) {#4}; 
}

\newlength{\mylabelwidth}
%Base coordinate, Level name, level label 
\newcommand{\addLevelLabel}[3]{
\settowidth{\mylabelwidth}{\pgfinterruptpicture #3 \endpgfinterruptpicture}
\node at ($(#2.north west -| #1)+(-0.2cm,-\defaultpgflinewidth*0.5)+(-\mylabelwidth*0.5,0)$) {#3};
\begin{pgfonlayer}{background}
\draw[dashed] ($(#2.north west -| #1)+(-0.1cm,-\defaultpgflinewidth*0.5)$) -- ($(#2.north west)+(0,-\defaultpgflinewidth*0.5)$);
\end{pgfonlayer}
}

%Lower Level name, Upper level name, brace label
\newcommand{\addBraceRight}[3]{
\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
(#1.south east) -- (#2.north east) node [black,midway,xshift=0.8cm,rotate=90] {\footnotesize
#3};
}

%Level name, dim label
\newcommand{\addDimensioningRight}[2]{
\draw[dashed] ($(#1.north east)+(0,-\defaultpgflinewidth*0.5)$) -- ($(#1.north east)+(0.6cm,-\defaultpgflinewidth*0.5)$);
\draw[dashed] ($(#1.south east)+(0,\defaultpgflinewidth*0.5)$) -- ($(#1.south east)+(0.6cm,\defaultpgflinewidth*0.5)$);
\draw[thick,<->] ($(#1.north east)+(0.3cm,-\defaultpgflinewidth*0.5)$) -- node[right,fill=white,inner sep=0pt,xshift=0.1cm] {#2} ($(#1.south east)+(0.3cm,\defaultpgflinewidth*0.5)$);
}

%Level name, dim label
\newcommand{\addDimensioningLeft}[2]{
\draw[dashed] ($(#1.north west)+(0,-\defaultpgflinewidth*0.5)$) -- ($(#1.north west)+(-0.6cm,-\defaultpgflinewidth*0.5)$);
\draw[dashed] ($(#1.south west)+(0,\defaultpgflinewidth*0.5)$) -- ($(#1.south west)+(-0.6cm,\defaultpgflinewidth*0.5)$);
\draw[thick,<->] ($(#1.north west)+(-0.3cm,-\defaultpgflinewidth*0.5)$) -- node[left,fill=white,inner sep=0pt,xshift=-0.1cm] {#2} ($(#1.south west)+(-0.3cm,\defaultpgflinewidth*0.5)$);
}



\begin{document}

\begin{tikzpicture}

[
%
]
\coordinate (txOneY) at (0,0);
\coordinate (txTwoY) at ($(txOneY)+(1.5,0)$);
\coordinate (baseLeft) at ($(txOneY)+(-0.75cm,0)$);
\coordinate (txOneZ) at ($(txTwoY)+(2,0)$);
\coordinate (txTwoZ) at ($(txOneZ)+(1.5,0)$);

\node (ytx1) at ($(txOneY)+(0,-0.5)$) {Tx1};
\node (ytx2) at ($(txTwoY)+(0,-0.5)$) {Tx2};
\node  at ($(txOneY)!0.5!(txTwoY) + (0,-1)$) {$\textbf{Rx2}$};
\node (ztx1) at ($(txOneZ)+(0,-0.5)$) {Tx1};
\node (ztx2) at ($(txTwoZ)+(0,-0.5)$) {Tx2};
\node  at ($(txOneZ)!0.5!(txTwoZ) + (0,-1)$) {$\textbf{Rx1}$};

\placeLevelOnTop{txOneY}{d1}{0.5cm}{${D}_1$}
\placeLevelOnTop{d1}{c1}{1cm}{${C}_1$}
\placeLevelOnTop{c1}{b1}{0.5cm}{${B}_1$}

\placeLevelOnTop{txTwoY}{b2}{0.5cm}{${B}_2$}

\placeLevelOnTop{txOneZ}{d1}{0.5cm}{${B}_1$}

\placeLevelOnTop{txTwoZ}{d2z}{0.5cm}{${D}_2$}
\placeLevelOnTop{d2z}{c2z}{1cm}{${C}_2$}
\placeLevelOnTop{c2z}{b2z}{0.5cm}{${B}_2$}
\addLevelLabel{baseLeft}{c2z}{$2n_d-n_c$}
\addLevelLabel{baseLeft}{d2z}{$n_d$}
\addLevelLabel{baseLeft}{b2z}{$n_c$}

\addDimensioningRight{c2z}{$l_1$}


\draw[thick] ($(baseLeft)+(0,-\defaultpgflinewidth*0.5)$) -- ($(txTwoY)+(0.75cm,-\defaultpgflinewidth*0.5)$);
\draw[thick] ($(txOneZ)+(-0.75,-\defaultpgflinewidth*0.5)$) -- ($(txTwoZ)+(0.75cm,-\defaultpgflinewidth*0.5)$);

\end{tikzpicture}




\end{document}

==> content/LDM_tikz/tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
      \pgf@temp
      \fi%
    },
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
        \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{\csname pgfk@/tikz/tikzmark prefix\endcsname#1\csname pgfk@/tikz/tikzmark suffix\endcsname}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname{\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
      \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}\save@orig@pic%
      \pgfsys@getposition{\pgfpictureid}\save@this@pic%
      \pgf@process{\pgfpointorigin\save@this@pic}%
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
      \pgf@process{\pgfpointorigin\save@orig@pic}%
      \advance\pgf@x by -\pgf@xa
      \advance\pgf@y by -\pgf@ya
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
          \advance \pgf@xa by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@x\relax
\advance \pgf@ya by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@y\relax
          \advance \pgf@xa by -\csname save@pg@\pgfpictureid\endcsname\pgf@x\relax
\advance \pgf@ya by -\csname save@pg@\pgfpictureid\endcsname\pgf@y\relax
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }
\begingroup
\catcode`\;=\active
\gdef\tikzmark@active#1#2{%
\tikz[remember picture with id=#2] #1;}
\endgroup
\def\tikzmark@nonactive#1#2{%
\tikz[remember picture with id=#2] #1;}
\newcommand\tikzmark@outside[2][]{%
  \ifnum\catcode`\;=\active
   \let\tikzmark@next=\tikzmark@active
  \else
   \let\tikzmark@next=\tikzmark@nonactive
  \fi
  \tikzmark@next{#1}{#2}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x pt}{\the\pgf@y pt}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark}[2][]{\only#3{\beameroriginal{\tikzmark}[{#1}]{#2}}}
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@#1}{%
      #3%
    }{%
      #2%
    }%
  }%
\newcommand\subnode[3][]{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@shape{rectangle}%
  \def\tikz@anchor{center}%
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
  {\PackageError{pgf}{Unknown shape ``\tikz@shape''}{}}%
  {%
    {%
      \let\pgf@sh@savedmacros=\pgfutil@empty% MW
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \def\pgf@sm@shape@name{\tikz@shape}% CJ % TT added prefix!
      \csname pgf@sh@s@\tikz@shape\endcsname%
      \pgf@sh@savedpoints%
      \pgf@sh@savedmacros% MW
      \pgftransformshift{%
        \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
       \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}% FIXME : this is double work!
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@node@name{\tikz@fig@name}%
      \ifx\pgf@node@name\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{\tikz@shape}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
        \pgfgettransform\pgf@temp
        \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
      \fi%
    }%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}
\def\usetikzmarklibrary{\pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}}%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

%% 
%% Copyright (C) 2011-2016 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.


==> content/ach_scheme.tex <==
\subsubsection*{Encoding at the transmitters}
Due to the partial wireless connectivity of the network under study, in which only the eNB is connected to both users while the HeNB is only connected to $U_1$, we propose that the eNB sends
\begin{itemize}
\item \underline{p}rivate information
\begin{itemize}
\item[--]  $\mathbf{u}_{1,p}[t]$ and $\mathbf{u}_{2,p}[t]$ intended for $U_1$
\item $\mathbf{v}_{1,p}[t]$ and $\mathbf{v}_{2,p}[t]$ intended for $U_2$
\end{itemize}
\end{itemize}
while the HeNB transmits
\begin{itemize}
\item\underline{p}rivate information $\mathbf{u}_{4,p}[t]$
\item and XORed information $\mathbf{w}_{\text{IN}}[t]=\mathbf{v}_{1,p}[t]\oplus \mathbf{u}_{3,p}[t]$ for \underline{i}nterference \underline{n}eutralization
\end{itemize} 
(in the $t-$th channel use ($t=1,\ldots, T_{E}$)). The resulting signal vectors at the HeNB and eNB are chosen according to:
\begin{equation}\label{eq:ldm_stack}
\mathbf{x}_{1}[t]=\begin{pmatrix}
\mathbf{0}_{l_4} \\ \mathbf{u}_{4,p}[t] \\ \mathbf{0}_{l_3} \\ \mathbf{w}_{\text{IN}}[t] \\ \mathbf{0}_{l_2}
\end{pmatrix},\qquad \mathbf{x}_{2}[t]=\begin{pmatrix}
\mathbf{u}_{2,p}[t] \\ \mathbf{v}_{2,p}[t] \\ \mathbf{v}_{1,p}[t] \\ \mathbf{u}_{1,p}[t] \\ \mathbf{0}_{l_1}
\end{pmatrix}.
\end{equation} 
%\begin{figure}[t]
%\begin{center}
%		\LDMstack
%	\caption{Transmitted Signal Vector Structure at $t-$th Channel Use of length $q=\max\{n_{d1},n_{d2},n_{d3}\}$ at (H)eNB}	
%	\label{fig:ldm_stack}
%	\end{center}
%\end{figure}
In all schemes $\mathbf{w}_{\text{IN}}[t]=\mathbf{v}_{1,p}[t]\oplus \mathbf{u}_{3,p}[t]$ is introduced, in such a way that the interference caused by private information $\mathbf{v}_{1,p}[t]$ is completely neutralized at $U_1$. Depending on the particular channel regime, certain signal levels are zero-padded to either avoid collision of private information at $U_1$ or to reduce the transmission power level of the HeNB. In the block representation illustrated in Eq. \eqref{eq:ldm_stack} this is captured by null vectors $\mathbf{0}_{l}$ of length $l=l_1,l_2,l_3,l_4$. Since, we are interested in maximizing $\bar{L}$, we focus on transmission schemes that utilize a single channel use $T_{E}=1$. Thus, in the sequel, we drop the time dependency in our notation. We denote the length of signal vectors $\mathbf{u}_{i,p}$, $i=1,\ldots,4$, $\mathbf{v}_{j,p}$, $j=1,2$, and $\mathbf{w}_{\text{IN}}$ by $R^{u}_{i,p}$, $R^{j,v}_{p}$ and $R^{w}_{\text{IN}}$, respectively.  

For $q=\max\{n_{d1},n_{d2},n_{d3}\}$, it is obvious that the eNB, on the one hand, can generate its signal vector $\mathbf{x}_{2}$ as long as
\begin{equation}\label{eq:tx_condition_eNB}
l_1+R_{1,p}^{u}+R_{2,p}^{u}+R_{1,p}^{v}+R_{2,p}^{v}\leq q,
\end{equation} while the HeNB, on the other hand, can construct its signal vector $\mathbf{x}_{1}$ only if 
\begin{align}
\label{eq:tx_condition_HeNB_1}
l_2+l_3+l_4+R_{4,p}^{u}+R_{\text{IN}}^{w}&\leq q, \\
\label{eq:tx_condition_HeNB_2}
R_{4,p}^{u}+R_{\text{IN}}^{w}&\leq \mu \bar{L}.
\end{align} The condition \eqref{eq:tx_condition_HeNB_2} holds since the HeNB is endowed with a finite-size cache of fractional size $\mu$.

\subsubsection*{Decoding at the receivers}

The transmission according to the block structure of Eq. \eqref{eq:ldm_stack} requires that at the respective receivers interference-decoding and treating interference as noise (TIN) is applied successively. The received signal vector at $U_1$ and $U_2$ are shown in Fig. \ref{fig:rx_sig}. In what follows,  we will specify the conditions under which both $U_1$ and $U_2$ can decode their desired signal components \emph{reliably}. 

\begin{figure*}
        \centering
        \begin{subfigure}[b]{0.475\textwidth}
            \centering
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node 							distance=3cm,thick,scale=1]
				\SCHEMERxone
			\end{tikzpicture}  
            \caption{{\small Received signal at $U_1$}}    
            \label{fig:rx_u1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}  
            \centering 
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node 							distance=3cm,thick,scale=1]
				\SCHEMERxtwo
			\end{tikzpicture} 
            \caption{{\small Received signal at $U_2$}}       
            \label{fig:rx_u2}
        \end{subfigure}
                \caption{\small The received signal vector of (a) $U_1$ and (b) $U_2$ are shown. Note that $U_1$ receives the superposition $\mathbf{S}^{q-n_{d1}}\mathbf{x}_1\oplus\mathbf{S}^{q-n_{d2}}\mathbf{x}_2$.} 
        \label{fig:rx_sig}
\end{figure*}

First, let us consider $U_2$. This receiver is interested in retrieving $\mathbf{v}_{j,p}$, $j=1,2$, from its received signal $\mathbf{S}^{q-n_{d3}}\mathbf{x}_2$. Successive decoding, however, starting from the top-most significant bit levels necessitates that prior to decoding $\mathbf{v}_{j,p}$, $j=1,2$, the undesired signal vector $\mathbf{u}_{2,p}$ has to decoded and canceled from the received signal vector $\mathbf{S}^{q-n_{d3}}\mathbf{x}_2$. Thus, $U_2$ can only decode $\mathbf{v}_{j,p}$, $j=1,2$ (cf. Fig. \ref{fig:rx_u2}), as long as 
\begin{equation}\label{eq:rx_condition_U2}
R_{2,p}^{u}+R_{1,p}^{v}+R_{2,p}^{v}\leq n_{d3}.
\end{equation}   

We now move to state the reliability conditions for $U_1$. Recall that $U_1$ receives the superposition $\mathbf{S}^{q-n_{d1}}\mathbf{x}_1\oplus\mathbf{S}^{q-n_{d2}}\mathbf{x}_2$ and aims at obtaining $\mathbf{u}_{1,p},\mathbf{u}_{2,p}$ and $\mathbf{u}_{4,p}$ directly as well as $\mathbf{u}_{3,p}$ indirectly by superimposing $\mathbf{v}_{1,p}$ and $\mathbf{w}_{\text{IN}}=\mathbf{v}_{1,p}\oplus\mathbf{u}_{3,p}$. Similarly to $U_2$'s condition \eqref{eq:rx_condition_U2}, we infer that the individual signals $\mathbf{S}^{q-n_{d1}}\mathbf{x}_1$ and $\mathbf{S}^{q-n_{d2}}\mathbf{x}_2$ have to be able to carry the set of signal components $\{\mathbf{w}_{\text{IN}},\mathbf{u}_{4,p}\}$ and $\{\mathbf{u}_{1,p},\mathbf{v}_{1,p},\mathbf{v}_{2,p},\mathbf{u}_{2,p}\}$, respectively, i.e., 
\begin{align}
\label{eq:rx_condition_U1_1}
l_3+l_4+R_{4,p}^{u}+R_{\text{IN}}^{w}&\leq n_{d1}, \\
\label{eq:rx_condition_U1_2}
R_{1,p}^{v}+R_{2,p}^{v}+R_{1,p}^{u}+R_{2,p}^{u}&\leq n_{d2},
\end{align} such that the desired signals $\mathbf{u}_{i,p}$, $i=1,\ldots,4$ are all received above noise level. The remaining conditions specify how overlaps between desired components are precluded. We avoid an overlap between  $\mathbf{u}_{4,p}$ and $\mathbf{u}_{2,p}$ if
\begin{equation}\label{eq:rx_condition_U1_3}
l_4+R_{4,p}^{u}\leq (n_{d1}-n_{d2})^{+}
\end{equation} is satisfied. As shown in Fig. \ref{fig:rx_u1}, full interference neutralization
% \footnote{We note that interference neutralization is only feasible for $\mu>0$.} 
by superposing $\mathbf{v}_{1,p}$ and $\mathbf{w}_{\text{IN}}$ is ensured if on the one hand the lowest bit levels of $\mathbf{v}_{1,p}$ and $\mathbf{w}_{\text{IN}}$ are aligned, i.e.,
\begin{equation}\label{eq:rx_condition_U1_4}
R_{1,p}^{v}+R_{2,p}^{v}+R_{2,p}^{u}+n_{d1}-n_{d2}=l_3+l_4+R_{\text{IN}}^{w}+R_{4,p}^{u},
\end{equation} and, on the other hand, the allocated number of bits for $\mathbf{v}_{1,p}$ and $\mathbf{w}_{\text{IN}}$ are identical, i.e., 
\begin{equation}\label{eq:rx_condition_U1_5}
R_{1,p}^{v}=R_{\text{IN}}^{w}.
\end{equation} We point out that through the alignment conditions \eqref{eq:rx_condition_U1_4} and \eqref{eq:rx_condition_U1_5}, overlaps between $\mathbf{u}_{1,p}$ and $\mathbf{w}_{\text{IN}}$ are prohibited. When all conditions \eqref{eq:tx_condition_eNB}--\eqref{eq:rx_condition_U1_5} are satisfied, the achievable rates of $U_1$ and $U_2$ become
\begin{subequations}
\begin{alignat}{2}
R_{U_1}&=R_{\text{IN}}^{w}+R_{1,p}^{u}+R_{2,p}^{u}+R_{4,p}^{u},\label{eq:ach_rate_U1}\\
R_{U_2}&=R_{1,p}^{v}+R_{2,p}^{v},\label{eq:ach_rate_U2}
\end{alignat}   
\end{subequations} respectively. 

\subsubsection*{Maximizing $\bar{L}$} Recall that our scheme maximizes $\bar{L}$ by determining the optimal vector of design variables $\mathcal{\boldsymbol{r}}^{*}$. The design parameters of our scheme are the rate allocation parameters and the respective null vectors. To this end, all design parameters are combined to the vector
\begin{equation*}
\mathcal{\boldsymbol{r}}=\Big(R_{1,p}^{u},R_{2,p}^{u},R_{4,p}^{u},R_{1,p}^{v},R_{2,p}^{v},R_{\text{IN}}^{w},l_1,l_2,l_3,l_4\Big)^{T}.
\end{equation*} We then solve the following linear optimization problem:
\begin{equation}\label{eq:lin_opt_problem}
\begin{aligned}
& \underset{\mathcal{\boldsymbol{r}}}{\max}
& & \bar{L}\triangleq\min\{R_{U_1},R_{U_2}\} \\
& \text{s.t.}
& & \eqref{eq:tx_condition_eNB}\text{--}\eqref{eq:rx_condition_U1_5}\text{ are satisfied}, \\
&&& \mathcal{\boldsymbol{r}} \geq \mathbf{0}.
\end{aligned}
\end{equation} In the sequel, we will solve the optimization problem for various channel regimes and thus determine $\bar{L}^{*}$. Recall that this means that $\Delta_{\text{det}}(\mu,n_F=0,\mathbf{n})=\nicefrac{1}{\bar{L}^{*}}$ channel uses are required to provide each user with a single bit. Before we solve the problem \eqref{eq:lin_opt_problem} for all channel regimes, we will exemplify our scheme for a specific channel setting.  

\begin{example}[Class A channel regime]\label{example_1}
In this example, we consider the channel $\mathbf{n}=(2,5,4)^{T}$ for $n_{F}=0$. This channel belongs to the class $A$ channel regime. Theorem \ref{th:1} gives us the corner points $A_1=\Big(\mu=0,\Delta_{\text{det}}^{*}(\mu=0,n_{F}=0,\mathbf{n})=\nicefrac{2}{5}\Big)$ and $B_2=\Big(\mu^{\prime}=\nicefrac{1}{3},\Delta_{\text{det}}^{*}(\mu=\nicefrac{1}{3},n_{F}=0,\mathbf{n})=\nicefrac{1}{3}\Big)$.

\begin{figure*}[t!]
\centering
\LDMblockone
\caption{{\small Example of proposed scheme for $n_{d1}=2$, $n_{d2}=5$ and $n_{d3}=4$. The cached content of the HeNB on the requested files $W_{d_1}$ and $W_{d_2}$ are $S_{d_1}=(a_2)$ and $S_{d_2}=(b_3)$. This corresponds to a fractional cache size of $\mu^{\prime}(\mathbf{n})=\nicefrac{1}{3}$.}}
\label{fig:AcScheme}
\end{figure*} 

At extreme point $A_1$ neither fronthauling nor edge caching involving the HeNB is performed. Thus, the F-RAN under study reduces to a broadcast channel in which the eNB is responsible for transmitting the requested files while the HeNB remains silent. Thus, the only relevant channel realizations are the eNB-$U_1$ and eNB-$U_2$ links with $n_{d2}=5$ and $n_{d3}=4$. We observe that the stronger of those two channels is the eNB-$U_1$ link with $n_{d2}=5$ ($n_{d3}\leq n_{d2}$). The optimal scheme equally distributes the transmission load of $n_{d2}=5$ bits to both users. That is, by sending $\nicefrac{n_{d2}}{2}=\nicefrac{5}{2}$ private information bits in a single channel use; or, alternatively by sending one bit in $\Delta_{\text{det}}^{*}(\mu=0,n_{F}=0,\mathbf{n})=\nicefrac{2}{5}$ channel uses, to $U_1$ and $U_2$, respectively. This scheme is feasible since the weaker channel $n_{d3}$ supports the transmission of $\nicefrac{n_{d2}}{2}$ bits ($\nicefrac{n_{d2}}{2}\leq n_{d3}$). These conditions are equivalent with $\mathbf{n}\in\mathcal{I}_0$. In summary, in the block representation this scheme is given by fixing the rate allocation parameters to $R_{1,p}^{u,*}+R_{2,p}^{u,*}=R_{2,p}^{v,*}=\nicefrac{n_{d2}}{2}=\nicefrac{5}{2}$, $l_2^{*}+l_3^{*}=n_{d2}=5$ and $R_{1,p}^{v,*}=R_{4,p}^{u,*}=R_{\text{IN}}^{w,*}=l_1^{*}=l_4^{*}=0$. We refer to the proof of Lemma \ref{lemma:2} and Remark \ref{remark_bc_conditions} for further details on this scheme.  

The extreme point $B_2$ is achievable through a cache-only transmission scheme. It requires one channel use and achieves a DTB of $\nicefrac{2}{(n_{d1}+n_{d3})}=\nicefrac{1}{3}$ at fractional cache size $\mu^{\prime}(\mathbf{n})=\nicefrac{(2n_{d1}+2n_{d3}-2n_{d2})}{(n_{d1}+n_{d3})}=\nicefrac{1}{3}$. Fig. \ref{fig:AcScheme} illustrates the scheme for the case when $U_1$ and $U_2$ request $W_{d_1}=(a_1,a_2,a_3)$ and $W_{d_2}=(b_1,b_2,b_3)$, respectively. In this case where the channel of the cross link $n_{d2}$ is the strongest, it is advantageous that the eNB transmits not only private information to $U_2$ but also to $U_1$. This implies that the rates $R_{1,p}^{u}, R_{2,p}^{u}$ are chosen to be non-zero whereas $l_1^{*}=0$. When we fix $R_{1,p}^{v,*}+R_{2,p}^{v,*}=\nicefrac{(n_{d1}+n_{d3})}{2}=3$ all bits ($b_1,b_2$ and $b_3$) of $W_{d_2}$ are conveyed to $U_2$. Note that the eNB-$U_2$ link is capable of reliably carrying $R_{1,p}^{v,*}+R_{2,p}^{v,*}=3$ bits to $U_2$ because $R_{1,p}^{v,*}+R_{2,p}^{v,*}=3<n_{d3}=4$ holds. The unused signal levels at the eNB of rate $R_{1,p}^{u,*}=\nicefrac{(n_{d3}-n_{d1})}{2}=1$ and $R_{2,p}^{u,*}=n_{d2}-n_{d3}=1$ are allocated to send private information $a_1$ and $a_3$ to $U_1$. To retrieve the remaining desired bit of $U_1$ ($a_2$), the interfering bit $b_3$ of $\mathbf{v}_{1,p}$ is neutralized by sending the single XOR combination ($R_{\text{IN}}^{w,*}=n_{d1}+n_{d3}-n_{d2}=1$) $a_2\oplus b_3$ at the \emph{highest} signal level of the HeNB. This is feasible since the HeNB retains $a_2$ and $b_3$ separately in its cache during the placement phase. This constitutes a fractional cache size $\mu^{\prime}(\mathbf{n})=\nicefrac{1}{3}$. With this strategy, $U_1$ receives $R_{1,p}^{u,*}+R_{2,p}^{u,*}=\nicefrac{(2n_{d2}-n_{d1}-n_{d3})}{2}=2$ bits ($a_1$ and $a_3$) of $W_{d_1}$ from the eNB while the remaining $R_{\text{IN}}^{w,*}=n_{d1}+n_{d3}-n_{d2}=1$ bits ($a_2$) are received through network coding which involves both HeNB and eNB. Since the HeNB's fractional cache size is $\nicefrac{1}{3}$, the HeNB cannot send any additional private information. For that reason, $R_{4,p}^{u,*}=l_3^{*}=l_4^{*}=0$ and $l_2^{*}=4$. 
%When generalizing the scheme, it is easy to see that the scheme is feasible for arbitrary $\mathbf{n}\in\mathcal{C}_1$. If the achievable per-user rate is a non-integer, two channel uses are required. For further details on this case, we point to our previous work \cite{prev_work}.    

Any point between the two corner points $A_1$ and $B_2$ is achieved through file splitting and time sharing between the policies at those two corner points. Such scheme is often termed \emph{memory sharing}. 
%As the transmission at \circled{$I_a$} and \circled{$II_b$} are feasible in $\mathcal{R}_{\text{\circled{$I_a$}}}=\mathcal{I}_0$ and $\mathcal{R}_{\text{\circled{$II_b$}}}=\mathcal{C}_1$, any intermediate point in the memory-latency tradeoff curve is achievable through memory sharing in the channel regime $\mathcal{R}_{1}\triangleq\mathcal{R}_{\text{\circled{$II_b$}}}
%\cap\mathcal{R}_{\text{\circled{$I_a$}}}=\mathcal{C}_1\cap\mathcal{I}_0$. In this particular channel regime, we notice that $\mathcal{R}_{1}=\mathcal{C}_1$ because $\mathcal{C}_1\cap\mathcal{I}_0^{C}=\emptyset$. However, this is not true for all channel regimes under study.  
\end{example}
\vspace{0.5em}
In the remainder of sub-section \ref{subsec:ser_upp_bound}, we will show the achievability of all relevant corner points that are based on cache-only transmission policies ($n_{F}=0$). To this end, we specify the optimal rate allocation parameters introduced as part of the generalized block structure that optimizes the linear program \eqref{eq:lin_opt_problem}.
\vspace{0.5em}    
\subsubsection*{Scheme for Corner Point $A_1$}
The achievability at this point follows from Lemma \ref{lemma:2} and \eqref{eq:DTB_lemma} (cf. Example \ref{example_1}). At this point, the optimal DTB corresponds to
%\begin{equation} \label{eq:opt_DTB_I_a}\begin{subnumcases}{n=}
%\Delta_0(\mathbf{n})=\begin{cases}\frac{2}{n_{d2}}\text{ for }\mathbf{n}\in\mathcal{I}_0\\\frac{1}{n_{d3}}\text{ for }\mathbf{n}\in\mathcal{I}_0^{C}\\\frac{2}{n_{d3}}\text{ for }\mathbf{n}\in\mathcal{I}_1\\\frac{1}{n_{d2}}\text{ for }\mathbf{n}\in\mathcal{I}_1^{C}\end{cases}.\ed{numcases}
%\end{equation}
%\begin{equation} \label{eq:opt_DTB_I_a}
\begin{subnumcases}{\Delta_0(\mathbf{n})=}
\frac{2}{n_{d2}}\text{ for }\mathbf{n}\in\mathcal{I}_0\\\frac{1}{n_{d3}}\text{ for }\mathbf{n}\in\mathcal{I}_0^{C}\\\frac{2}{n_{d3}}\text{ for }\mathbf{n}\in\mathcal{I}_1\\\frac{1}{n_{d2}}\text{ for }\mathbf{n}\in\mathcal{I}_1^{C}.\end{subnumcases}
%\end{equation}
%This is achieved by setting the rate allocation parameters to $l_2=\max\{n_{d1},n_{d2},n_{d3}\}$, $R_{p}^{v}=\nicefrac{1}{\Delta_0(\mathbf{n})}$, $l_1=l_2-\nicefrac{2}{\Delta_0(\mathbf{n})}$, 
%\begin{equation}\label{eq:R_1_p_R_2_p_u}
%(R_{1,p}^{u},R_{2,p}^{u})^{T}=\begin{cases}(\nicefrac{1}{\Delta_0(\mathbf{n})},0)\text{ for } n_{d2}\geq n_{d3}\\(0,\nicefrac{1}{\Delta_0(\mathbf{n})})\text{ for } n_{d2}\leq n_{d3}\end{cases},
%\end{equation}
%and the remaining variables to $0$. 
We observe that the achievable DTB is in accordance with Theorem \ref{th:1} for $\mu=0$. 

\subsubsection*{Scheme for Corner Point \circled{$II_b$}}

% Control
\newcolumntype{C}{>{\centering\arraybackslash}p{4.0em}}
\begin{table}[t]
%\centering
\caption{Rate allocation parameters for corner point \protect\circled{$II_b$} at fractional cache size $\mu^{\prime}(\mathbf{n})$}
\label{tab:rate_alloc_param}
\begin{tabular}{|c||c|C|C|c|c|c|c|}
\hline
Regime & $\mathcal{C}_1$ & $\mathcal{R}_2$ & $\mathcal{R}_3$ & $\mathcal{C}_4$ & $\mathcal{R}_{51}$ & $\mathcal{C}_{52}$ & $\mathcal{C}_{61}$ 
\\ \hline 
$R_{3,p}^{u}$ & $0$ & \multicolumn{2}{c|}{$0$} & $n_{d3}-n_{d2}$ & $0$ & $0$ & $n_{d1}-n_{d2}$
\\ \hline
$R_{2,p}^{u}$ & $\frac{n_{d3}-n_{d1}}{2}$ &  \multicolumn{2}{c|}{$0$} & $0$ & $n_{d3}-n_{d2}$ & $\frac{n_{d3}-n_{d1}}{2}$ & $n_{d3}-n_{d1}$  
\\ \hline
$R_{1,p}^{u}$ & $n_{d2}-n_{d3}$ &  \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $0$ & $0$ & $0$ 
\\ \hline
$R_{\text{IN}}^{w}$  & $n_{d1}+n_{d3}-n_{d2}$ & \multicolumn{2}{c|}{$2n_{d3}-n_{d2}$} & $n_{d2}$ & $2n_{d2}-n_{d3}$ & $n_{d1}$ & $n_{d1}+n_{d2}-n_{d3}$
\\ \hline
$R_{p}^{v}$  & $\frac{n_{d1}+n_{d3}}{2}$ & \multicolumn{2}{c|}{$n_{d3}$} & $n_{d3}$ & $n_{d2}$ & $\frac{n_{d1}+n_{d3}}{2}$ & $n_{d1}$ 
\\ \hline
$l_4$ & \multicolumn{3}{c|}{$0$} & $n_{d1}-n_{d3}$ & \multicolumn{3}{c|}{$0$}
\\ \hline
$l_3$ & $0$ & $n_{d2}-n_{d3}$ & $n_{d1}-n_{d3}$ & $0$ & $n_{d1}+n_{d3}-2n_{d2}$ & $0$ & $n_{d3}-n_{d1}$  
\\ \hline
$l_2$ & $2n_{d2}-n_{d1}-n_{d3}$ & \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d1}$
\\ \hline
$l_1$ & $0$ & $0$ & $n_{d1}-n_{d2}$ & $n_{d1}-n_{d3}$ & $0$ & $0$ & $0$ 
\\ \hline
\end{tabular}
\end{table}

The encoding at the transmitters, both eNB and HeNB, follows along the block building structure of Fig. \ref{fig:ldm_stack}. Similarly to Example \ref{example_1}, the length of each signal vector is appropriately determined to individually account for all channel regimes while maximizing the \emph{symmetric} per-use rate. This has the effect that the latency of providing each user with its requested file are the same. All the proposed schemes require $T_{E}=1$ channel use to perform optimally. Table \ref{tab:rate_alloc_param} indicates the rate allocation parameters and the \emph{largest} channel regime set under which \eqref{eq:user_rate_1_and_2} and \eqref{eq:cache_size_req} are both satisfied. Note that the achievable DTB and $\mu^{\prime}_{\text{Ach}}$ (specified in \eqref{eq:frac_cache_size}) match \eqref{eq:DTB_theorem_th_1_low_fronthaul}, \eqref{eq:DTB_theorem_cloud_th_2_low_fronthaul} and \eqref{eq:mu_prime}, respectively.
\vspace{0.5em}
\subsubsection*{Scheme for Corner Points \circled{$II_a$} and \circled{$III$}} 

% Control
\newcolumntype{C}{>{\centering\arraybackslash}p{6.0em}}
\begin{table}[h]
\centering
\setlength\tabcolsep{4pt}
\begin{minipage}{0.48\textwidth}
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$II_a$} at fractional cache size $\mu^{\prime\prime}(\mathbf{n})$}
\begin{tabular}{|c||C|C|}
\hline
Regime & $\mathcal{R}_{4}^{\prime}$ & $\mathcal{R}_{61}^{\prime}$ \\ \hline 
$R_{3,p}^{u}$ & \multicolumn{2}{c|}{$n_{d3}-2n_{d2}$} \\ \hline
$R_{2,p}^{u}$ & \multicolumn{2}{c|}{$n_{d2}$} \\ \hline
$R_{1,p}^{u}$ & \multicolumn{2}{c|}{$0$} \\ \hline
$R_{\text{IN}}^{w}$  & \multicolumn{2}{c|}{$0$} \\ \hline
$R_{p}^{v}$  & \multicolumn{2}{c|}{$n_{d3}-n_{d2}$} \\ \hline
$l_4$ & \multicolumn{2}{c|}{$n_{d1}+n_{d2}-n_{d3}$} \\ \hline
$l_3$ & $n_{d2}$ & $n_{d2}+n_{d3}-n_{d1}$ \\ \hline
$l_2$ & \multicolumn{2}{c|}{$0$} \\ \hline
$l_1$ & $n_{d1}-n_{d3}$ & $0$ \\ \hline
\end{tabular}
\label{tab:rate_alloc_II_a} 
\end{minipage}%
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$III$} at fractional cache size $\mu^{\prime\prime\prime}(\mathbf{n})$} 
\begin{tabular}{|c||c|}
\hline
Regime & $\mathcal{C}_{62}$ \\ \hline 
$R_{3,p}^{u}$ & $n_{d1}-n_{d2}$ \\ \hline
$R_{2,p}^{u}$ & $n_{d2}$ \\ \hline
$R_{1,p}^{u}$ & $0$ \\ \hline
$R_{\text{IN}}^{w}$  & $0$ \\ \hline
$R_{p}^{v}$  & $n_{d1}$ \\ \hline
$l_4$ & $0$ \\ \hline
$l_3$ & $0$ \\ \hline
$l_2$ & $n_{d2}+n_{d3}-n_{d1}$ \\ \hline
$l_1$ & $n_{d3}-n_{d1}-n_{d2}$ \\ \hline
\end{tabular}
\label{tab:rate_alloc_III} 
\end{minipage}
\end{table}

For these two corner points, we adopt the general block structure of Fig. \ref{fig:ldm_stack}. Tables \ref{tab:rate_alloc_II_a} and \ref{tab:rate_alloc_III} outline the rate allocation parameters for both extreme points.    


\subsection{Lower Bound (Converse) on the Minimum DTB for $n_{F}\geq 0$}
\label{subsec:ser_low_bound_nF_greater_0}

\begin{proposition}[Lower Bound on the Minimum DTB]\label{prop:2}
For the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} with $n_F\geq 0$, the optimal DTB $\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})$ is lower bounded as
\begin{equation}
\label{eq:ser_lb_cache_only_nF_greater_0}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})\geq\Delta_{\text{LB}}(\mu,n_F,\mathbf{n}),
\end{equation}
where $\Delta_{\text{LB}}(\mu,n_F,\mathbf{n})$ is the solution of the linear optimization problem
\begin{subequations}
\label{eq:lb_cache_only_nF_greater_0}
\begin{align}
& \underset{\Delta_{E},\Delta_{F}}{\text{minimize}}
& & \Delta_{E}+\Delta_{F} \label{eq:zielfunktion}\\
& \text{subject to}
& & \Delta_{E}+\Delta_{F}\frac{n_{F}}{\max\{n_{d2},n_{d3}\}} \geq \frac{2-\mu}{\max\{n_{d2},n_{d3}\}} \label{eq:constraint_1}\\
& & & \Delta_{E}+\Delta_{F}\frac{n_{F}}{n_{d2}} \geq \frac{1-\mu}{n_{d2}} \label{eq:constraint_2}\\
& & & \Delta_{E}\geq \max\Bigg\{\frac{1}{n_{d3}},\frac{1}{\max\{n_{d1},n_{d2}\}},\frac{2}{\max\{n_{d1}+n_{d3},n_{d2}\}}\Bigg\} \label{eq:constraint_3}\\
& & & \Delta_{F}\geq 0 \label{eq:constraint_4}
\end{align}
\end{subequations}
and $\Delta_{E}$ and $\Delta_{F}$ denoting the individual DTBs of wireless and fronthaul transmissions. 
\end{proposition}
\noindent\begin{IEEEproof}
The proof of Proposition \ref{prop:2} is presented in Appendix \ref{app:lw_bound_ser_nF_greater_0}.   
\end{IEEEproof}
We next present multiple corollaries that specialize the lower bound of Proposition \ref{prop:2} to different settings of fronthaul capacities $n_{F}$. 
\begin{corollary}[Lower Bound for Low-Fronthaul Capacity Regime]\label{corr:1} For the F-RAN under study in the low-fronthaul capacity regime with $n_{F}\leq n_{d2}$, the DTB is lower bounded as
\begin{equation}\label{eq:lw_bound_low_fronthaul_capacity_regime}
\Delta^{*}_{\text{det}}(\mu,n_{F},\mathbf{n})\geq \max\Bigg\{\frac{1}{n_{d3}},\frac{1}{\max\{n_{d1},n_{d2}\}},\frac{2}{\max\{n_{d1}+n_{d3},n_{d2}\}},\frac{1-\mu}{n_{d2}},\frac{2-\mu}{\max\{n_{d2},n_{d3}\}}\Bigg\}. 
\end{equation}
\end{corollary}
\noindent \begin{IEEEproof}
We note that the lower bound on the wireless DTB $\Delta_{E}$ (see \eqref{eq:constraint_3}) is also a valid bound on the DTB $\Delta_{E}+\Delta_{F}$ due to the non-negativity of the fronthaul DTB $\Delta_{F}$ (cf. \eqref{eq:constraint_4}). Furthermore, for $n_{F}\leq n_{d2}$ the left-hand side (LHS) of \eqref{eq:constraint_1} and \eqref{eq:constraint_2} are upper bounded by the overall DTB $\Delta_{E}+\Delta_{F}$. Thus, \eqref{eq:constraint_1}--\eqref{eq:constraint_3} are all active lower bounds on the DTB. This concludes the proof.   
\end{IEEEproof}
\begin{remark} We see that the lower bound on the DTB $\Delta_{E}+\Delta_{F}$ in \eqref{eq:lw_bound_low_fronthaul_capacity_regime} coincides with the lower bound on $\Delta_{E}$ for $n_{F}=0$ in Proposition \ref{prop:1}. 
\end{remark}
\begin{corollary}[Lower Bound for High-Fronthaul Capacity Regime]\label{corr:2} For the F-RAN under study in the high-fronthaul capacity regime with $n_{F}\geq\max\{n_{d2},n_{d3}\}$, the DTB is lower bounded as
\begin{align}\label{eq:lw_bound_high_fronthaul_capacity_regime}
\Delta^{*}_{\text{det}}(\mu,n_{F},\mathbf{n})\geq \max\Bigg\{&\frac{2-\mu}{n_F}+\Bigg(1-\frac{\max\{n_{d2},n_{d3}\}}{n_{F}}\Bigg)\Delta_{\text{LB}}^{\prime}(\mathbf{n}),\nonumber\\& \frac{1-\mu}{n_{F}}+\Bigg(1-\frac{n_{d2}}{n_{F}}\Bigg)\Delta_{\text{LB}}^{\prime}(\mathbf{n}),\:\: \Delta_{\text{LB}}^{\prime}(\mathbf{n})\Bigg\}, 
\end{align} where $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ is defined in \eqref{eq:dlb_main}.
\end{corollary}
\noindent \begin{IEEEproof}
First, we note that $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ is identical to the right-hand side (RHS) of \eqref{eq:constraint_3}. This bound is a valid bound on the DTB $\Delta_{E}+\Delta_{F}$. For $n_{F}\geq\max\{n_{d2},n_{d3}\}$, we combine \eqref{eq:constraint_1} and \eqref{eq:constraint_2} with \eqref{eq:constraint_3}, which yields
\begin{subequations}
\label{eq:lb_reformulate_high_fronthaul}
\begin{align}
\Delta_{E}+\Delta_{F} & \geq \frac{2-\mu}{n_F}+\Bigg(1-\frac{\max\{n_{d2},n_{d3}\}}{n_{F}}\Bigg)\Delta_{\text{LB}}^{\prime}(\mathbf{n}) \label{eq:reformulate_constraint_1_high_fronthaul}\\
\Delta_{E}+\Delta_{F} & \geq \frac{1-\mu}{n_{F}}+\Bigg(1-\frac{n_{d2}}{n_{F}}\Bigg)\Delta_{\text{LB}}^{\prime}(\mathbf{n}). \label{eq:reformulate_constraint_2_high_fronthaul}
\end{align}
\end{subequations} The RHSs of inequalities \eqref{eq:reformulate_constraint_1_high_fronthaul}, \eqref{eq:reformulate_constraint_2_high_fronthaul} and \eqref{eq:constraint_3} result in \eqref{eq:lw_bound_high_fronthaul_capacity_regime} of Corollary \ref{corr:2}.    
\end{IEEEproof}
\begin{corollary}[Lower Bound for Medium-Fronthaul Capacity Regime in $\mathcal{I}_1$]\label{corr:3} For the F-RAN under study in the medium-fronthaul capacity regime $n_{F}\in[n_{d2},\max\{n_{d2},n_{d3}\}]$ and channel regime $\mathbf{n}\in\mathcal{I}_1$, the DTB is lower bounded as
\begin{align}\label{eq:lw_bound_medium_fronthaul_capacity_regime}
\Delta^{*}_{\text{det}}(\mu,n_{F},\mathbf{n})\geq \max\Bigg\{&\frac{2-\mu}{n_{d3}},\:\: \Delta_{\text{LB}}^{\prime}(\mathbf{n})\Bigg\}, 
\end{align} where $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ is defined in \eqref{eq:dlb_main}.
\end{corollary}
\noindent \begin{IEEEproof}
We observe that for $n_{F}\leq \max\{n_{d2},n_{d3}\}$, $\Delta_{E}+\Delta_{F}$ is an upper bound on the LHS of \eqref{eq:constraint_1}. For $\mathbf{n}\in\mathcal{I}_1$, it is easy to see that for any $\mu\in[0,1]$
\begin{equation}\label{eq:inequality_medium_fronthaul_I_1}
\Delta_{E}+\Delta_{F}\geq \frac{2-\mu}{n_{d3}}\geq\frac{1-\mu}{n_{d2}}
\end{equation} holds. Thus, only \eqref{eq:constraint_1} and \eqref{eq:constraint_3} are active lower bounds on the DTB. Combining these two bounds leads to \eqref{eq:lw_bound_medium_fronthaul_capacity_regime}.  
\end{IEEEproof}
\begin{corollary}[Lower Bound for Medium-Fronthaul Capacity Regime in $\mathcal{I}_1^{C}$]\label{corr:4} For the F-RAN under study in the medium-fronthaul capacity regime $n_{F}\in[n_{d2},\max\{n_{d2},n_{d3}\}]$ and channel regime $\mathbf{n}\in\mathcal{I}_1^{C}$, the DTB is lower bounded as
\begin{align}\label{eq:lw_bound_medium_fronthaul_capacity_regime_I1_C}
\Delta^{*}_{\text{det}}(\mu,n_{F},\mathbf{n})\geq\begin{cases}\max\Big\{\frac{1-\mu}{n_F}+\big(1-\frac{n_{d2}}{n_F}\big)\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n}),\:\:\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})\Big\}&\text{ for }\mu\leq \mu^{\prime\prime}(\mathbf{n})\\\max\Big\{\frac{2-\mu}{n_{d3}},\:\: \Delta_{\text{LB}}^{\prime}(\mathbf{n})\Big\}&\text{ for }\mu\geq \mu^{\prime\prime}(\mathbf{n})\end{cases}, 
\end{align} where $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ is defined in \eqref{eq:dlb_main} and $\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})$ equals
\begin{equation}\label{eq:delta_LB_prime_prime}
\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})=\max\Bigg\{\frac{1}{n_{d3}-n_{d2}},\:\:\Delta_{\text{LB}}^{\prime}(\mathbf{n})\Bigg\}.
\end{equation}
\end{corollary}
\noindent \begin{IEEEproof}
We observe that for $n_{F}\leq n_{d3}$, $\Delta_{E}+\Delta_{F}$ is an upper bound on the LHS of \eqref{eq:constraint_1}. For $\mathbf{n}\in\mathcal{I}_1^{C}$, one can show that for any $\mu\in[\mu^{\prime\prime}(\mathbf{n}),1]$
\begin{equation}\label{eq:inequality_medium_fronthaul_I_1}
\Delta_{E}+\Delta_{F}\geq \frac{2-\mu}{n_{d3}}\geq\frac{1-\mu}{n_{d2}}
\end{equation} holds. We infer that for this case only \eqref{eq:constraint_1} and \eqref{eq:constraint_3} are active lower bounds on the DTB. Combining these two bounds leads to the second case of \eqref{eq:lw_bound_medium_fronthaul_capacity_regime_I1_C}. For $\mu\in[0,\mu^{\prime\prime}(\mathbf{n})]$, on the other hand, we bound \eqref{eq:constraint_1} as follows:
\begin{eqnarray}\label{eq:bounding_constraint_1}
%\Delta_{E}+\Delta_{F}\geq \Delta_{E}+\Delta_{F}\frac{n_{F}}{n_{d3}}\geq \Delta_{E}\stackrel{(a)}\geq\frac{2-\mu}{n_{d3}}\geq \frac{2-\mu}{n_{d3}} \Bigg|_{\mu=\mu^{\prime\prime}(\mathbf{n})}=\frac{1}{n_{d3}-n_{d2}}
\Delta_{E}+\Delta_{F}\geq \Delta_{E}+\Delta_{F}\frac{n_{F}}{n_{d3}}\geq \Delta_{E}\geq\frac{2-\mu}{n_{d3}}\geq \frac{2-\mu}{n_{d3}} \Bigg|_{\mu=\mu^{\prime\prime}(\mathbf{n})}=\frac{1}{n_{d3}-n_{d2}}
\end{eqnarray} 
Using \eqref{eq:bounding_constraint_1} and \eqref{eq:constraint_3} together gives us a new lower bound \eqref{eq:delta_LB_prime_prime} on $\Delta_{E}$ (and ultimately on $\Delta_{E}+\Delta_{F}$). We obtain an additional bound on the DTB by combining \eqref{eq:delta_LB_prime_prime} and \eqref{eq:constraint_2}. This concludes the proof.     
\end{IEEEproof}
\subsection{Upper Bound (Achievability) on the Minimum DTB for $n_{F}\geq 0$}
\label{subsec:ser_upp_bound_nF_greater_0}

In this sub-section, we propose schemes to cover different operating channel regimes of the network under study for the cloud-only ($\mu=0$) case. As previously explained, we will only focus on the achievability at corner points \circled{$I_r$}, $r\in\{b,c,d\}$. Remaining intermediate points in the tradeoff curves on the DTB follow from the the convexity of the DTB (cf. Lemma \ref{lemma:1}). To show the achievability at extreme point
\begin{enumerate}[label=(\Alph*)]
\item \circled{$I_b$},
\item \circled{$I_c$}
\item and \circled{$I_d$},
\end{enumerate} we borrow results on the achievability of the \emph{cache-only case} of their respective, neighboring extreme point
\begin{enumerate}[label=(\Alph*)]
\item \circled{$II_b$}
\item \circled{$II_a$}
\item and \circled{$III$}
\end{enumerate} at cache sizes $\mu^{\prime}(\mathbf{n}), \mu^{\prime\prime}(\mathbf{n})$ and $\mu^{\prime\prime\prime}(\mathbf{n})$, respectively. In the sequel, we use the notation of the building block structure of sub-section \ref{subsec:ser_upp_bound}. We denote the requested file of $U_k$, $k=\{1,2\}$, by $W_{dk}$. 

The general idea of our proposed scheme is to apply a fronthaul transmission policy in such a way that the optimal \emph{wireless} latency $\Delta_{E}^{*}(\mu_{G}(\mathbf{n}),n_{F}=0,\mathbf{n})$ of the neighboring extreme points \circled{$II_b$}, \circled{$II_a$} and \circled{$III$} achieved at cache sizes $\mu_{G}(\mathbf{n})\in\{\mu^{\prime}(\mathbf{n}), \mu^{\prime\prime}(\mathbf{n}), \mu^{\prime\prime\prime}(\mathbf{n})\}$ become feasible at $\mu=0$ at the cost of additional fronthaul latency. $\Delta_{E}^{*}$ incurs when transmitting the requested files, each of length $L=R_{U}$ (see \eqref{eq:user_rate_1_and_2}), to $U_1$ and $U_2$ through the wireless channel without invoking the fronthaul link. Recall that the achievability of $\Delta_{E}^{*}(\mu_{G}(\mathbf{n}),n_{F}=0,\mathbf{n})$ was discussed in sub-section \ref{subsec:ser_upp_bound}. The rate allocation parameters are available in Tables \ref{tab:rate_alloc_param} through \ref{tab:rate_alloc_III}. To this end, the cloud server forms 
\begin{enumerate}[label=(\alph*)]
\item $R_{3,p}^{u}$ UNXORed bits of $W_{d1}$
\item and $R_{\text{IN}}^{w}$ XORed bits of $W_{d1}$ and $W_{d2}$
\end{enumerate} in the same manner as in the achievability scheme of \circled{$II_b$}, \circled{$II_a$} and \circled{$III$}, respectively. These bits are transmitted through the fronthaul link to the HeNB. Recall from Equation \eqref{eq:frac_cache_size} and Tables \ref{tab:rate_alloc_param} through \ref{tab:rate_alloc_III} that $\mu_{G}(\mathbf{n})L=R_{3,p}^{u}+R_{\text{IN}}^{w}$. Transmitting these $\mu_{G}(\mathbf{n})L$ bits induces a latency of $\Delta_{F}=\nicefrac{\mu_{G}(\mathbf{n})}{n_F}$. Thus, the overall DTB-latency becomes $\Delta_{E}+\Delta_{F}$, that is,
\begin{enumerate}[label=(\Alph*)]
\item \begin{equation}
\Delta_{\text{LB}}^{\prime}(\mathbf{n})+\frac{\mu^{\prime}(\mathbf{n})}{n_F} \end{equation}
\item \begin{equation}
\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})+\frac{\mu^{\prime\prime}(\mathbf{n})}{n_F} \end{equation}
\item and \begin{equation}
\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})+\frac{\mu^{\prime\prime\prime}(\mathbf{n})}{n_F}, \end{equation}
\end{enumerate} which is identical to $\Delta^{*}_{\text{det}}(\mu=0,n_F,\mathbf{n})$ of Theorem \ref{th:1}--\ref{th:3} for the underlying fronthaul capacity and channel regimes.

%In sub-section \ref{subsec:ser_upp_bound}, we have seen that cache-only schemes achieve the optimal DTB $\Delta_{E}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ at fractional cache size $\mu^{\prime}(\mathbf{n})$ in extreme point \circled{$II_b$}. This latency incurs when transmitting the requested files, each of length $L=R_{U}$ (see \eqref{eq:user_rate_1_and_2}), to $U_1$ and $U_2$ through the wireless channel without invoking the fronthaul link. At $\mu=0$ and $n_F\geq\max\{n_{d2},n_{d3}\}$, the exact same optimal \emph{wireless latency} $\Delta_{E}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ can be achieved at the cost of additional fronthaul latency $\Delta_{F}$. To this end, the cloud server forms 
%\begin{enumerate}[label=(\alph*)]
%\item $R_{3,p}^{u}$ UNXORed bits of $W_{d1}$
%\item and $R_{\text{IN}}^{w}$ XORed bits of $W_{d1}$ and $W_{d2}$
%\end{enumerate} in the same manner as in achievability scheme for \circled{$II_b$} and transmits them through its fronthaul link to the HeNB. We recall from Equation \eqref{eq:frac_cache_size} that $\mu^{\prime}(\mathbf{n})L=R_{3,p}^{u}+R_{\text{IN}}^{w}$. Transmitting these $\mu^{\prime}(\mathbf{n})L$ bits induces a latency of $\Delta_{F}=\nicefrac{\mu^{\prime}(\mathbf{n})}{n_F}$. Thus, the overall DTB-latency becomes $\Delta_{E}+\Delta_{F}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})+\nicefrac{\mu^{\prime}(\mathbf{n})}{n_F}$, which is identical to $\Delta^{*}_{\text{det}}(\mu=0,n_F,\mathbf{n})$ of Theorem \ref{th:1} and \ref{th:2} for $n_F\geq\max\{n_{d2},n_{d3}\}$ and $\mu^{\prime}(\mathbf{n})$ given in \eqref{eq:mu_prime}.
%  
%\vspace{0.5em}
%\subsubsection*{Scheme for Corner Point \circled{$I_b$}}
%
%In sub-section \ref{subsec:ser_upp_bound}, we have seen that cache-only schemes achieve the optimal DTB $\Delta_{E}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ at fractional cache size $\mu^{\prime}(\mathbf{n})$ in extreme point \circled{$II_b$}. This latency incurs when transmitting the requested files, each of length $L=R_{U}$ (see \eqref{eq:user_rate_1_and_2}), to $U_1$ and $U_2$ through the wireless channel without invoking the fronthaul link. At $\mu=0$ and $n_F\geq\max\{n_{d2},n_{d3}\}$, the exact same optimal \emph{wireless latency} $\Delta_{E}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ can be achieved at the cost of additional fronthaul latency $\Delta_{F}$. To this end, the cloud server forms 
%\begin{enumerate}[label=(\alph*)]
%\item $R_{3,p}^{u}$ UNXORed bits of $W_{d1}$
%\item and $R_{\text{IN}}^{w}$ XORed bits of $W_{d1}$ and $W_{d2}$
%\end{enumerate} in the same manner as in achievability scheme for \circled{$II_b$} and transmits them through its fronthaul link to the HeNB. We recall from Equation \eqref{eq:frac_cache_size} that $\mu^{\prime}(\mathbf{n})L=R_{3,p}^{u}+R_{\text{IN}}^{w}$. Transmitting these $\mu^{\prime}(\mathbf{n})L$ bits induces a latency of $\Delta_{F}=\nicefrac{\mu^{\prime}(\mathbf{n})}{n_F}$. Thus, the overall DTB-latency becomes $\Delta_{E}+\Delta_{F}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})+\nicefrac{\mu^{\prime}(\mathbf{n})}{n_F}$, which is identical to $\Delta^{*}_{\text{det}}(\mu=0,n_F,\mathbf{n})$ of Theorem \ref{th:1} and \ref{th:2} for $n_F\geq\max\{n_{d2},n_{d3}\}$ and $\mu^{\prime}(\mathbf{n})$ given in \eqref{eq:mu_prime}.

%\subsubsection*{Scheme for Corner Point \circled{$I_c$} and \circled{$I_d$}}
%In the previous sub-section, we have seen that \emph{irrespective} of $n_F$ the optimal DTB $\nicefrac{T_E}{L}=\nicefrac{2}{(n_{d1}+n_{d3})}$ is achieved at fractional cache size $\mu^{\prime}$. This latency incurs when transmitting the requested files, each of length $L=n_{d1}+n_{d3}$, to $U_1$ and $U_2$ through the wireless channel without invoking the fronthaul link. At $\mu=0$ and $n_F\geq\max\{n_{d2},n_{d3}\}$, the exact same optimal wireless latency $\nicefrac{T_E}{L}=\nicefrac{2}{(n_{d1}+n_{d3})}$ can be achieved at the cost of additional fronthaul latency $\nicefrac{T_F}{L}$. To this end, the cloud server forms $\mu^{\prime}L=2(n_{d1}+n_{d3}-n_{d2})$ XORed bits (cf. Fig. 3(a) and (b)) of files $W_1$ and $W_2$ and transmits them through its fronthaul link to the HeNB. This fronthaul transmission induces a latency of $\nicefrac{T_F}{L}=\nicefrac{\mu^{\prime}}{n_F}$. Thus, the overall DTB-latency becomes $\nicefrac{T_F}{L}+\nicefrac{T_E}{L}$, which is identical to $\Delta^{*}_{\text{det}}(\mu=0,n_F)$.        



==> content/cache_separability_par.tex <==
%\subsubsection*{Scheme for Corner Points \circled{$II_a$}, \circled{$II_b$} and \circled{$III$}}  
%The schemes for these three corner points are directly deducible from schemes for corner points \circled{$II_{a,S}$}, \circled{$II_{b,S}$} and \circled{$III_{S}$} of the serial fronthaul-edge transmission (see sub-section \ref{subsec:ser_upp_bound}). In this paragraph, we use the indices $S$ and $P$ to distinguish corner points of serial transmissions from those for parallel transmissions. Through careful comparison of Theorems \ref{th:1}--\ref{th:3} with \ref{th:5}--\ref{th:7}, one can verify that \begin{subequations}
%\label{eq:mu_par_vs_mu_ser}
%\begin{alignat}{3}
%\mu_{S}^{\prime}(\mathbf{n})L&=\mu_{P}^{\prime}(n_F,\mathbf{n})L+n_{F},\label{eq:mu_par_vs_mu_ser_1}\\ \mu_{S}^{\prime\prime}(\mathbf{n})L&=\mu_{P}^{\prime\prime}(n_F,\mathbf{n})L+n_{F},\label{eq:mu_par_vs_mu_ser_2} \\ \mu_{S}^{\prime\prime\prime}(\mathbf{n})L&=\mu_{P}^{\prime\prime\prime}(n_F,\mathbf{n})L+n_{F}.\label{eq:mu_par_vs_mu_ser_3}
%\end{alignat}
%\end{subequations}
%These equations suggest that the HeNB's cached content at corner points \circled{$II_{a,S}$}, \circled{$II_{b,S}$} and \circled{$III_{S}$} are separable into two distinct components attributed to edge caching and fronthauling for the case of parallel transmission. 
%
%In the following, we explicitly account for the cache separability and propose how to map the achievability scheme of serial to parallel fronthaul-edge transmission. The mapping is done as follows:
%
%We keep the signal structure for both cases identical, i.e.,  
%\begin{subequations}
%\label{eq:decomposing_signals}
%\begin{alignat}{3}
%\mathbf{u}_{i,p}^{P}[t]&=\mathbf{u}_{i,p}^{S},\qquad i=1,\ldots,3,\label{eq:decomposing_signals_1}\\ \mathbf{v}_{1,p}^{P}[t]&=\mathbf{v}_{p}^{S},\label{eq:decomposing_signals_2} \\ \mathbf{w}_{\text{IN }}^{P}[t]&=\mathbf{w}_{\text{IN }}^{S},\label{eq:decomposing_signals_3}
%\end{alignat}
%\end{subequations} for $t=[t_1:t_2],\forall b$. These equalities are tantamount to identical rate allocation. Thus, the rates of the remaining signal vectors of the generalized block structure in Fig. \ref{fig:ldm_stack_par}, the fronthaul-edge transmission block and $\mathbf{v}_{2,p}^{P}[t]$, are set to $0$. To account for the separability of the HeNB's cached of serial transmission according to \eqref{eq:mu_par_vs_mu_ser}, we decompose signals $\mathbf{u}_{3,p}[t]$ and $\mathbf{w}_{\text{IN}}[t]$ for the parallel transmission case into sub-signals attributed to edge caching and fronthauling (indices $C$ and $F$) according to
%\begin{subequations}
%\label{eq:decomposing}
%\begin{alignat}{2}
%\mathbf{u}_{3,p}[t]&=\Big(\mathbf{u}_{3,p}^{C}[t]),\mathbf{u}_{3,p}^{F}[t]\Big)^{T},\label{eq:decomposing_1}\\ \mathbf{w}_{\text{IN}}[t]&=\Big(\mathbf{w}_{\text{IN}}^{C}[t],\mathbf{w}_{\text{IN}}^{F}[t]\Big)^{T},\label{eq:decomposing_2}
%\end{alignat}
%\end{subequations} with rate allocation 
%\begin{subequations}
%\label{eq:decomposing_rate}
%\begin{alignat}{2}
%R_{3,p}^{F}[t]+R_{\text{IN}}^{F}[t]&=n_{F},
%\label{eq:decomposing_rate_1}\\ R_{3,p}^{C}[t]+R_{\text{IN}}^{C}[t]&=\begin{cases}\mu_{P}^{\prime}(n_{F},\mathbf{n})L=\mu_{S}^{\prime}(\mathbf{n})L-n_F\quad&\text{ at \circled{$II_b$}}\\\mu_{P}^{\prime\prime}(n_{F},\mathbf{n})L=\mu_{S}^{\prime\prime}(\mathbf{n})L-n_F\quad&\text{ at \circled{$II_a$}}\\\mu_{P}^{\prime\prime\prime}(n_{F},\mathbf{n})L=\mu_{S}^{\prime\prime\prime}(\mathbf{n})L-n_F\quad&\text{ at \circled{$III$}} \end{cases},\label{eq:decomposing_rate_2}
%\end{alignat}
%\end{subequations} for $t=[t_1:t_2],\forall b$, and
%\begin{equation}\label{eq:nF_max_corner_points_II_III}
%n_{F}\leq\begin{cases}\mu_{S}^{\prime}(\mathbf{n})L\quad&\text{ at \circled{$II_b$}}\\\mu_{S}^{\prime\prime}(\mathbf{n})L\quad&\text{ at \circled{$II_a$}}\\\mu_{S}^{\prime\prime\prime}(\mathbf{n})L\quad&\text{ at \circled{$III$}}\end{cases}.
%\end{equation} This concludes the achievability at these points for the case of parallel transmission. 

%Thus, the required number of cached bits for parallel transmission reduces by $n_F$ bits through fronthaul.
%Thus, the rate allocation parameters of parallel and serial transmission are identical except of fixing  
%We can therefore map the achievability scheme of serial to parallel fronthaul-edge transmission. The mapping is done by setting the rate allocation parameters of the parallel transmission    
% 


==> content/old_stuff_maybe_useful_later.tex <==
This results in Theorems \ref{th:1}--\ref{th:4}. To state these theorems we define the following channel regimes $\{\mathcal{C}_i\}_{i=1}^{6}$. 
\begin{equation}\label{eq:basic_channel_regimes}
\begin{cases}\mathcal{C}_1=\{n_{d1}+n_{d3}\geq n_{d2}\geq n_{d3} \geq n_{d1}\}\\\mathcal{C}_2=\{n_{d1}+n_{d3}\geq n_{d2}\geq n_{d1} \geq n_{d3}\}\\\mathcal{C}_3=\{n_{d1}+n_{d3}\geq n_{d1}\geq n_{d2} \geq n_{d3}\}\\\mathcal{C}_4=\{n_{d1}\geq n_{d3} \geq n_{d2}\}\\\mathcal{C}_5=\{n_{d1}+n_{d3}\geq n_{d3}\geq n_{d2} \geq n_{d1}\}\\\mathcal{C}_6=\{n_{d3}\geq n_{d1}\geq n_{d2}\}\\
\mathcal{C}_7=\{n_{d2}\geq n_{d1}+n_{d3}\}\end{cases}
\end{equation}
As far as $\mathcal{C}_5$ and $\mathcal{C}_6$ are concerned, we have to split each of them further into disjoint sub-channel regimes according to
\begin{equation}\label{eq:sub_channel_regimes_c5}
\begin{cases}\mathcal{C}_{51}=\{n_{d1}+n_{d3}\geq n_{d3}\geq n_{d2} \geq n_{d1},\:\: n_{d1}+n_{d3}\geq 2n_{d2}\}\\\mathcal{C}_{52}=\{2n_{d2}\geq n_{d1}+n_{d3}\geq n_{d3}\geq n_{d2} \geq n_{d1}\}\end{cases}
\end{equation} and 
\begin{equation}\label{eq:sub_channel_regimes_c6}
\begin{cases}\mathcal{C}_{61}=\{n_{d1}+n_{d2}\geq n_{d3}\geq n_{d1}\geq n_{d2}\}\\\mathcal{C}_{62}=\{n_{d3}\geq n_{d1}+n_{d2}\geq n_{d1}\geq n_{d2}\}\end{cases}.
\end{equation}
\vspace{.5em}


\begin{theorem}\label{th:1}
In the channel regimes $\mathbf{n}\in\{\mathcal{R}_i\}_{i=1}^{4}$, $\mathcal{R}_{51}$, $\mathcal{R}_{52}$ and $\mathcal{R}_{61}$ given by
\begin{equation}\label{eq:channel_regimes_th_1}
\begin{cases}\mathcal{R}_1\triangleq\mathcal{C}_1\cap\mathcal{I}_0\\\mathcal{R}_2\triangleq\mathcal{C}_2\cap\mathcal{I}_0\\
\mathcal{R}_3\triangleq\mathcal{C}_3\cap\mathcal{I}_0\\\mathcal{R}_4\triangleq\mathcal{C}_4\cap\mathcal{I}_1\\
\mathcal{R}_{51}\triangleq\mathcal{C}_{51}\cap\mathcal{I}_1\\
\mathcal{R}_{52}\triangleq\mathcal{C}_{52}\cap\mathcal{I}_1\\
\mathcal{R}_{61}\triangleq\mathcal{C}_{61}\cap\mathcal{I}_1\end{cases},
\end{equation} the optimal DTB of the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} at fronthaul capacities
\begin{enumerate}[label=(\alph*)]
\item $0\leq n_{F}\leq\max\{n_{d2},n_{d3}\}$
\item $n_{F}\geq\max\{n_{d2},n_{d3}\}$
\end{enumerate}
corresponds to 
\begin{enumerate}[label=(\alph*)]
\item \begin{equation}\label{eq:DTB_theorem_th_1_low_fronthaul}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\begin{cases}\frac{2-\mu}{\max\{n_{d2},n_{d3}\}}\qquad&\text{for }0\leq\mu\leq\mu^{\prime}(\mathbf{n})\\\frac{2-\mu^{\prime}(\mathbf{n})}{\max\{n_{d2},n_{d3}\}}\qquad&\text{for }\mu^{\prime}(\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation} 
\NoIndent{and}
\item \begin{equation}\label{eq:DTB_theorem_cloud_th_1_high_fronthaul}
\Delta_{\text{det}}^{*}(\mu,n_{F},\mathbf{n})=\begin{cases}\frac{2-\mu}{n_{F}}+\Big(1-\frac{\max\{n_{d2},n_{d3}\}}{n_{F}}\Big)\Delta_{\text{LB}}^{\prime}(\mathbf{n})&\text{for }0\leq\mu\leq\mu^{\prime}(\mathbf{n})\\\frac{2-\mu^{\prime}(\mathbf{n})}{\max\{n_{d2},n_{d3}\}}&\text{for }\mu^{\prime}(\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation}
\end{enumerate} respectively, where
\begin{equation}\label{eq:mu_prime}
\mu^{\prime}(\mathbf{n})=2-\max\{n_{d2},n_{d3}\}\Delta_{\text{LB}}^{\prime}(\mathbf{n})
\end{equation} and \begin{equation}\label{eq:dlb_main}  
\Delta_{\text{LB}}^{\prime}(\mathbf{n})=\max\Bigg\{\frac{1}{n_{d3}},\frac{1}{\max\{n_{d1},n_{d2}\}}, \frac{2}{\max\{n_{d1}+n_{d3},n_{d2}\}}\Bigg\}.
\end{equation}
\end{theorem}
\vspace{.5em}
\begin{theorem}\label{th:2}
In the channel regimes $\mathbf{n}\in\mathcal{R}_4^{\prime}$ and $\mathcal{R}_{61}^{\prime}$ given by
\begin{equation}\label{eq:channel_regimes_th_2}
\begin{cases}\mathcal{R}_4^{\prime}\triangleq\mathcal{C}_4\cap\mathcal{I}_1^{C}\\
\mathcal{R}_{61}^{\prime}\triangleq\mathcal{C}_{61}\cap\mathcal{I}_1^{C}\end{cases},
\end{equation} the optimal DTB of the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} at fronthaul capacities 
\begin{enumerate}[label=(\alph*)]
\item $0\leq n_{F}\leq n_{d2}$
\item $n_{d2}\leq n_{F}\leq n_{d3}$
\item $n_{F}\geq n_{d3}$
\end{enumerate} is given by
\begin{enumerate}[label=(\alph*)]
\item \begin{equation}\label{eq:DTB_theorem_cloud_th_2_low_fronthaul}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\begin{cases}\frac{1-\mu}{n_{d2}}\qquad&\text{for }0\leq\mu\leq\mu^{\prime\prime}(\mathbf{n})\\ \frac{2-\mu}{\max\{n_{d2},n_{d3}\}}\qquad&\text{for }\mu^{\prime\prime}(\mathbf{n})\leq\mu\leq\mu^{\prime}(\mathbf{n})\\\frac{2-\mu^{\prime}(\mathbf{n})}{\max\{n_{d2},n_{d3}\}}\qquad&\text{for }\mu^{\prime}(\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation} 
\item \begin{equation}\label{eq:DTB_theorem_cloud_th_2_medium_fronthaul}
\Delta_{\text{det}}^{*}(\mu,n_{F},\mathbf{n})=\begin{cases}\frac{1-\mu}{n_{F}}+\Big(1-\frac{n_{d2}}{n_{F}}\Big)\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})&\text{for }0\leq\mu\leq\mu^{\prime\prime}(\mathbf{n})\\\frac{2-\mu}{\max\{n_{d2},n_{d3}\}}&\text{for }\mu^{\prime\prime}(\mathbf{n})\leq\mu\leq \mu^{\prime}(\mathbf{n})\\\frac{2-\mu^{\prime}(\mathbf{n})}{\max\{n_{d2},n_{d3}\}}&\text{for }\mu^{\prime}(\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation}
\NoIndent{and}
\item Equation \eqref{eq:DTB_theorem_cloud_th_1_high_fronthaul}, 
\end{enumerate} respectively. $\mathbf{\mu}^{\prime}(\mathbf{n})$ and $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ are defined in \eqref{eq:mu_prime} and \eqref{eq:dlb_main}. The other parameters in \eqref{eq:DTB_theorem_cloud_th_2_low_fronthaul}--\eqref{eq:DTB_theorem_cloud_th_2_medium_fronthaul} are as follows: \begin{equation}\label{eq:mu_prime_prime}
\mu^{\prime\prime}(\mathbf{n})=\frac{n_{d3}-2n_{d2}}{n_{d3}-n_{d2}},
\end{equation} and
\begin{equation}\label{eq:dlb_main_prime_prime}  
  \Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})=\max\Bigg\{\frac{1}{n_{d3}-n_{d2}},\Delta_{\text{LB}}^{\prime}(\mathbf{n})\Bigg\}.
\end{equation}
\end{theorem}
\vspace{.5em}
\begin{theorem}\label{th:3}
In the channel regime $\mathbf{n}\in\mathcal{R}_{62}^{\prime}$ given by 
\begin{equation}\label{eq:channel_regimes_th_3}
\mathcal{R}_{62}^{\prime}\triangleq\mathcal{C}_{62}\cap\mathcal{I}_1^{C},
\end{equation} the optimal DTB of the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} at fronthaul capacities
\begin{enumerate}[label=(\alph*)]
\item $0\leq n_{F}\leq n_{d2}$
\item $n_{F}\geq n_{d2}$
\end{enumerate} corresponds to
\begin{enumerate}[label=(\alph*)]
\item \begin{equation}\label{eq:DTB_theorem_cloud_th_3_low_fronthaul}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\begin{cases}\frac{1-\mu}{n_{d2}}\qquad&\text{for }0\leq\mu\leq\mu^{\prime\prime\prime}(\mathbf{n})\\\frac{1-\mu^{\prime\prime\prime}(\mathbf{n})}{n_{d2}}\qquad&\text{for }\mu^{\prime\prime\prime}(\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation}
\NoIndent{and}
\item \begin{equation}\label{eq:DTB_theorem_cloud_th_3_high_fronthaul}
\Delta_{\text{det}}^{*}(\mu,n_{F},\mathbf{n})=\begin{cases}\frac{1-\mu}{n_{F}}+\Big(1-\frac{n_{d2}}{n_{F}}\Big)\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})&\text{for }0\leq\mu\leq\mu^{\prime\prime\prime}(\mathbf{n})\\\frac{1-\mu^{\prime\prime\prime}(\mathbf{n})}{n_{d2}}&\text{for }\mu^{\prime\prime\prime}(\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation}
\end{enumerate} respectively, where $\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})$ is given in \eqref{eq:dlb_main_prime_prime} and $\mu^{\prime\prime\prime}(\mathbf{n})$ is   \begin{equation}\label{eq:mu_prime_prime_prime}
\mu^{\prime\prime\prime}(\mathbf{n})=\frac{n_{d1}-n_{d2}}{n_{d1}}.
\end{equation}
\end{theorem}
\begin{theorem}[Constant DTB]\label{th:4}
In the channel regimes \begin{equation}\label{eq:channel_regimes_th_4}
\begin{cases}\mathcal{R}_2^{\prime}\triangleq\mathcal{C}_2\cap\mathcal{I}_0^{C}\\
\mathcal{R}_3^{\prime}\triangleq\mathcal{C}_3\cap\mathcal{I}_0^{C}\\
\mathcal{R}_{51}^{\prime}\triangleq\mathcal{C}_{51}\cap\mathcal{I}_1^{C}\\
\mathcal{C}_7\end{cases}, \end{equation}
the optimal DTB of the cloud and cache-aided HetNet for any $n_{F}\geq 0$ does not depend on the fractional cache size $\mu$ and remains constant. It corresponds to \begin{equation}\label{eq:DTB_theorem_cloud_th_3_cache_ineff}
\Delta_{\text{det}}(\mu,n_F,\mathbf{n})=\Delta_0(\mathbf{n}),
\end{equation} where $\Delta_0(\mathbf{n})$ is defined in \eqref{eq:DTB_lemma}.
%\noindent \begin{IEEEproof} (Theorem \ref{th:1}--\ref{th:4}) Lower (converse) and upper bounds (achievability) on the DTB are derived for the case of active and inactive ($n_{F}=0$) fronthaul links. Lower bound on the DTB are provided in sub-sections \ref{subsec:ser_low_bound} and \ref{subsec:ser_low_bound_nF_greater_0} while upper bounds can be found in sub-sections \ref{subsec:ser_upp_bound} and \ref{subsec:ser_upp_bound_nF_greater_0}. 
%\end{IEEEproof}
% Remarks

\begin{figure*}
        \centering
        \begin{subfigure}[b]{0.475\textwidth}
            \centering
            \begin{tikzpicture}[scale=1]
            \Resulttwo
            \end{tikzpicture}
            \caption{{\small $\mathbf{n}\in\{\mathcal{R}_i\}_{i=1}^{4},\mathcal{R}_{51},\mathcal{R}_{52}$ and $\mathcal{R}_{61}$}}    
            \label{fig:th_1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}  
            \centering 
            \begin{tikzpicture}[scale=1]
            \Resultthree
            \end{tikzpicture}
            \caption{{\small $\mathbf{n}\in\mathcal{R}_{4}^{\prime}$ and $\mathcal{R}_{61}^{\prime}$}}     
            \label{fig:th_2}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \begin{tikzpicture}[scale=1]
            \Resultfour
            \end{tikzpicture}
            \caption{{\small $\mathbf{n}\in\mathcal{R}_{62}^{\prime}$}}    
            \label{fig:th_3}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \begin{tikzpicture}[scale=1]
            \Resultfive
            \end{tikzpicture}
            \caption{{\small $\mathbf{n}\in\mathcal{R}_{2}^{\prime},\mathcal{R}_{3}^{\prime},\mathcal{R}_{51}^{\prime}$ and $\mathcal{C}_{7}$}}  
            \label{fig:th_4}
        \end{subfigure}
        \caption[DTB as a function of $\mu$ for various channel regimes and distinct fronthaul capacities]
        {\small DTB as a function of $\mu$ for various channel regimes and distinct fronthaul capacities} 
        \label{fig:results}
\end{figure*}
\vspace{.5em}
\begin{remark}[Decreasing DTB Monotonicity in $\mu$]
In all channel regimes specified in Equations \eqref{eq:channel_regimes_th_1}, \eqref{eq:channel_regimes_th_2} and \eqref{eq:channel_regimes_th_3}, edge caching and fronthauling decrease the latency with increasing fractional cache size (cf. Fig. \ref{fig:th_1}--\ref{fig:th_3}). At the threshold cache size $\mu_{\text{th}}(\mathbf{n})$ (e.g. in channel regimes \eqref{eq:channel_regimes_th_1} and \eqref{eq:channel_regimes_th_2} $\mu_{\text{th}}(\mathbf{n})=\mu^{\prime}(\mathbf{n})$), the lowest overall latency corresponds to the optimal \emph{wireless} latency\footnote{For instance in $\mathcal{R}_2$, caching more than a fraction $\mu^{\prime}(\mathbf{n})=\nicefrac{(2n_{d3}-n_{d2})}{n_{d3}}$ of any file will not lead to any improvement of the optimal DTB of $\nicefrac{1}{n_{d3}}$. This is because in this case the wireless link from eNB to $U_2$ functions as a bottleneck.}. Or in other words, at this cache size prefetched information at the HeNB is just enough so that the requested files are transmitted directly over the wireless channel from eNB/HeNB to the users without requiring any fronthauling transmissions ($T_{F}=0$). This observation is independent of the fronthaul capacity. 
%fronthauling, irrespective of its capacity, is unneeded ($T_{F}=0$) and only wireless transmissions from eNB/HeNB to the users. 
When operating at any fractional cache size \emph{below} $\mu_{\text{th}}(\mathbf{n})$, however,  
% in the range $\mu\in[0,\mu_{\text{th}}(\mathbf{n})[$, 
edge caching along with fronthauling reduces the latency further than a system without cloud processing ($n_{F}=0$) either partially or entirely over the cache size range $\Big[0,\mu_{\text{th}}(\mathbf{n})\Big)$ as a function of the fronthaul capacity. For instance, in channel regimes \eqref{eq:channel_regimes_th_2} (cf. Fig \ref{fig:th_2}), optimal cloud-and cache-based schemes with fronthaul links
\begin{enumerate}[label=(\Alph*)]
% \item in the \emph{low-fronthaul capacity} range $[0,n_{d2}]$
%\item in the \emph{medium-fronthaul capacity} range $[n_{d2},n_{d3}]$
\item in the \emph{medium-fronthaul capacity} range $(n_{d2},\max\{n_{d2},n_{d3}\}]$
%\item and in the \emph{high-fronthaul capacity} range $[n_{d3},\infty)$
\item and in the \emph{high-fronthaul capacity} range $(\max\{n_{d2},n_{d3}\},\infty)$
\end{enumerate} strictly outperform cache-only schemes 
\begin{enumerate}[label=(\Alph*)]
\item partially in the sub-interval $\Big[0,\mu^{\prime\prime}(\mathbf{n})\Big)$ of $\Big[0,\mu^{\prime}(\mathbf{n})\Big)$
\item and entirely over the interval $\Big[0,\mu^{\prime}(\mathbf{n})\Big)$.
\end{enumerate} As one would expect intuitively, we observe that for any fronthaul capacity the extent to which fronthauling (in addition to edge caching) reduces the latency to a system without cloud capabilities decays with increasing cache size.  
\end{remark}
\vspace{.5em}
\begin{remark}[Constant DTB]
In all channel regimes of \eqref{eq:channel_regimes_th_4}, edge caching and/or fronthauling is not beneficial. This means that neither a large HeNB cache nor high-fronthaul capacities from cloud to the HeNB can lead to any latency improvement in comparison to the case for $(\mu=0,n_F=0)$. Consequently, only the eNB is involved in the transmission while the HeNB remains silent. As a result, the optimal latency corresponds to the optimal DTB given in Lemma \ref{lemma:2} for the broadcast channel. 
% for the channel at fractional cache size $\mu=0$.   
\end{remark}
\vspace{.5em}
\begin{remark}[Regimes $\mathcal{C}_4$ and $\mathcal{C}_{61}$] For $n_F\leq n_{d3}$, the DTB performance in $\mathcal{R}_{4}$ and $\mathcal{R}_{4}^{\prime}$ 
% as well as $\mathcal{R}_{61}$ and $\mathcal{R}_{61}^{\prime}$ 
are in general not identical. This arises from performance differences at fractional cache size $\mu=0$ for complementary broadcast conditions $\mathcal{I}_1$ and $\mathcal{I}_1^{C}$ (see Remark \ref{remark_bc_conditions}). 
For $n_{F}\geq n_{d3}$ these conditions become irrelevant and the optimal DTB of channel regimes $\mathcal{R}_{4}$ and $\mathcal{R}_{4}^{\prime}$ 
% as well as $\mathcal{R}_{61}$ and $\mathcal{R}_{61}^{\prime}$, 
collapses to the same expression. Thus, Equation \eqref{eq:DTB_theorem_cloud_th_1_high_fronthaul} actually holds for the union $\mathcal{C}_4=\mathcal{R}_{4}\cup \mathcal{R}_{4}^{\prime}$. The same behavior applies for $\mathcal{R}_{61}$ and $\mathcal{R}_{61}^{\prime}$ as well. These observations are illustrated in Fig. \ref{fig:th_1} and \ref{fig:th_2}.  
\end{remark}
\vspace{.5em}
\begin{remark}[Threshold Fronthaul Capacity $n_{F,\text{th}}$]
We see from Theorem \ref{th:1}--\ref{th:3} that for low fronthaul capacities below a threshold $n_{F,\text{th}}$ (e.g. $n_{F,\text{th}}=n_{d2}$ for channel regimes specified in \eqref{eq:channel_regimes_th_2}), cache-only schemes remain optimal. We term the range $[0,n_{F,\text{th}}]$ as \emph{low-fronthaul capacity} regime. 
\end{remark}
\vspace{0.5em}
In the remainder of this section, we develop lower (cf. \ref{subsec:ser_low_bound} and \ref{subsec:ser_low_bound_nF_greater_0}) and upper bounds (see \ref{subsec:ser_upp_bound} and \ref{subsec:ser_upp_bound_nF_greater_0}) on the DTB for the cases of active and inactive fronthaul links. We put the emphasis on the upper bounds. In the respective sub-sections, we introduce transmission schemes which achieve the optimal DTB provided in Theorem \ref{th:1}--\ref{th:4} (cf. Fig. \ref{fig:results}). To this end, various schemes are proposed to cover different operating channel regimes of the network under study. Initially, we will focus on the cache-only ($n_F=0$) case. This will turn to be useful when considering the achievability in the setting with non-zero fronthaul capacity links ($n_F\geq 0$) in sub-section \ref{subsec:ser_upp_bound_nF_greater_0}. Due to the convexity of the DTB (cf. Lemma \ref{lemma:1}), we establish the achievability of corner points in the latency-memory tradeoff curves. In Fig. \ref{fig:results}, depending on the operating channel regime, these corner points are denoted by \circled{$I_r$}, % $r\in\{a,b,c,d,e\}$, 
$r\in\{a,b,c,d\}$, \circled{$II_s$}, $s\in\{a,b\}$, and \circled{$III$}. In this regard, we will show that corner points 
\begin{itemize}
\item \circled{$I_a$}, \circled{$II_a$}, \circled{$II_b$} and \circled{$III$} involve only edge caching and do not require any fronthaul transmission ($n_{F}=0$); thus, representing cache-only transmission policies, whereas
\item \circled{$I_r$}, $r\in\{b,c,d\}$, involve only fronthauling and do not require edge caching ($\mu=0$); thus, representing cloud-only transmission policies. 
\end{itemize} Generally speaking, the DTB at fractional cache size $\mu$ which lies between two neighboring corner points (say \circled{A} and \circled{B}) cache sizes' is achieved through file splitting and time sharing between the policies at corner point \circled{A} and \circled{B}. This strategy is only operational at a channel regime under which the transmission policy at \circled{A}, $\mathcal{R}_{\circled{A}}$, and the transmission policy at \circled{B}, $\mathcal{R}_{\circled{B}}$ are \emph{both} feasible. This is given by the \emph{non-empty} set $\mathcal{R}_{\circled{A}}\cap\mathcal{R}_{\circled{B}}$. 

%But before we describe the schemes in detail, we suggest a general building block structure that all schemes have in common. This block structure is applicable to cache-only schemes ($n_{F}=0$). 
%But before we describe the scheme in detail, we describe the main building blocks.

\subsection{Lower Bound (Converse) on the Minimum DTB for $n_{F}=0$}
\label{subsec:ser_low_bound}

\begin{proposition}[Lower Bound on the Minimum DTB on Cache-Only F-RAN]\label{prop:1}
For the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} with $n_F=0$, the optimal DTB $\Delta_{\text{det}}^{*}(\mu,\mathbf{n})$ is lower bounded as
\begin{equation}
\label{eq:ser_lb_cache_only}
\Delta_{\text{det}}^{*}(\mu,\mathbf{n})\geq\Delta_{\text{LB}}(\mu,\mathbf{n}),
\end{equation}
where \begin{equation}
\label{eq:lb_cache_only}
\Delta_{\text{LB}}(\mu,\mathbf{n})=\max\Bigg\{\frac{1}{n_{d3}},\frac{1}{\max\{n_{d1},n_{d2}\}}, \frac{2}{\max\{n_{d1}+n_{d3},n_{d2}\}},\frac{1-\mu}{n_{d2}},\frac{2-\mu}{\max\{n_{d2},n_{d3}\}}\Bigg\}.
\end{equation}
\end{proposition}
\noindent\begin{IEEEproof}
The proof of Proposition \ref{prop:1} is presented in Appendix \ref{app:lw_bound_ser}.   
\end{IEEEproof}

\subsection{Upper Bound (Achievability) on the Minimum DTB for $n_{F}=0$}
\label{subsec:ser_upp_bound}

In this sub-section, we propose schemes to cover different operating channel regimes of the network under study for the cache-only ($n_F=0$) case. As previously explained, we will only focus on the achievability at corner points \circled{$I_a$}, \circled{$II_a$}, \circled{$II_b$} and \circled{$III$}. Remaining intermediate points in the tradeoff curves on the DTB follow from the argument of convexity (cf. Lemma \ref{lemma:1}). But before we describe the schemes in detail, we suggest a general building block structure that all schemes have in common. This block structure is applicable to cache-only schemes ($n_{F}=0$). 
%But before we describe the scheme in detail, we describe the main building blocks.

\subsubsection*{Building Blocks}
Due to the partial wireless connectivity of the network under study, in which only the eNB is connected to both users while the HeNB is only connected to $U_1$, we propose that the eNB sends
% \begin{enumerate}
\begin{itemize}
\item \underline{p}rivate information
\begin{itemize}
\item[--]  $\mathbf{u}_{1,p}[t]$ and $\mathbf{u}_{2,p}[t]$ intended for $U_1$
\item $\mathbf{v}_{p}[t]$ intended for $U_2$
\end{itemize}
\end{itemize}
while the HeNB transmits
\begin{itemize}
\item\underline{p}rivate information $\mathbf{u}_{3,p}[t]$
\item and XORed information $\mathbf{w}_{\text{IN}}[t]$ for \underline{i}nterference \underline{n}eutralization
\end{itemize} 
(in the $t-$th channel use ($t=1,\ldots, T_{E}$)) (cf. Fig. \ref{fig:ldm_stack}). 
\begin{figure}[t]
\begin{center}
		\LDMstack
	\caption{Transmitted Signal Vector Structure at $t-$th Channel Use of length $q=\max\{n_{d1},n_{d2},n_{d3}\}$ at (H)eNB}	
	\label{fig:ldm_stack}
	\end{center}
\end{figure}
In all schemes $\mathbf{w}_{\text{IN}}[t]$ is introduced, in such a way that the interference caused by private information $\mathbf{v}_{p}[t]$ is partially, or even completely, neutralized at $U_1$. Depending on the particular channel regime, certain signal levels are zero-padded to either avoid collision of private information at $U_1$ or to reduce the transmission power level of the HeNB. In the block representation illustrated in Fig. \ref{fig:ldm_stack} this is captured by null vectors $\mathbf{0}_{l}$ of length $l=l_1,l_2,l_3,l_4$. In the sequel, we focus on transmission schemes that utilize a single channel use ($T_{E}=1$). Thus, we drop the time dependency in our notation. We denote the length of signal vectors $\mathbf{u}_{i,p}$, $i=1,\ldots,3$, $\mathbf{v}_{p}$ and $\mathbf{w}_{\text{IN}}$ by $R^{u}_{i,p}$, $R^{v}_{p}$ and $R^{w}_{\text{IN}}$, respectively.  

The transmission according to the block structure of Fig. \ref{fig:ldm_stack} requires that at the respective receivers interference-decoding and treating interference as noise (TIN) is applied successively such that the achievable rates of $U_1$ and $U_2$ for $T_{E}=1$ become
\begin{subequations}
\begin{alignat}{2}
R_{U_1}&=R_{\text{IN}}^{w}+\sum_{i=1}^{3}R^{u}_{i,p},\label{eq:ach_rate_U1}\\
R_{U_2}&=R^{v}_{p},\label{eq:ach_rate_U2}
\end{alignat}   
\end{subequations} respectively. The proposed scheme forces the fractional cache size to be \begin{equation}
\label{eq:frac_cache_size}
\mu^{\prime}_{\text{Ach}}(\mathbf{n})=\frac{R_{3,p}^{u}+R_{\text{IN}}^{w}}{R_{U_2}}.
\end{equation} The design parameters of our scheme are the rate allocation parameters $R_{i,p}^{u},R_{p}^{v},R_{\text{IN}}^{w}$ and the respective null vectors. 
%For all channel regimes at given fractional cache size $\mu\in[0,1]$, we carefully choose the rate allocation parameters $R_{i,p}^{u},R_{p}^{v},R_{\text{IN}}^{w}$ and the respective null vectors 
We carefully choose these non-negative design variables such that the achievable per-user rates are identical, i.e.,
\begin{equation}
\label{eq:user_rate_1_and_2}
R_{U_1}\stackrel{!}{=}R_{U_2}\triangleq R_{U}
\end{equation} and as large as possible while simultaenously equating the achievable fractional cache size with the given cache size $\mu$, i.e., \begin{equation}
\label{eq:cache_size_req}
\mu^{\prime}_{\text{Ach}}(\mathbf{n})\stackrel{!}{=}\mu.
\end{equation}
Through the design criterion \eqref{eq:user_rate_1_and_2}, the transmission strategy would not favor any user; hence, making the completion time, thus the latency, for delivering the requested files identical to both users. We follow that each user can reliably decode $R_{U}$ bits per channel use, or in other words, $\Delta_{\text{det}}(\mu=\mu^{\prime}_{\text{Ach}},n_F=0,\mathbf{n})=\nicefrac{1}{R_U}$ channel uses are required to provide each user with one bit. To exemplify our scheme, we show the achievability for a specific channel setting. 
\begin{figure*}[t!]
\centering
\LDMblockone
\caption{Example of proposed scheme for channel regime $\mathcal{R}_1$ with $n_{d1}=2$, $n_{d2}=5$ and $n_{d3}=4$. The cached content of the HeNB on the requested files $W_{d_1}$ and $W_{d_2}$ are $S_{d_1}=(a_2)$ and $S_{d_2}=(b_3)$. This corresponds to a fractional cache size of $\mu^{\prime}(\mathbf{n})=\nicefrac{1}{3}$.}
\label{fig:AcScheme}
\end{figure*} 

\begin{example}[Regime $\mathcal{R}_1$]\label{example_1}
In this example, we consider the channel $\mathbf{n}=(2,5,4)^{T}\in\mathcal{R}_1$ for $n_{F}=0$. Theorem \ref{th:1} gives us the corner points \circled{$I_a$}$\:=\Big(\mu=0,\Delta_{\text{det}}^{*}(\mu=0,n_{F}=0,\mathbf{n})=\nicefrac{2}{5}\Big)$ and \circled{$II_b$}$\:=\Big(\mu^{\prime}=\nicefrac{1}{3},\Delta_{\text{det}}^{*}(\mu=\nicefrac{1}{3},n_{F}=0,\mathbf{n})=\nicefrac{1}{3}\Big)$.

At extreme point \circled{$I_a$} neither fronthauling nor edge caching involving the HeNB is performed. Thus, the F-RAN under study reduces to a broadcast channel in which the eNB is responsible for transmitting the requested files while the HeNB remains silent. Thus, the only relevant channel realizations are $n_{d2}=5$ and $n_{d3}=4$. We observe that the stronger of those two channels is $n_{d2}=5$ ($n_{d3}\leq n_{d2}$). The optimal scheme equally distributes the transmission load of $n_{d2}=5$ bits to both users. That is, by sending $\nicefrac{n_{d2}}{2}=\nicefrac{5}{2}$ private information bits in a single channel use; or, alternatively by sending one bit in $\Delta_{\text{det}}^{*}(\mu=0,n_{F}=0,\mathbf{n})=\nicefrac{2}{5}$ channel uses, to $U_1$ and $U_2$, respectively. This scheme is feasible since the weaker channel $n_{d3}$ supports the transmission of $\nicefrac{n_{d2}}{2}$ bits ($\nicefrac{n_{d2}}{2}\leq n_{d3}$). These conditions are equivalent with $\mathbf{n}\in\mathcal{I}_0$. In summary, in the block representation this scheme is given by fixing the rate allocation parameters to $R_{2,p}^{u}=R_{p}^{v}=\nicefrac{n_{d2}}{2}=\nicefrac{5}{2}$, $l_2=n_{d2}=5$ and $R_{1,p}^{u}=R_{3,p}^{u}=R_{\text{IN}}^{w}=l_1=l_3=l_4=0$. We refer to the proof of Lemma \ref{lemma:2} and Remark \ref{remark_bc_conditions} for further details on this scheme.  

The extreme point \circled{$II_b$} is achievable through cache-only transmission schemes in channel regimes $\mathbf{n}\in\mathcal{C}_1\supseteq\mathcal{R}_1$. It requires one channel use and achieves a DTB of $\nicefrac{2}{(n_{d1}+n_{d3})}=\nicefrac{1}{3}$ at fractional cache size $\mu^{\prime}(\mathbf{n})=\nicefrac{(2n_{d1}+2n_{d3}-2n_{d2})}{(n_{d1}+n_{d3})}=\nicefrac{1}{3}$. Fig. \ref{fig:AcScheme} illustrates the scheme for the case when $U_1$ and $U_2$ request $W_{d_1}=(a_1,a_2,a_3)$ and $W_{d_2}=(b_1,b_2,b_3)$, respectively. In this case where the channel of the cross link $n_{d2}$ is the strongest, it is advantageous that the eNB transmits not only private information to $U_2$ but also to $U_1$. This implies that the rates $R_{1,p}^{u}, R_{2,p}^{u}$ are chosen to be non-zero whereas $l_1=0$. From the perspective of $U_2$, the optimal DTB of $\nicefrac{1}{3}$ is then only achievable if we fix $R_{p}^{v}=\nicefrac{(n_{d1}+n_{d3})}{2}=3$ in order to convey bits $b_1,b_2$ and $b_3$. Note that the eNB-$U_2$ link is capable of reliably carrying $R_{p}^{v}=3$ bits to $U_2$ because $R_{p}^{v}=3<n_{d3}=4$ holds in $\mathcal{C}_1$. The unused signal levels at the eNB of rate $R_{1,p}^{u}=\nicefrac{(n_{d3}-n_{d1})}{2}=1$ and $R_{2,p}^{u}=n_{d2}-n_{d3}=1$ are allocated to send private information $a_1$ and $a_3$ to $U_1$.  To retrieve the remaining desired bit of $U_1$ ($a_2$), the interfering bit $b_3$ of $\mathbf{v}_{p}$ is neutralized by sending the single XOR combination ($R_{\text{IN}}^{w}=n_{d1}+n_{d3}-n_{d2}=1$) $a_2\oplus b_3$ at the \emph{highest} signal level of the HeNB. Therefore, the HeNB retains $a_2$ and $b_3$ in its cache during the placement phase. This constitutes a fractional cache size $\mu^{\prime}(\mathbf{n})=\nicefrac{1}{3}$. With this strategy, $U_1$ receives $R_{1,p}^{u}+R_{2,p}^{u}=\nicefrac{(2n_{d2}-n_{d1}-n_{d3})}{2}=2$ bits ($a_1$ and $a_3$) of $W_{d_1}$ from the eNB while the remaining $R_{\text{IN}}^{w}=n_{d1}+n_{d3}-n_{d2}=1$ bits ($a_2$) are received through network coding which involves both HeNB and eNB. Sending additional private information from the HeNB would not increase the achievable rate of $U_2$ any further. For that reason, $R_{3,p}^{u}=l_3=0$ and $l_2=4$. When generalizing the scheme, it is easy to see that the scheme is feasible for arbitrary $\mathbf{n}\in\mathcal{C}_1$. If the achievable per-user rate is a non-integer, two channel uses are required. For further details on this case, we point to our previous work \cite{prev_work}.    

Any point between the two corner points \circled{$I_a$} and \circled{$II_b$} is achieved through file splitting and time sharing between the policies at those two corner points. Such scheme is often termed \emph{memory sharing}. As the transmission at \circled{$I_a$} and \circled{$II_b$} are feasible in $\mathcal{R}_{\text{\circled{$I_a$}}}=\mathcal{I}_0$ and $\mathcal{R}_{\text{\circled{$II_b$}}}=\mathcal{C}_1$, any intermediate point in the memory-latency tradeoff curve is achievable through memory sharing in the channel regime $\mathcal{R}_{1}\triangleq\mathcal{R}_{\text{\circled{$II_b$}}}
\cap\mathcal{R}_{\text{\circled{$I_a$}}}=\mathcal{C}_1\cap\mathcal{I}_0$. In this particular channel regime, we notice that $\mathcal{R}_{1}=\mathcal{C}_1$ because $\mathcal{C}_1\cap\mathcal{I}_0^{C}=\emptyset$. However, this is not true for all channel regimes under study.  
\end{example}
\vspace{0.5em}
In the remainder of sub-section \ref{subsec:ser_upp_bound}, we will show the achievability of all relevant corner points that are based on cache-only transmission policies ($n_{F}=0$). To this end, we specify the rate allocation parameters introduced as part of the generalized block structure (see Fig. \ref{fig:ldm_stack}).
\vspace{0.5em}    
\subsubsection*{Scheme for Corner Point \circled{$I_a$}}
The achievability at this point follows from Lemma \ref{lemma:2} and \eqref{eq:DTB_lemma} (cf. Example \ref{example_1}). At this point, the optimal DTB corresponds to
%\begin{equation} \label{eq:opt_DTB_I_a}\begin{subnumcases}{n=}
%\Delta_0(\mathbf{n})=\begin{cases}\frac{2}{n_{d2}}\text{ for }\mathbf{n}\in\mathcal{I}_0\\\frac{1}{n_{d3}}\text{ for }\mathbf{n}\in\mathcal{I}_0^{C}\\\frac{2}{n_{d3}}\text{ for }\mathbf{n}\in\mathcal{I}_1\\\frac{1}{n_{d2}}\text{ for }\mathbf{n}\in\mathcal{I}_1^{C}\end{cases}.\ed{numcases}
%\end{equation}
%\begin{equation} \label{eq:opt_DTB_I_a}
\begin{subnumcases}{\Delta_0(\mathbf{n})=}
\frac{2}{n_{d2}}\text{ for }\mathbf{n}\in\mathcal{I}_0\\\frac{1}{n_{d3}}\text{ for }\mathbf{n}\in\mathcal{I}_0^{C}\\\frac{2}{n_{d3}}\text{ for }\mathbf{n}\in\mathcal{I}_1\\\frac{1}{n_{d2}}\text{ for }\mathbf{n}\in\mathcal{I}_1^{C}.\end{subnumcases}
%\end{equation}
This is achieved by setting the rate allocation parameters to $l_2=\max\{n_{d1},n_{d2},n_{d3}\}$, $R_{p}^{v}=\nicefrac{1}{\Delta_0(\mathbf{n})}$, $l_1=l_2-\nicefrac{2}{\Delta_0(\mathbf{n})}$, 
\begin{equation}\label{eq:R_1_p_R_2_p_u}
(R_{1,p}^{u},R_{2,p}^{u})^{T}=\begin{cases}(\nicefrac{1}{\Delta_0(\mathbf{n})},0)\text{ for } n_{d2}\geq n_{d3}\\(0,\nicefrac{1}{\Delta_0(\mathbf{n})})\text{ for } n_{d2}\leq n_{d3}\end{cases},
\end{equation}
and the remaining variables to $0$. We observe that the achievable DTB is in accordance with Theorem \ref{th:1}--\ref{th:4} for $\mu=0$. 

\subsubsection*{Scheme for Corner Point \circled{$II_b$}}

% Control
\newcolumntype{C}{>{\centering\arraybackslash}p{4.0em}}
\begin{table}[t]
%\centering
\caption{Rate allocation parameters for corner point \protect\circled{$II_b$} at fractional cache size $\mu^{\prime}(\mathbf{n})$}
\label{tab:rate_alloc_param}
\begin{tabular}{|c||c|C|C|c|c|c|c|}
\hline
Regime & $\mathcal{C}_1$ & $\mathcal{R}_2$ & $\mathcal{R}_3$ & $\mathcal{C}_4$ & $\mathcal{R}_{51}$ & $\mathcal{C}_{52}$ & $\mathcal{C}_{61}$ 
\\ \hline 
$R_{3,p}^{u}$ & $0$ & \multicolumn{2}{c|}{$0$} & $n_{d3}-n_{d2}$ & $0$ & $0$ & $n_{d1}-n_{d2}$
\\ \hline
$R_{2,p}^{u}$ & $\frac{n_{d3}-n_{d1}}{2}$ &  \multicolumn{2}{c|}{$0$} & $0$ & $n_{d3}-n_{d2}$ & $\frac{n_{d3}-n_{d1}}{2}$ & $n_{d3}-n_{d1}$  
\\ \hline
$R_{1,p}^{u}$ & $n_{d2}-n_{d3}$ &  \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $0$ & $0$ & $0$ 
\\ \hline
$R_{\text{IN}}^{w}$  & $n_{d1}+n_{d3}-n_{d2}$ & \multicolumn{2}{c|}{$2n_{d3}-n_{d2}$} & $n_{d2}$ & $2n_{d2}-n_{d3}$ & $n_{d1}$ & $n_{d1}+n_{d2}-n_{d3}$
\\ \hline
$R_{p}^{v}$  & $\frac{n_{d1}+n_{d3}}{2}$ & \multicolumn{2}{c|}{$n_{d3}$} & $n_{d3}$ & $n_{d2}$ & $\frac{n_{d1}+n_{d3}}{2}$ & $n_{d1}$ 
\\ \hline
$l_4$ & \multicolumn{3}{c|}{$0$} & $n_{d1}-n_{d3}$ & \multicolumn{3}{c|}{$0$}
\\ \hline
$l_3$ & $0$ & $n_{d2}-n_{d3}$ & $n_{d1}-n_{d3}$ & $0$ & $n_{d1}+n_{d3}-2n_{d2}$ & $0$ & $n_{d3}-n_{d1}$  
\\ \hline
$l_2$ & $2n_{d2}-n_{d1}-n_{d3}$ & \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d1}$
\\ \hline
$l_1$ & $0$ & $0$ & $n_{d1}-n_{d2}$ & $n_{d1}-n_{d3}$ & $0$ & $0$ & $0$ 
\\ \hline
\end{tabular}
\end{table}

The encoding at the transmitters, both eNB and HeNB, follows along the block building structure of Fig. \ref{fig:ldm_stack}. Similarly to Example \ref{example_1}, the length of each signal vector is appropriately determined to individually account for all channel regimes while maximizing the \emph{symmetric} per-use rate. This has the effect that the latency of providing each user with its requested file are the same. All the proposed schemes require $T_{E}=1$ channel use to perform optimally. Table \ref{tab:rate_alloc_param} indicates the rate allocation parameters and the \emph{largest} channel regime set under which \eqref{eq:user_rate_1_and_2} and \eqref{eq:cache_size_req} are both satisfied. Note that the achievable DTB and $\mu^{\prime}_{\text{Ach}}$ (specified in \eqref{eq:frac_cache_size}) match \eqref{eq:DTB_theorem_th_1_low_fronthaul}, \eqref{eq:DTB_theorem_cloud_th_2_low_fronthaul} and \eqref{eq:mu_prime}, respectively.
\vspace{0.5em}
\subsubsection*{Scheme for Corner Points \circled{$II_a$} and \circled{$III$}} 

% Control
\newcolumntype{C}{>{\centering\arraybackslash}p{6.0em}}
\begin{table}[h]
\centering
\setlength\tabcolsep{4pt}
\begin{minipage}{0.48\textwidth}
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$II_a$} at fractional cache size $\mu^{\prime\prime}(\mathbf{n})$}
\begin{tabular}{|c||C|C|}
\hline
Regime & $\mathcal{R}_{4}^{\prime}$ & $\mathcal{R}_{61}^{\prime}$ \\ \hline 
$R_{3,p}^{u}$ & \multicolumn{2}{c|}{$n_{d3}-2n_{d2}$} \\ \hline
$R_{2,p}^{u}$ & \multicolumn{2}{c|}{$n_{d2}$} \\ \hline
$R_{1,p}^{u}$ & \multicolumn{2}{c|}{$0$} \\ \hline
$R_{\text{IN}}^{w}$  & \multicolumn{2}{c|}{$0$} \\ \hline
$R_{p}^{v}$  & \multicolumn{2}{c|}{$n_{d3}-n_{d2}$} \\ \hline
$l_4$ & \multicolumn{2}{c|}{$n_{d1}+n_{d2}-n_{d3}$} \\ \hline
$l_3$ & $n_{d2}$ & $n_{d2}+n_{d3}-n_{d1}$ \\ \hline
$l_2$ & \multicolumn{2}{c|}{$0$} \\ \hline
$l_1$ & $n_{d1}-n_{d3}$ & $0$ \\ \hline
\end{tabular}
\label{tab:rate_alloc_II_a} 
\end{minipage}%
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$III$} at fractional cache size $\mu^{\prime\prime\prime}(\mathbf{n})$} 
\begin{tabular}{|c||c|}
\hline
Regime & $\mathcal{C}_{62}$ \\ \hline 
$R_{3,p}^{u}$ & $n_{d1}-n_{d2}$ \\ \hline
$R_{2,p}^{u}$ & $n_{d2}$ \\ \hline
$R_{1,p}^{u}$ & $0$ \\ \hline
$R_{\text{IN}}^{w}$  & $0$ \\ \hline
$R_{p}^{v}$  & $n_{d1}$ \\ \hline
$l_4$ & $0$ \\ \hline
$l_3$ & $0$ \\ \hline
$l_2$ & $n_{d2}+n_{d3}-n_{d1}$ \\ \hline
$l_1$ & $n_{d3}-n_{d1}-n_{d2}$ \\ \hline
\end{tabular}
\label{tab:rate_alloc_III} 
\end{minipage}
\end{table}

For these two corner points, we adopt the general block structure of Fig. \ref{fig:ldm_stack}. Tables \ref{tab:rate_alloc_II_a} and \ref{tab:rate_alloc_III} outline the rate allocation parameters for both extreme points.    


\subsection{Lower Bound (Converse) on the Minimum DTB for $n_{F}\geq 0$}
\label{subsec:ser_low_bound_nF_greater_0}

\begin{proposition}[Lower Bound on the Minimum DTB]\label{prop:2}
For the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} with $n_F\geq 0$, the optimal DTB $\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})$ is lower bounded as
\begin{equation}
\label{eq:ser_lb_cache_only_nF_greater_0}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})\geq\Delta_{\text{LB}}(\mu,n_F,\mathbf{n}),
\end{equation}
where $\Delta_{\text{LB}}(\mu,n_F,\mathbf{n})$ is the solution of the linear optimization problem
\begin{subequations}
\label{eq:lb_cache_only_nF_greater_0}
\begin{align}
& \underset{\Delta_{E},\Delta_{F}}{\text{minimize}}
& & \Delta_{E}+\Delta_{F} \label{eq:zielfunktion}\\
& \text{subject to}
& & \Delta_{E}+\Delta_{F}\frac{n_{F}}{\max\{n_{d2},n_{d3}\}} \geq \frac{2-\mu}{\max\{n_{d2},n_{d3}\}} \label{eq:constraint_1}\\
& & & \Delta_{E}+\Delta_{F}\frac{n_{F}}{n_{d2}} \geq \frac{1-\mu}{n_{d2}} \label{eq:constraint_2}\\
& & & \Delta_{E}\geq \max\Bigg\{\frac{1}{n_{d3}},\frac{1}{\max\{n_{d1},n_{d2}\}},\frac{2}{\max\{n_{d1}+n_{d3},n_{d2}\}}\Bigg\} \label{eq:constraint_3}\\
& & & \Delta_{F}\geq 0 \label{eq:constraint_4}
\end{align}
\end{subequations}
and $\Delta_{E}$ and $\Delta_{F}$ denoting the individual DTBs of wireless and fronthaul transmissions. 
\end{proposition}
\noindent\begin{IEEEproof}
The proof of Proposition \ref{prop:2} is presented in Appendix \ref{app:lw_bound_ser_nF_greater_0}.   
\end{IEEEproof}
We next present multiple corollaries that specialize the lower bound of Proposition \ref{prop:2} to different settings of fronthaul capacities $n_{F}$. 
\begin{corollary}[Lower Bound for Low-Fronthaul Capacity Regime]\label{corr:1} For the F-RAN under study in the low-fronthaul capacity regime with $n_{F}\leq n_{d2}$, the DTB is lower bounded as
\begin{equation}\label{eq:lw_bound_low_fronthaul_capacity_regime}
\Delta^{*}_{\text{det}}(\mu,n_{F},\mathbf{n})\geq \max\Bigg\{\frac{1}{n_{d3}},\frac{1}{\max\{n_{d1},n_{d2}\}},\frac{2}{\max\{n_{d1}+n_{d3},n_{d2}\}},\frac{1-\mu}{n_{d2}},\frac{2-\mu}{\max\{n_{d2},n_{d3}\}}\Bigg\}. 
\end{equation}
\end{corollary}
\noindent \begin{IEEEproof}
We note that the lower bound on the wireless DTB $\Delta_{E}$ (see \eqref{eq:constraint_3}) is also a valid bound on the DTB $\Delta_{E}+\Delta_{F}$ due to the non-negativity of the fronthaul DTB $\Delta_{F}$ (cf. \eqref{eq:constraint_4}). Furthermore, for $n_{F}\leq n_{d2}$ the left-hand side (LHS) of \eqref{eq:constraint_1} and \eqref{eq:constraint_2} are upper bounded by the overall DTB $\Delta_{E}+\Delta_{F}$. Thus, \eqref{eq:constraint_1}--\eqref{eq:constraint_3} are all active lower bounds on the DTB. This concludes the proof.   
\end{IEEEproof}
\begin{remark} We see that the lower bound on the DTB $\Delta_{E}+\Delta_{F}$ in \eqref{eq:lw_bound_low_fronthaul_capacity_regime} coincides with the lower bound on $\Delta_{E}$ for $n_{F}=0$ in Proposition \ref{prop:1}. 
\end{remark}
\begin{corollary}[Lower Bound for High-Fronthaul Capacity Regime]\label{corr:2} For the F-RAN under study in the high-fronthaul capacity regime with $n_{F}\geq\max\{n_{d2},n_{d3}\}$, the DTB is lower bounded as
\begin{align}\label{eq:lw_bound_high_fronthaul_capacity_regime}
\Delta^{*}_{\text{det}}(\mu,n_{F},\mathbf{n})\geq \max\Bigg\{&\frac{2-\mu}{n_F}+\Bigg(1-\frac{\max\{n_{d2},n_{d3}\}}{n_{F}}\Bigg)\Delta_{\text{LB}}^{\prime}(\mathbf{n}),\nonumber\\& \frac{1-\mu}{n_{F}}+\Bigg(1-\frac{n_{d2}}{n_{F}}\Bigg)\Delta_{\text{LB}}^{\prime}(\mathbf{n}),\:\: \Delta_{\text{LB}}^{\prime}(\mathbf{n})\Bigg\}, 
\end{align} where $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ is defined in \eqref{eq:dlb_main}.
\end{corollary}
\noindent \begin{IEEEproof}
First, we note that $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ is identical to the right-hand side (RHS) of \eqref{eq:constraint_3}. This bound is a valid bound on the DTB $\Delta_{E}+\Delta_{F}$. For $n_{F}\geq\max\{n_{d2},n_{d3}\}$, we combine \eqref{eq:constraint_1} and \eqref{eq:constraint_2} with \eqref{eq:constraint_3}, which yields
\begin{subequations}
\label{eq:lb_reformulate_high_fronthaul}
\begin{align}
\Delta_{E}+\Delta_{F} & \geq \frac{2-\mu}{n_F}+\Bigg(1-\frac{\max\{n_{d2},n_{d3}\}}{n_{F}}\Bigg)\Delta_{\text{LB}}^{\prime}(\mathbf{n}) \label{eq:reformulate_constraint_1_high_fronthaul}\\
\Delta_{E}+\Delta_{F} & \geq \frac{1-\mu}{n_{F}}+\Bigg(1-\frac{n_{d2}}{n_{F}}\Bigg)\Delta_{\text{LB}}^{\prime}(\mathbf{n}). \label{eq:reformulate_constraint_2_high_fronthaul}
\end{align}
\end{subequations} The RHSs of inequalities \eqref{eq:reformulate_constraint_1_high_fronthaul}, \eqref{eq:reformulate_constraint_2_high_fronthaul} and \eqref{eq:constraint_3} result in \eqref{eq:lw_bound_high_fronthaul_capacity_regime} of Corollary \ref{corr:2}.    
\end{IEEEproof}
\begin{corollary}[Lower Bound for Medium-Fronthaul Capacity Regime in $\mathcal{I}_1$]\label{corr:3} For the F-RAN under study in the medium-fronthaul capacity regime $n_{F}\in[n_{d2},\max\{n_{d2},n_{d3}\}]$ and channel regime $\mathbf{n}\in\mathcal{I}_1$, the DTB is lower bounded as
\begin{align}\label{eq:lw_bound_medium_fronthaul_capacity_regime}
\Delta^{*}_{\text{det}}(\mu,n_{F},\mathbf{n})\geq \max\Bigg\{&\frac{2-\mu}{n_{d3}},\:\: \Delta_{\text{LB}}^{\prime}(\mathbf{n})\Bigg\}, 
\end{align} where $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ is defined in \eqref{eq:dlb_main}.
\end{corollary}
\noindent \begin{IEEEproof}
We observe that for $n_{F}\leq \max\{n_{d2},n_{d3}\}$, $\Delta_{E}+\Delta_{F}$ is an upper bound on the LHS of \eqref{eq:constraint_1}. For $\mathbf{n}\in\mathcal{I}_1$, it is easy to see that for any $\mu\in[0,1]$
\begin{equation}\label{eq:inequality_medium_fronthaul_I_1}
\Delta_{E}+\Delta_{F}\geq \frac{2-\mu}{n_{d3}}\geq\frac{1-\mu}{n_{d2}}
\end{equation} holds. Thus, only \eqref{eq:constraint_1} and \eqref{eq:constraint_3} are active lower bounds on the DTB. Combining these two bounds leads to \eqref{eq:lw_bound_medium_fronthaul_capacity_regime}.  
\end{IEEEproof}
\begin{corollary}[Lower Bound for Medium-Fronthaul Capacity Regime in $\mathcal{I}_1^{C}$]\label{corr:4} For the F-RAN under study in the medium-fronthaul capacity regime $n_{F}\in[n_{d2},\max\{n_{d2},n_{d3}\}]$ and channel regime $\mathbf{n}\in\mathcal{I}_1^{C}$, the DTB is lower bounded as
\begin{align}\label{eq:lw_bound_medium_fronthaul_capacity_regime_I1_C}
\Delta^{*}_{\text{det}}(\mu,n_{F},\mathbf{n})\geq\begin{cases}\max\Big\{\frac{1-\mu}{n_F}+\big(1-\frac{n_{d2}}{n_F}\big)\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n}),\:\:\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})\Big\}&\text{ for }\mu\leq \mu^{\prime\prime}(\mathbf{n})\\\max\Big\{\frac{2-\mu}{n_{d3}},\:\: \Delta_{\text{LB}}^{\prime}(\mathbf{n})\Big\}&\text{ for }\mu\geq \mu^{\prime\prime}(\mathbf{n})\end{cases}, 
\end{align} where $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ is defined in \eqref{eq:dlb_main} and $\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})$ equals
\begin{equation}\label{eq:delta_LB_prime_prime}
\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})=\max\Bigg\{\frac{1}{n_{d3}-n_{d2}},\:\:\Delta_{\text{LB}}^{\prime}(\mathbf{n})\Bigg\}.
\end{equation}
\end{corollary}
\noindent \begin{IEEEproof}
We observe that for $n_{F}\leq n_{d3}$, $\Delta_{E}+\Delta_{F}$ is an upper bound on the LHS of \eqref{eq:constraint_1}. For $\mathbf{n}\in\mathcal{I}_1^{C}$, one can show that for any $\mu\in[\mu^{\prime\prime}(\mathbf{n}),1]$
\begin{equation}\label{eq:inequality_medium_fronthaul_I_1}
\Delta_{E}+\Delta_{F}\geq \frac{2-\mu}{n_{d3}}\geq\frac{1-\mu}{n_{d2}}
\end{equation} holds. We infer that for this case only \eqref{eq:constraint_1} and \eqref{eq:constraint_3} are active lower bounds on the DTB. Combining these two bounds leads to the second case of \eqref{eq:lw_bound_medium_fronthaul_capacity_regime_I1_C}. For $\mu\in[0,\mu^{\prime\prime}(\mathbf{n})]$, on the other hand, we bound \eqref{eq:constraint_1} as follows:
\begin{eqnarray}\label{eq:bounding_constraint_1}
%\Delta_{E}+\Delta_{F}\geq \Delta_{E}+\Delta_{F}\frac{n_{F}}{n_{d3}}\geq \Delta_{E}\stackrel{(a)}\geq\frac{2-\mu}{n_{d3}}\geq \frac{2-\mu}{n_{d3}} \Bigg|_{\mu=\mu^{\prime\prime}(\mathbf{n})}=\frac{1}{n_{d3}-n_{d2}}
\Delta_{E}+\Delta_{F}\geq \Delta_{E}+\Delta_{F}\frac{n_{F}}{n_{d3}}\geq \Delta_{E}\geq\frac{2-\mu}{n_{d3}}\geq \frac{2-\mu}{n_{d3}} \Bigg|_{\mu=\mu^{\prime\prime}(\mathbf{n})}=\frac{1}{n_{d3}-n_{d2}}
\end{eqnarray} 
Using \eqref{eq:bounding_constraint_1} and \eqref{eq:constraint_3} together gives us a new lower bound \eqref{eq:delta_LB_prime_prime} on $\Delta_{E}$ (and ultimately on $\Delta_{E}+\Delta_{F}$). We obtain an additional bound on the DTB by combining \eqref{eq:delta_LB_prime_prime} and \eqref{eq:constraint_2}. This concludes the proof.     
\end{IEEEproof}
\subsection{Upper Bound (Achievability) on the Minimum DTB for $n_{F}\geq 0$}
\label{subsec:ser_upp_bound_nF_greater_0}

In this sub-section, we propose schemes to cover different operating channel regimes of the network under study for the cloud-only ($\mu=0$) case. As previously explained, we will only focus on the achievability at corner points \circled{$I_r$}, $r\in\{b,c,d\}$. Remaining intermediate points in the tradeoff curves on the DTB follow from the the convexity of the DTB (cf. Lemma \ref{lemma:1}). To show the achievability at extreme point
\begin{enumerate}[label=(\Alph*)]
\item \circled{$I_b$},
\item \circled{$I_c$}
\item and \circled{$I_d$},
\end{enumerate} we borrow results on the achievability of the \emph{cache-only case} of their respective, neighboring extreme point
\begin{enumerate}[label=(\Alph*)]
\item \circled{$II_b$}
\item \circled{$II_a$}
\item and \circled{$III$}
\end{enumerate} at cache sizes $\mu^{\prime}(\mathbf{n}), \mu^{\prime\prime}(\mathbf{n})$ and $\mu^{\prime\prime\prime}(\mathbf{n})$, respectively. In the sequel, we use the notation of the building block structure of sub-section \ref{subsec:ser_upp_bound}. We denote the requested file of $U_k$, $k=\{1,2\}$, by $W_{dk}$. 

The general idea of our proposed scheme is to apply a fronthaul transmission policy in such a way that the optimal \emph{wireless} latency $\Delta_{E}^{*}(\mu_{G}(\mathbf{n}),n_{F}=0,\mathbf{n})$ of the neighboring extreme points \circled{$II_b$}, \circled{$II_a$} and \circled{$III$} achieved at cache sizes $\mu_{G}(\mathbf{n})\in\{\mu^{\prime}(\mathbf{n}), \mu^{\prime\prime}(\mathbf{n}), \mu^{\prime\prime\prime}(\mathbf{n})\}$ become feasible at $\mu=0$ at the cost of additional fronthaul latency. $\Delta_{E}^{*}$ incurs when transmitting the requested files, each of length $L=R_{U}$ (see \eqref{eq:user_rate_1_and_2}), to $U_1$ and $U_2$ through the wireless channel without invoking the fronthaul link. Recall that the achievability of $\Delta_{E}^{*}(\mu_{G}(\mathbf{n}),n_{F}=0,\mathbf{n})$ was discussed in sub-section \ref{subsec:ser_upp_bound}. The rate allocation parameters are available in Tables \ref{tab:rate_alloc_param} through \ref{tab:rate_alloc_III}. To this end, the cloud server forms 
\begin{enumerate}[label=(\alph*)]
\item $R_{3,p}^{u}$ UNXORed bits of $W_{d1}$
\item and $R_{\text{IN}}^{w}$ XORed bits of $W_{d1}$ and $W_{d2}$
\end{enumerate} in the same manner as in the achievability scheme of \circled{$II_b$}, \circled{$II_a$} and \circled{$III$}, respectively. These bits are transmitted through the fronthaul link to the HeNB. Recall from Equation \eqref{eq:frac_cache_size} and Tables \ref{tab:rate_alloc_param} through \ref{tab:rate_alloc_III} that $\mu_{G}(\mathbf{n})L=R_{3,p}^{u}+R_{\text{IN}}^{w}$. Transmitting these $\mu_{G}(\mathbf{n})L$ bits induces a latency of $\Delta_{F}=\nicefrac{\mu_{G}(\mathbf{n})}{n_F}$. Thus, the overall DTB-latency becomes $\Delta_{E}+\Delta_{F}$, that is,
\begin{enumerate}[label=(\Alph*)]
\item \begin{equation}
\Delta_{\text{LB}}^{\prime}(\mathbf{n})+\frac{\mu^{\prime}(\mathbf{n})}{n_F} \end{equation}
\item \begin{equation}
\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})+\frac{\mu^{\prime\prime}(\mathbf{n})}{n_F} \end{equation}
\item and \begin{equation}
\Delta_{\text{LB}}^{\prime\prime}(\mathbf{n})+\frac{\mu^{\prime\prime\prime}(\mathbf{n})}{n_F}, \end{equation}
\end{enumerate} which is identical to $\Delta^{*}_{\text{det}}(\mu=0,n_F,\mathbf{n})$ of Theorem \ref{th:1}--\ref{th:3} for the underlying fronthaul capacity and channel regimes.

%In sub-section \ref{subsec:ser_upp_bound}, we have seen that cache-only schemes achieve the optimal DTB $\Delta_{E}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ at fractional cache size $\mu^{\prime}(\mathbf{n})$ in extreme point \circled{$II_b$}. This latency incurs when transmitting the requested files, each of length $L=R_{U}$ (see \eqref{eq:user_rate_1_and_2}), to $U_1$ and $U_2$ through the wireless channel without invoking the fronthaul link. At $\mu=0$ and $n_F\geq\max\{n_{d2},n_{d3}\}$, the exact same optimal \emph{wireless latency} $\Delta_{E}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ can be achieved at the cost of additional fronthaul latency $\Delta_{F}$. To this end, the cloud server forms 
%\begin{enumerate}[label=(\alph*)]
%\item $R_{3,p}^{u}$ UNXORed bits of $W_{d1}$
%\item and $R_{\text{IN}}^{w}$ XORed bits of $W_{d1}$ and $W_{d2}$
%\end{enumerate} in the same manner as in achievability scheme for \circled{$II_b$} and transmits them through its fronthaul link to the HeNB. We recall from Equation \eqref{eq:frac_cache_size} that $\mu^{\prime}(\mathbf{n})L=R_{3,p}^{u}+R_{\text{IN}}^{w}$. Transmitting these $\mu^{\prime}(\mathbf{n})L$ bits induces a latency of $\Delta_{F}=\nicefrac{\mu^{\prime}(\mathbf{n})}{n_F}$. Thus, the overall DTB-latency becomes $\Delta_{E}+\Delta_{F}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})+\nicefrac{\mu^{\prime}(\mathbf{n})}{n_F}$, which is identical to $\Delta^{*}_{\text{det}}(\mu=0,n_F,\mathbf{n})$ of Theorem \ref{th:1} and \ref{th:2} for $n_F\geq\max\{n_{d2},n_{d3}\}$ and $\mu^{\prime}(\mathbf{n})$ given in \eqref{eq:mu_prime}.
%  
%\vspace{0.5em}
%\subsubsection*{Scheme for Corner Point \circled{$I_b$}}
%
%In sub-section \ref{subsec:ser_upp_bound}, we have seen that cache-only schemes achieve the optimal DTB $\Delta_{E}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ at fractional cache size $\mu^{\prime}(\mathbf{n})$ in extreme point \circled{$II_b$}. This latency incurs when transmitting the requested files, each of length $L=R_{U}$ (see \eqref{eq:user_rate_1_and_2}), to $U_1$ and $U_2$ through the wireless channel without invoking the fronthaul link. At $\mu=0$ and $n_F\geq\max\{n_{d2},n_{d3}\}$, the exact same optimal \emph{wireless latency} $\Delta_{E}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ can be achieved at the cost of additional fronthaul latency $\Delta_{F}$. To this end, the cloud server forms 
%\begin{enumerate}[label=(\alph*)]
%\item $R_{3,p}^{u}$ UNXORed bits of $W_{d1}$
%\item and $R_{\text{IN}}^{w}$ XORed bits of $W_{d1}$ and $W_{d2}$
%\end{enumerate} in the same manner as in achievability scheme for \circled{$II_b$} and transmits them through its fronthaul link to the HeNB. We recall from Equation \eqref{eq:frac_cache_size} that $\mu^{\prime}(\mathbf{n})L=R_{3,p}^{u}+R_{\text{IN}}^{w}$. Transmitting these $\mu^{\prime}(\mathbf{n})L$ bits induces a latency of $\Delta_{F}=\nicefrac{\mu^{\prime}(\mathbf{n})}{n_F}$. Thus, the overall DTB-latency becomes $\Delta_{E}+\Delta_{F}=\Delta_{\text{LB}}^{\prime}(\mathbf{n})+\nicefrac{\mu^{\prime}(\mathbf{n})}{n_F}$, which is identical to $\Delta^{*}_{\text{det}}(\mu=0,n_F,\mathbf{n})$ of Theorem \ref{th:1} and \ref{th:2} for $n_F\geq\max\{n_{d2},n_{d3}\}$ and $\mu^{\prime}(\mathbf{n})$ given in \eqref{eq:mu_prime}.

%\subsubsection*{Scheme for Corner Point \circled{$I_c$} and \circled{$I_d$}}
%In the previous sub-section, we have seen that \emph{irrespective} of $n_F$ the optimal DTB $\nicefrac{T_E}{L}=\nicefrac{2}{(n_{d1}+n_{d3})}$ is achieved at fractional cache size $\mu^{\prime}$. This latency incurs when transmitting the requested files, each of length $L=n_{d1}+n_{d3}$, to $U_1$ and $U_2$ through the wireless channel without invoking the fronthaul link. At $\mu=0$ and $n_F\geq\max\{n_{d2},n_{d3}\}$, the exact same optimal wireless latency $\nicefrac{T_E}{L}=\nicefrac{2}{(n_{d1}+n_{d3})}$ can be achieved at the cost of additional fronthaul latency $\nicefrac{T_F}{L}$. To this end, the cloud server forms $\mu^{\prime}L=2(n_{d1}+n_{d3}-n_{d2})$ XORed bits (cf. Fig. 3(a) and (b)) of files $W_1$ and $W_2$ and transmits them through its fronthaul link to the HeNB. This fronthaul transmission induces a latency of $\nicefrac{T_F}{L}=\nicefrac{\mu^{\prime}}{n_F}$. Thus, the overall DTB-latency becomes $\nicefrac{T_F}{L}+\nicefrac{T_E}{L}$, which is identical to $\Delta^{*}_{\text{det}}(\mu=0,n_F)$.        



==> content/old_tables.tex <==
%% Tables that assumed n_f<= n_F,max

% Beginning
\begin{table}[h]
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$I_a$} at fractional cache size $\mu^{\prime}=0$ for $n_{F}\in[0,n_{F,\max}(\mathbf{n})]$ in channel regimes $\mathcal{C}_{1},\mathcal{R}_{2}$ and $\mathcal{R}_{3}$}
\label{tab:rate_alloc_I_a_R1_R3}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Regime & \multicolumn{2}{c|}{$\mathcal{C}_1$} & \multicolumn{2}{c|}{$\mathcal{R}_2$} & \multicolumn{2}{c|}{$\mathcal{R}_3$}
\\ \hline
Time $t$ & $t_1$ & $t_2$ & $t_1$ & $t_2$ & $t_1$ & $t_2$ 
\\ \hline
$R_{3,p}^{u}$ &  \multicolumn{6}{c|}{$0$} 
\\ \hline
$R_{2,p}^{u}$  & $n_{d3}-n_{d1}$ & $0$ &  \multicolumn{4}{c|}{$0$}
\\ \hline
$R_{1,p}^{u}$  &  \multicolumn{6}{c|}{$n_{d2}-n_{d3}$} 
\\ \hline
$R_{\text{FE}}^{u}$ & $n_{d1}+n_{d3}-n_{d2}-n_{F}$ & $0$ & $2n_{d3}-n_{d2}-n_{F}$ & $0$ & $2n_{d3}-n_{d2}-n_{F}$ & $0$
\\ \hline
$R_{\text{IN}}^{w}$ & \multicolumn{6}{c|}{$n_F$}
\\ \hline
$R_{\text{FE}}^{v}$  & $n_F$  & $n_{d1}+n_{d3}-n_{d2}$ & $n_F$  & $2n_{d3}-n_{d2}$ & $n_F$ & $2n_{d3}-n_{d2}$
\\ \hline
$R_{2,p}^{v}$ & $n_{d2}-n_{d3}$ & $n_{d2}-n_{d1}$ &  \multicolumn{4}{c|}{$n_{d2}-n_{d3}$}  
\\ \hline
$R_{1,p}^{v}$ & \multicolumn{6}{c|}{$0$}
\\ \hline
$l_4$ & \multicolumn{6}{c|}{$0$}
\\ \hline
$l_3$ &  \multicolumn{6}{c|}{$n_{d1}+n_{d3}-n_{d2}-n_{F}$}
\\ \hline
$l_2$  &  \multicolumn{4}{c|}{$2n_{d2}-n_{d1}-n_{d3}$} &  \multicolumn{2}{c|}{$n_{d2}-n_{d3}$}   
\\ \hline
$l_1$ &  \multicolumn{4}{c|}{$0$} &  \multicolumn{2}{c|}{$n_{d1}-n_{d2}$} 
\\ \hline 
\hline
$n_{F,\max}(\mathbf{n})$ & \multicolumn{2}{c|}{$n_{d1}+n_{d3}-n_{d2}$} & \multicolumn{2}{c|}{$2n_{d3}-n_{d2}$} & \multicolumn{2}{c|}{$2n_{d3}-n_{d2}$} \\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$I_a$} at fractional cache size $\mu^{\prime}=0$ for $n_{F}\in[0,n_{F,\max}(\mathbf{n})]$ in channel regimes $\mathcal{R}_{51}$ and $\mathcal{C}_{52}$}
\label{tab:rate_alloc_I_a_R51_R52}
\begin{tabular}{|c|c|c|c|c|}
\hline
Regime & \multicolumn{2}{c|}{$\mathcal{R}_{51}$} & \multicolumn{2}{c|}{$\mathcal{C}_{52}$} 
\\ \hline
Time $t$ & $t_1$ & $t_2$ & $t_1$ & $t_2$ 
\\ \hline
$R_{3,p}^{u}$ &  \multicolumn{4}{c|}{$0$}
\\ \hline
$R_{2,p}^{u}$  & \multicolumn{2}{c|}{$n_{d3}-n_{d2}$} & $n_{d3}-n_{d2}$ & $n_{d2}-n_{d1}$
\\ \hline
$R_{1,p}^{u}$  &  \multicolumn{4}{c|}{$0$}
\\ \hline
$R_{\text{FE}}^{u}$ & $2n_{d2}-n_{d3}-n_{F}$ & $0$ & $n_{d1}-n_{F}$ & $0$
\\ \hline
$R_{\text{IN}}^{w}$ & \multicolumn{4}{c|}{$n_F$}
\\ \hline
$R_{\text{FE}}^{v}$  & $n_F$  & $2n_{d2}-n_{d3}$ & $n_F$  & $n_{d1}$ 
\\ \hline
$R_{2,p}^{v}$ & \multicolumn{2}{c|}{$0$} & $2n_{d2}-n_{d1}-n_{d3}$ & $0$  
\\ \hline
$R_{1,p}^{v}$ & \multicolumn{4}{c|}{$n_{d3}-n_{d2}$}
\\ \hline
$l_4$ & \multicolumn{4}{c|}{$0$}
\\ \hline
$l_3$ &  \multicolumn{4}{c|}{$n_{d1}-n_{F}$}
\\ \hline
$l_2$  &  \multicolumn{4}{c|}{$n_{d3}-n_{d1}$} 
\\ \hline
$l_1$ &  \multicolumn{4}{c|}{$0$} 
\\ \hline 
\hline
$n_{F,\max}(\mathbf{n})$ & \multicolumn{2}{c|}{$2n_{d2}-n_{d3}$} & \multicolumn{2}{c|}{$n_{d1}$}
\\ \hline
\end{tabular}
\end{table}

\newcolumntype{C}{>{\centering\arraybackslash}p{11.0em}}
\begin{table}[h]
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$I_a$} at fractional cache size $\mu^{\prime}=0$ for $n_{F}\in[0,n_{F,\max}(\mathbf{n})]$ in channel regimes $\mathcal{R}_{4}$ and $\mathcal{R}_{61}$}
\label{tab:rate_alloc_I_a_R4_R62}
\begin{tabular}{|c||C|c|c|C|}
\hline
Regime & \multicolumn{2}{c|}{$\mathcal{R}_{4}$} & \multicolumn{2}{c|}{$\mathcal{R}_{61}$} 
\\ \hline
Time $t$ & $t_1$ & $t_2$ & $t_1$ & $t_2$ 
\\ \hline
%$R_{3,p}^{u}$ & $\min\Big\{\big(n_F-n_{d2}\big)^{+},n_{d3}-n_{d2}\Big\}$  & 
%\\ \hline
 $R_{3,p}^{u}$ & $\min\{n_{d3}-n_{d2},n_{F}\}$ & $\min\big\{(n_F-n_{d2}^{+},n_{F,\max}(\mathbf{n})-n_{d2}\big\}$  &  $\min\{n_{F},n_{d1}-n_{d2}\}$ & $\big(n_F-n_{d1}-n_{d2}+n_{d3}\big)^{+}$
 \\ \hline
$R_{2,p}^{u}$  & \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$0$}
\\ \hline
$R_{1,p}^{u}$  & \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$0$}
\\ \hline
$R_{\text{FE}}^{u}$ & $\min\{n_{d2},n_{d3}-n_{F}\}$ & $\big(n_{d3}-n_{d2}-n_{F}\big)^{+}$ & $\min\{n_{d2},n_{d1}-n_{F}\}$ & $\max\{n_{d3}-n_{d2}-n_{F},n_{d3}-n_{d1}\}$ 
\\ \hline
$R_{\text{IN}}^{w}$ & $\big(n_{d2}+n_F-n_{d3}\big)^{+}$ & $\min\{n_{d2},n_{F}\}$ & $\big(n_{d2}+n_F-n_{d1}\big)^{+}$ & $\min\{n_{F},n_{d1}+n_{d2}-n_{d3}\}$
\\ \hline
$R_{\text{FE}}^{v}$  & $\max\{n_{d3}-n_{d2},n_{F}\}$ & $\min\{n_{d2}+n_{F},n_{d3}\}$ & $\max\{n_{d1}-n_{d2},n_{F}\}$ & $\max\{2n_{d2}-n_{d3}+n_{F},n_{d1}+n_{d2}-n_{d3}\}$
\\ \hline
$R_{2,p}^{v}$ & \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$0$}
\\ \hline
$R_{1,p}^{v}$ & \multicolumn{2}{c|}{$0$} & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d2}$ 
\\ \hline
%$l_4$ &  $\max\Big\{\min\big\{n_{d1}-n_F,n_{d1}-n_{d2}\big\},n_{d1}-n_{d3}\Big\}$ & 
%\\ \hline
$l_4$ & $\max\{n_{d1}-n_{d3},n_{d1}-n_{d2}-n_{F}\}$ & $\min\big\{n_{d1}-n_F,n_{d1}-n_{d2}\big\}$ & $\big(n_{d1}-n_{d2}-n_F\big)^{+}$ & $\min\{2n_{d1}-n_{d3}-n_{F},n_{d1}-n_{d2}\}$
\\ \hline
$l_3$ & $\min\{n_{d2},n_{d3}-n_{F}\}$ & $\big(n_{d2}-n_{F}\big)^{+}$ & $\min\{n_{d2},n_{d1}-n_{F}\}$ & $\min\{n_{d3}-n_{d1},n_{d2}-n_{F}\}$
\\ \hline
$l_2$  & \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$n_{d3}-n_{d1}$}
\\ \hline
$l_1$ & \multicolumn{2}{c|}{$n_{d1}-n_{d3}$} & \multicolumn{2}{c|}{$0$}
\\ \hline \hline
$n_{F,\max}(\mathbf{n})$ & \multicolumn{2}{c|}{$n_{d3}$} & \multicolumn{2}{c|}{$2n_{d1}-n_{d3}$}
\\ \hline
\end{tabular}
\end{table}











% End

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Control
%\newcolumntype{C}{>{\centering\arraybackslash}p{4.0em}}

%\begin{landscape}
%\begin{table}[]
%\centering
%\caption{My caption}
%\label{my-label}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%\hline
%Regime & \multicolumn{2}{c|}{$\mathcal{R}_1$} & \multicolumn{2}{c|}{$\mathcal{R}_2$} & \multicolumn{2}{c|}{$\mathcal{R}_3$} & \multicolumn{2}{c|}{$\mathcal{R}_4$} & \multicolumn{2}{c|}{$\mathcal{R}_{51}$} & \multicolumn{2}{c|}{$\mathcal{R}_6$} & \multicolumn{2}{c|}{$\mathcal{R}_7$}
%\\ \hline
%\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 
%\\ \hline
%$R_{4,p}^{u}$ &  & & \multicolumn{4}{c|}{$0$} & $\min\{n_F,n_{d3}-n_{d2}\}$ &  & \multicolumn{2}{c|}{$0$} &                             &        &                             &        
%\\ \hline
%$R_{3,p}^{u}$ &  & & \multicolumn{4}{c|}{$0$} & $0$ &  & $n_{d3}-n_{d2}$ & $0$ &                             &        &                             &        
%\\ \hline
%$R_{2,p}^{u}$  &  & & $2n_{d3}-n_{d2}-n_{F}$ & $0$ &  $2n_{d3}-n_{d2}-n_{F}$ & $0$ & $\min\{n_{d2}, n_{d3}-n_{F}\}$ & $(n_{d3}-n_{d2}-n_{F})^{+}$ & $2n_{d2}-n_{d3}-n_{F}$ & $n_{d3}-n_{d2}$ &                             &        &                             &        
%\\ \hline
%$R_{1,p}^{u}$  &  & & \multicolumn{4}{c|}{$n_{d2}-n_{d3}$} & $0$ &  & \multicolumn{2}{c|}{$0$} &                             &        &                             &        
%\\ \hline
%$R_{\text{IN}}^{w}$ & & & \multicolumn{4}{c|}{$n_{F}$} & $(n_{d2}+n_{F}-n_{d3})^{+}$ & $\min\{n_{F},n_{d2}\}$ & \multicolumn{2}{c|}{$n_F$} &                             &        &                             &        
%\\ \hline
%$R_{2,p}^{v}$ &  &  & $n_{d2}-n_{d3}$ & $0$ & $n_{d2}-n_{d3}$ & $0$ & $0$ & $\min\{2n_{d2}+n_{F}-n_{d3},n_{d2}\}$ & $n_F$ & $0$ &                             &        &                             &        
%\\ \hline
%$R_{1,p}^{v}$ & &   & $n_{F}$ & $n_{d3}$ & $n_{F}$ & $n_{d3}$ &  $\max\{n_{d3}-n_{d2},n_{F}\}$ & $n_{d3}-n_{d2}$ & $n_{d3}-n_{d2}$ & $n_{d2}$ &                             &        &                             &        
%\\ \hline
%$l_4$ & & & \multicolumn{4}{c|}{$0$} & $\max\{n_{d1}-n_{d2}-n_{F},n_{d1}-n_{d3}\}$ &  & \multicolumn{2}{c|}{$0$} &                             &        &                             &        
%\\ \hline
%$l_3$ &  &  & \multicolumn{4}{c|}{$n_{d1}+n_{d3}-n_{d2}-n_{F}$} & $\min\{n_{d2},n_{d3}-n_{F}\}$ & $0$ & \multicolumn{2}{c|}{$n_{d1}+n_{d3}-2n_{d2}$} &                             &        &                             &        
%\\ \hline
%$l_2$  &  &  & \multicolumn{2}{c|}{$2n_{d2}-n_{d1}-n_{d3}$} & \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $(n_{d3}-n_{d2}-n_{F})^{+}$ & \multicolumn{2}{c|}{$2n_{d2}-n_{d1}-n_F$} &                             &        &                             &        
%\\ \hline
%$l_1$  &   &  &  \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$n_{d1}-n_{d2}$} & \multicolumn{2}{c|}{$n_{d1}-n_{d3}$} & \multicolumn{2}{c|}{$0$} &                             &        &                             &        
%\\ \hline
%\end{tabular}
%\end{table}
%\end{landscape}

%\begin{landscape}
%\begin{table}[]
%\centering
%\caption{My caption}
%\label{my-label}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%\hline
%Regime & \multicolumn{2}{c|}{$\mathcal{R}_1$} & \multicolumn{2}{c|}{$\mathcal{R}_2$} & \multicolumn{2}{c|}{$\mathcal{R}_3$} & \multicolumn{2}{c|}{$\mathcal{R}_4$} & \multicolumn{2}{c|}{$\mathcal{R}_{51}$}
%\\ \hline
%\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 
%\\ \hline
%$R_{4,p}^{u}$ &  & & \multicolumn{4}{c|}{$0$} & $\min\{n_F,n_{d3}-n_{d2}\}$ &  & \multicolumn{2}{c|}{$0$}
%\\ \hline
%$R_{3,p}^{u}$ &  & & \multicolumn{4}{c|}{$0$} & $0$ &  & $n_{d3}-n_{d2}$ & $0$  
%\\ \hline
%$R_{2,p}^{u}$  &  & & $2n_{d3}-n_{d2}-n_{F}$ & $0$ &  $2n_{d3}-n_{d2}-n_{F}$ & $0$ & $\min\{n_{d2}, n_{d3}-n_{F}\}$ & $(n_{d3}-n_{d2}-n_{F})^{+}$ & $2n_{d2}-n_{d3}-n_{F}$ & $n_{d3}-n_{d2}$
%\\ \hline
%$R_{1,p}^{u}$  &  & & \multicolumn{4}{c|}{$n_{d2}-n_{d3}$} & $0$ &  & \multicolumn{2}{c|}{$0$}
%\\ \hline
%$R_{\text{IN}}^{w}$ & & & \multicolumn{4}{c|}{$n_{F}$} & $(n_{d2}+n_{F}-n_{d3})^{+}$ & $\min\{n_{F},n_{d2}\}$ & \multicolumn{2}{c|}{$n_F$}
%\\ \hline
%$R_{2,p}^{v}$ &  &  & $n_{d2}-n_{d3}$ & $0$ & $n_{d2}-n_{d3}$ & $0$ & $0$ & $\min\{2n_{d2}+n_{F}-n_{d3},n_{d2}\}$ & $n_F$ & $0$
%\\ \hline
%$R_{1,p}^{v}$ & &   & $n_{F}$ & $n_{d3}$ & $n_{F}$ & $n_{d3}$ &  $\max\{n_{d3}-n_{d2},n_{F}\}$ & $n_{d3}-n_{d2}$ & $n_{d3}-n_{d2}$ & $n_{d2}$
%\\ \hline
%$l_4$ & & & \multicolumn{4}{c|}{$0$} & $\max\{n_{d1}-n_{d2}-n_{F},n_{d1}-n_{d3}\}$ &  & \multicolumn{2}{c|}{$0$} 
%\\ \hline
%$l_3$ &  &  & \multicolumn{4}{c|}{$n_{d1}+n_{d3}-n_{d2}-n_{F}$} & $\min\{n_{d2},n_{d3}-n_{F}\}$ & $0$ & \multicolumn{2}{c|}{$n_{d1}+n_{d3}-2n_{d2}$} 
%\\ \hline
%$l_2$  &  &  & \multicolumn{2}{c|}{$2n_{d2}-n_{d1}-n_{d3}$} & \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $(n_{d3}-n_{d2}-n_{F})^{+}$ & \multicolumn{2}{c|}{$2n_{d2}-n_{d1}-n_F$} 
%\\ \hline
%$l_1$  &   &  &  \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$n_{d1}-n_{d2}$} & \multicolumn{2}{c|}{$n_{d1}-n_{d3}$} & \multicolumn{2}{c|}{$0$} 
%\\ \hline
%\end{tabular}
%\end{table}
%\end{landscape}

%\begin{table}[]
%\centering
%\caption{My caption}
%\label{my-label}
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%Regime & \multicolumn{2}{c|}{$\mathcal{C}_{52}$} & \multicolumn{2}{c|}{$\mathcal{R}_{61}$}
%\\ \hline
%\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Slot 1} & Slot 2 & \multicolumn{1}{l|}{Slot 1} & Slot 2 
%\\ \hline
%$R_{4,p}^{u}$ & $0$ &   &  &        
%\\ \hline
%$R_{3,p}^{u}$  & $0$  &  &   &        
%\\ \hline
%$R_{2,p}^{u}$ & $n_{d1}+n_{d3}-n_{d2}-n_{F}$ &  &  &        
%\\ \hline
%$R_{1,p}^{u}$ & $0$   &  &   &        
%\\ \hline
%$R_{\text{IN}}^{w}$ & $n_{F}$ &  &  &        
%\\ \hline
%$R_{2,p}^{v}$ & $2n_{d2}-n_{d1}-n_{d3}$  &  &  &        
%\\ \hline
%$R_{1,p}^{v}$ & $n_{d3}-n_{d2}-n_{F}$  &  & &        
%\\ \hline
%$l_4$ & $0$  &  &    &        
%\\ \hline
%$l_3$ & $n_{d1}-n_{F}$ &    &   &        
%\\ \hline
%$l_2$  & $n_{d3}-n_{d1}$ &   &   &        
%\\ \hline
%$l_1$ & $0$  &   &   &        
%\\ \hline
%\end{tabular}
%\end{table}


==> content/temp_maybe_useful_latter.tex <==
\subsubsection*{Scheme for Corner Point \circled{$II_b$}}
% Control
\newcolumntype{C}{>{\centering\arraybackslash}p{4.0em}}
\begin{table}[t]
%\centering
\caption{Rate allocation parameters for the proposed scheme for $n_{F}=0$ at fractional cache size $\mu^{\prime}(\mathbf{n})$}
%\label{tab:rate_alloc_param}
%\begin{tabular}{|c||c|C|C|c|c|c|c|}
%\hline
%Regime & $\mathcal{R}_1$ & $\mathcal{R}_2$ & $\mathcal{R}_3$ & $\mathcal{R}_4$ & $\mathcal{R}_5$ & $\mathcal{R}_6$ & $\mathcal{R}_7$ \\ \hline 
%$R_{3,p}^{u}$ & $0$ & \multicolumn{2}{c|}{$0$} & $n_{d3}-n_{d2}$ & $n_{d1}-n_{d2}$ & $0$ & $0$ \\ \hline
%$R_{2,p}^{u}$ & $\frac{n_{d3}-n_{d1}}{2}$ &  \multicolumn{2}{c|}{$0$} & $0$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d2}$ & $\frac{n_{d3}-n_{d1}}{2}$ \\ \hline
%$R_{1,p}^{u}$ & $n_{d2}-n_{d3}$ &  \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $0$ & $0$ & $0$ \\ \hline
%$R_{\text{IN}}^{w}$  & $n_{d1}+n_{d3}-n_{d2}$ & \multicolumn{2}{c|}{$2n_{d3}-n_{d2}$} & $n_{d2}$ & $n_{d1}+n_{d2}-n_{d3}$ & $2n_{d2}-n_{d3}$ & $n_{d1}$ \\ \hline
%$R_{p}^{v}$  & $\frac{n_{d1}+n_{d3}}{2}$ & \multicolumn{2}{c|}{$n_{d3}$} & $n_{d3}$ & $n_{d1}$ & $n_{d2}$ & $\frac{n_{d1}+n_{d3}}{2}$\\ \hline
%$l_4$ &\multicolumn{7}{|c|}{$0$} \\ \hline
%$l_3$ & $0$ & $0$ & $n_{d1}-n_{d2}$ & $0$ & $n_{d3}-n_{d1}$ & $n_{d1}+n_{d3}-2n_{d2}$ & $0$ \\ \hline
%$l_2$ & $2n_{d2}-n_{d1}-n_{d3}$ & \multicolumn{2}{c|}{$2n_{d2}-2n_{d3}$} & $0$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d1}$ \\ \hline
%$l_1$ & $0$ & $0$ & $n_{d1}-n_{d2}$ & $n_{d1}-n_{d3}$ & $0$ & $0$ & $0$ \\ \hline
%\end{tabular}
%\end{table}
\label{tab:rate_alloc_param}
\begin{tabular}{|c||c|C|C|c|c|c|c|}
\hline
Regime & $\mathcal{R}_1$ & $\mathcal{R}_2$ & $\mathcal{R}_3$ & $\mathcal{C}_4$ & $\mathcal{R}_{51}$ & $\mathcal{R}_{52}$ & $\mathcal{C}_{61}$ 
\\ \hline 
$R_{3,p}^{u}$ & $0$ & \multicolumn{2}{c|}{$0$} & $n_{d3}-n_{d2}$ & $0$ & $0$ & $n_{d1}-n_{d2}$
\\ \hline
$R_{2,p}^{u}$ & $\frac{n_{d3}-n_{d1}}{2}$ &  \multicolumn{2}{c|}{$0$} & $0$ & $n_{d3}-n_{d2}$ & $\frac{n_{d3}-n_{d1}}{2}$ & $n_{d3}-n_{d1}$  
\\ \hline
$R_{1,p}^{u}$ & $n_{d2}-n_{d3}$ &  \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $0$ & $0$ & $0$ 
\\ \hline
$R_{\text{IN}}^{w}$  & $n_{d1}+n_{d3}-n_{d2}$ & \multicolumn{2}{c|}{$2n_{d3}-n_{d2}$} & $n_{d2}$ & $2n_{d2}-n_{d3}$ & $n_{d1}$ & $n_{d1}+n_{d2}-n_{d3}$
\\ \hline
$R_{p}^{v}$  & $\frac{n_{d1}+n_{d3}}{2}$ & \multicolumn{2}{c|}{$n_{d3}$} & $n_{d3}$ & $n_{d2}$ & $\frac{n_{d1}+n_{d3}}{2}$ & $n_{d1}$ 
\\ \hline
$l_4$ & \multicolumn{3}{|c|}{$0$} & $n_{d1}-n_{d3}$ & \multicolumn{3}{c|}{$0$}
\\ \hline
$l_3$ & $0$ & $n_{d2}-n_{d3}$ & $n_{d1}-n_{d3}$ & $0$ & $n_{d1}+n_{d3}-2n_{d2}$ & $0$ & $n_{d3}-n_{d1}$  
\\ \hline
$l_2$ & $2n_{d2}-n_{d1}-n_{d3}$ & \multicolumn{2}{c|}{$n_{d2}-n_{d3}$} & $0$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d1}$
\\ \hline
$l_1$ & $0$ & $0$ & $n_{d1}-n_{d2}$ & $n_{d1}-n_{d3}$ & $0$ & $0$ & $0$ 
\\ \hline
\end{tabular}
\end{table}

The  first  scheme  is  developed for the  channel regimes $\mathcal{R}_1$--$\mathcal{R}_7$. Through the comparison with the converse, we show that this scheme performs optimally at fractional cache size $\mu^{\prime}(\mathbf{n})$ from \eqref{eq:mu_prime}.  

The encoding at the transmitters, both eNB and HeNB, follows along the building structure of Fig. \ref{fig:ldm_stack}. The length of each signal vector is appropriately determined to individually account for all channel regimes while maximizing the \emph{symmetric} per-use rate. This has the effect that the latency of providing each user with its requested file are the same. All the proposed schemes require $T_{E}=1$ channel use to perform optimally.   

The transmission according to the block structure of Fig. \ref{fig:ldm_stack} require that at the respective receivers interference-decoding and treating interference as noise (TIN) is applied successively such that the achievable rates of $U_1$ and $U_2$ for $T_{E}=1$ become
\begin{subequations}
\begin{alignat}{2}
R_{U_1}&=R_{\text{IN}}^{w}+\sum_{i=1}^{3}R^{u}_{i,p},\label{eq:ach_rate_U1}\\
R_{U_2}&=R^{v}_{p},\label{eq:ach_rate_U2}
\end{alignat}   
\end{subequations} respectively.  
%\begin{subequations}
%\begin{alignat}{2}
%R_{U_1}&=R_{\text{IN}}^{w}+\sum_{i=1}^{3}R^{u}_{i,p}\label{eq:ach_rate_U1}\\
%R_{U_2}&=\sum_{j=1}^{2}R^{v}_{j,p},\label{eq:ach_rate_U2}
%\end{alignat}   
%\end{subequations} respectively.  
For the channel regimes $\mathcal{R}_1$--$\mathcal{R}_7$, we carefully choose the rate allocation parameters $R_{i,p}^{u},R_{p}^{v},R_{\text{IN}}^{w}$ and the respective null vectors such that the achievable per-user rates are identical, i.e.,
\begin{equation}
\label{eq:user_rate_1_and_2}
R_{U_1}=R_{U_2}\triangleq R_{U}
\end{equation} at fractional cache size \begin{equation}
\label{eq:frac_cache_size}
\mu^{\prime}_{\text{Ach}}(\mathbf{n})=\frac{R_{3,p}^{u}+R_{\text{IN}}^{w}}{R_{U}}.
\end{equation}
Table \ref{tab:rate_alloc_param} summarizes how the rate allocation parameters ought to be chosen so that \eqref{eq:user_rate_1_and_2} and \eqref{eq:frac_cache_size} are both satisfied. As a result, the proposed transmission strategy would not favor any user; hence, making the completion time, thus the latency, for delivering the requested files fair to both users. We follow that each user can reliably decode $R_{U}$ bits per channel use, or in other words, $\Delta_{\text{det}}(\mu=\mu^{\prime}_{\text{Ach}},n_F=0,\mathbf{n})=\nicefrac{1}{R_U}$ channel uses are required to provide each user with one bit. Note that the achievable DTB and $\mu^{\prime}_{\text{Ach}}$ match \eqref{eq:DTB_theorem} and \eqref{eq:mu_prime}, respectively. This proves the achievability of Theorem \ref{th:1} for all seven regimes corresponding to this scheme.

\subsubsection*{Scheme for Regimes $\mathcal{R}_{61}^{\prime}$} 
% Control
\newcolumntype{C}{>{\centering\arraybackslash}p{6.0em}}
\begin{table}[t]
\centering
\caption{Rate allocation parameters for the proposed scheme for $n_{F}=0$ at fractional cache sizes $\mu^{\prime\prime}(\mathbf{n})$ (left) and $\mu^{\prime\prime\prime}(\mathbf{n})$ (right)}
\label{tab:rate_alloc_param_new}
\begin{tabular}{|c||C|C|}
\hline
Regime & $\mathcal{R}_{4}^{\prime}$ & $\mathcal{R}_{61}^{\prime}$ \\ \hline 
$R_{3,p}^{u}$ & \multicolumn{2}{c|}{$n_{d3}-2n_{d2}$} \\ \hline
$R_{2,p}^{u}$ & \multicolumn{2}{c|}{$n_{d2}$} \\ \hline
$R_{1,p}^{u}$ & \multicolumn{2}{c|}{$0$} \\ \hline
$R_{\text{IN}}^{w}$  & \multicolumn{2}{c|}{$0$} \\ \hline
$R_{p}^{v}$  & \multicolumn{2}{c|}{$n_{d3}-n_{d2}$} \\ \hline
$l_4$ & \multicolumn{2}{c|}{$n_{d1}+n_{d2}-n_{d3}$} \\ \hline
$l_3$ & $n_{d2}$ & $n_{d2}+n_{d3}-n_{d1}$ \\ \hline
$l_2$ & \multicolumn{2}{c|}{$0$} \\ \hline
$l_1$ & $n_{d1}-n_{d3}$ & $0$ \\ \hline
\end{tabular}
% Other Table (Side by Side)
\hspace{10em}
\begin{tabular}{|c||c|}
\hline
Regime & $\mathcal{R}_{62}^{\prime}$ \\ \hline 
$R_{3,p}^{u}$ & $n_{d1}-n_{d2}$ \\ \hline
$R_{2,p}^{u}$ & $n_{d2}$ \\ \hline
$R_{1,p}^{u}$ & $0$ \\ \hline
$R_{\text{IN}}^{w}$  & $0$ \\ \hline
$R_{p}^{v}$  & $n_{d1}$ \\ \hline
$l_4$ & $0$ \\ \hline
$l_3$ & $0$ \\ \hline
$l_2$ & $n_{d2}+n_{d3}-n_{d1}$ \\ \hline
$l_1$ & $n_{d3}-n_{d1}-n_{d2}$ \\ \hline
\end{tabular}
\end{table}

==> content/temp_par.tex <==
\section{Parallel Transmission}
\label{sec:par_trans}

In  this  section,  we  provide  coinciding lower bounds (converse) and upper bounds (achievability) on the minimum DTB for the F-RAN in Fig. \ref{fig:HetNet} for a parallel fronthaul-edge transmission under various channel regimes. The main result of this section is stated in the following theorems.
%This results in Theorems \ref{th:5}--\ref{th:8}.
\vspace{.5em}
%\begin{theorem}\label{th:5}
%In the channel regimes 
%\begin{enumerate}[label=(\alph*)]
%\item $\mathbf{n}\in\{\mathcal{R}_i\}_{i=1}^{4}$, $\mathcal{R}_{51}$, $\mathcal{R}_{52}$
%\item $\mathbf{n}\in\mathcal{R}_{62}^{\prime}$
%\end{enumerate} the optimal DTB of the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} for a parallel fronthaul-edge transmission at fronthaul capacities $n_{F}\in[0,n_{F,\max}(\mathbf{n})]$ corresponds to 
%\begin{enumerate}[label=(\alph*)]
%\item \begin{equation}\label{eq:DTB_theorem_th_5_1}
%\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\begin{cases}\frac{2-\mu}{n_{F}+\max\{n_{d2},n_{d3}\}}\qquad&\text{for }0\leq\mu\leq\mu_{P}^{\prime}(n_F,\mathbf{n})\\\frac{2-\mu_{P}^{\prime}(n_F,\mathbf{n})}{n_{F}+\max\{n_{d2},n_{d3}\}}\qquad&\text{for }\mu_{P}^{\prime}(n_F,\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation} 
%\NoIndent{and}
%\item \begin{equation}\label{eq:eq:DTB_theorem_th_5_2}
%\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\begin{cases}\frac{1-\mu}{n_{F}+n_{d2}}\qquad&\text{for }0\leq\mu\leq\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})\\\frac{1-\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})}{n_{F}+n_{d2}}\qquad&\text{for }\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation}
%\end{enumerate} respectively, where
%\begin{equation}\label{eq:mu_prime_par}
%\mu_{P}^{\prime}(n_F,\mathbf{n})=2-\Big(n_F+\max\{n_{d2},n_{d3}\}\Big)\Delta_{\text{LB}}^{\prime}(\mathbf{n}),
%\end{equation}
%\begin{equation}\label{eq:mu_prime_prime_prime_par}
%\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})=1-\Big(n_F+n_{d2}\Big)\Delta_{\text{LB}}^{\prime}(\mathbf{n})=\frac{n_{d1}-n_{d2}-n_{F}}{n_{d1}}.
%\end{equation} and 
%\begin{equation}\label{eq:nF_max}  
%n_{F,\max}(\mathbf{n})=\max\Bigg\{\frac{1}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-n_{d2},\frac{2}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-\max\{n_{d2},n_{d3}\}\Bigg\}.
%\end{equation}
%\begin{equation}\label{eq:nF_max}  
%n_{F,\max}(\mathbf{n})=\frac{2}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-\max\{n_{d2},n_{d3}\}.
%\end{equation}
%\end{theorem}
\begin{theorem}\label{th:2}
The DTB of the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} under parallel fronthaul-edge transmissions for any $n_{F}\geq 0$ and $\mu\in[0,1]$ is given by
\begin{equation}\label{eq:DTB_theorem_th_2}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\max\Bigg\{\frac{1-\mu}{n_{F}+n_{d2}},\frac{2-\mu}{n_{F}+\max\{n_{d2},n_{d3}\}},\Delta_{\text{LB}}^{\prime}(\mathbf{n})\Bigg\},
\end{equation} where
\begin{equation}\label{eq:mu_prime_par}
\mu_{P}^{\prime}(n_F,\mathbf{n})=2-\Big(n_F+\max\{n_{d2},n_{d3}\}\Big)\Delta_{\text{LB}}^{\prime}(\mathbf{n})
\end{equation} and 
\begin{equation}\label{eq:nF_max}  
n_{F,\max}(\mathbf{n})=\max\Bigg\{\frac{1}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-n_{d2},\frac{2}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-\max\{n_{d2},n_{d3}\}\Bigg\}.
\end{equation}
%\begin{equation}\label{eq:nF_max}  
%n_{F,\max}(\mathbf{n})=\frac{2}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-\max\{n_{d2},n_{d3}\}.
%\end{equation}
\end{theorem}
\begin{theorem}\label{th:5}
In the channel regimes $\mathbf{n}\in\{\mathcal{R}_i\}_{i=1}^{4}$, $\mathcal{R}_{51}$, $\mathcal{R}_{52}$ and $\mathcal{R}_{61}$ the optimal DTB of the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} for a parallel fronthaul-edge transmission at fronthaul capacities $n_{F}\in[0,n_{F,\max}(\mathbf{n})]$ corresponds to 
\begin{equation}\label{eq:DTB_theorem_th_5}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\begin{cases}\frac{2-\mu}{n_{F}+\max\{n_{d2},n_{d3}\}}\qquad&\text{for }0\leq\mu\leq\mu_{P}^{\prime}(n_F,\mathbf{n})\\\frac{2-\mu_{P}^{\prime}(n_F,\mathbf{n})}{n_{F}+\max\{n_{d2},n_{d3}\}}\qquad&\text{for }\mu_{P}^{\prime}(n_F,\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation} where
\begin{equation}\label{eq:mu_prime_par}
\mu_{P}^{\prime}(n_F,\mathbf{n})=2-\Big(n_F+\max\{n_{d2},n_{d3}\}\Big)\Delta_{\text{LB}}^{\prime}(\mathbf{n})
\end{equation} and 
\begin{equation}\label{eq:nF_max}  
n_{F,\max}(\mathbf{n})=\max\Bigg\{\frac{1}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-n_{d2},\frac{2}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-\max\{n_{d2},n_{d3}\}\Bigg\}.
\end{equation}
%\begin{equation}\label{eq:nF_max}  
%n_{F,\max}(\mathbf{n})=\frac{2}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})}-\max\{n_{d2},n_{d3}\}.
%\end{equation}
\end{theorem}
\vspace{.5em}
\begin{theorem}\label{th:6}
In the channel regimes $\mathbf{n}\in\mathcal{R}_4^{\prime}$ and $\mathcal{R}_{61}^{\prime}$ the optimal DTB of the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} for a parallel fronthaul-edge transmission at fronthaul capacities 
\begin{enumerate}[label=(\alph*)]
\item $0\leq n_{F}\leq n_{F,\text{IM}}(\mathbf{n})\triangleq n_{d3}-2n_{d2}$
\item $n_{F,\text{IM}}(\mathbf{n})\leq n_{F}\leq n_{F,\max}(\mathbf{n})$
\end{enumerate} is given by
\begin{enumerate}[label=(\alph*)]
\item \begin{equation}\label{eq:DTB_theorem_cloud_th_6_low_fronthaul_par}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\begin{cases}\frac{1-\mu}{n_{F}+n_{d2}}\qquad&\text{for }0\leq\mu\leq\mu^{\prime\prime}_{P}(n_{F},\mathbf{n})\\ \frac{2-\mu}{n_{F}+\max\{n_{d2},n_{d3}\}}\qquad&\text{for }\mu^{\prime\prime}_{P}(n_{F},\mathbf{n})\leq\mu\leq\mu^{\prime}_{P}(n_{F},\mathbf{n})\\\frac{2-\mu^{\prime}_{P}(n_{F},\mathbf{n})}{n_{F}+\max\{n_{d2},n_{d3}\}}\qquad&\text{for }\mu^{\prime}_{P}(n_{F},\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation} 
\NoIndent{and}
\item Equation \eqref{eq:DTB_theorem_th_5}, 
\end{enumerate} respectively. $\mathbf{\mu}^{\prime}_{P}(n_{F},\mathbf{n})$ and $n_{F,\max}(\mathbf{n})$ are defined in \eqref{eq:mu_prime_par} and \eqref{eq:nF_max}. The fractional cache size $\mathbf{\mu}^{\prime\prime}_{P}(n_{F},\mathbf{n})$ in \eqref{eq:DTB_theorem_cloud_th_6_low_fronthaul_par} corresponds to: \begin{equation}\label{eq:mu_prime_prime_par}
\mu^{\prime\prime}_{P}(n_{F},\mathbf{n})=\frac{n_{d3}-2n_{d2}-n_{F}}{n_{d3}-n_{d2}}.
\end{equation}
\end{theorem}
\vspace{.5em}
\begin{theorem}\label{th:7}
In the channel regime $\mathbf{n}\in\mathcal{R}_{62}^{\prime}$ the optimal DTB of the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} for a parallel fronthaul-edge transmission at fronthaul capacities $n_{F}\in[0,n_{F,\max}(\mathbf{n})]$ corresponds to
\begin{equation}\label{eq:DTB_theorem_cloud_th_7_low_fronthaul_par}
\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})=\begin{cases}\frac{1-\mu}{n_{F}+n_{d2}}\qquad&\text{for }0\leq\mu\leq\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})\\\frac{1-\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})}{n_{F}+n_{d2}}\qquad&\text{for }\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})\leq\mu\leq 1\end{cases},\end{equation} where $\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})$ is   \begin{equation}\label{eq:mu_prime_prime_prime_par}
\mu^{\prime\prime\prime}_{P}(n_{F},\mathbf{n})=1-\big(n_F+n_{d2}\big)\Delta_{\text{LB}}^{\prime}(\mathbf{n})=\frac{n_{d1}-n_{d2}-n_{F}}{n_{d1}}.
\end{equation}
\end{theorem}
\begin{theorem}[Constant DTB]\label{th:8}
In the channel regimes \begin{equation}\label{eq:channel_regimes_th_8}
\begin{cases}\{\mathcal{R}_i\}_{i=1}^{3}\\
\mathcal{C}_4\\
\{\mathcal{R}_{5i}\}_{i=1}^{2}\\
\mathcal{C}_{61}\\\mathcal{R}_{62}^{\prime}\end{cases}, \end{equation}
the optimal DTB of the cloud and cache-aided HetNet for any $n_{F}\geq n_{F,\max}(\mathbf{n})$ does not depend on the fractional cache size $\mu$ and remains constant. It corresponds to \begin{equation}\label{eq:DTB_theorem_cloud_th_8_cache_ineff}
\Delta_{\text{det}}(\mu,n_F,\mathbf{n})=\Delta_{\text{LB}}^{\prime}(\mathbf{n}).
\end{equation}
\end{theorem}
\noindent \begin{IEEEproof} (Theorem \ref{th:5}--\ref{th:8}) Lower bounds on the DTB are provided in sub-section \ref{subsec:par_low_bound} while upper bounds can be found in sub-section \ref{subsec:par_upp_bound}. 
\end{IEEEproof}
\begin{figure*}
        \centering
        \begin{subfigure}[b]{0.475\textwidth}
            \centering
            \begin{tikzpicture}[scale=1]
            \Resultonepar
            \end{tikzpicture}
            \caption{{\small $\mathbf{n}\in\{\mathcal{R}_i\}_{i=1}^{4},\mathcal{R}_{51},\mathcal{R}_{52}$ and $\mathcal{R}_{61}$}}    
            \label{fig:th_5}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}  
            \centering 
            \begin{tikzpicture}[scale=1]
            \Resulttwopar
            \end{tikzpicture}
            \caption{{\small $\mathbf{n}\in\mathcal{R}_{4}^{\prime}$ and $\mathcal{R}_{61}^{\prime}$}}     
            \label{fig:th_6}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \begin{tikzpicture}[scale=1]
            \Resulthreepar
            \end{tikzpicture}
            \caption{{\small $\mathbf{n}\in\mathcal{R}_{62}^{\prime}$}}    
            \label{fig:th_7}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \begin{tikzpicture}[scale=1]
            \Resultfourpar
            \end{tikzpicture}
            \caption{{\small $\mathbf{n}\in\mathcal\{{R}_{i}\}_{i=1}^{3},\mathcal{C}_{4},\mathcal{R}_{51},\mathcal{R}_{52},\mathcal{C}_{61}$ and $\mathcal{R}_{62}^{\prime}$}}  
            \label{fig:th_8}
        \end{subfigure}
        \caption[DTB as a function of $\mu$ for various channel regimes and distinct fronthaul capacities]
        {\small DTB as a function of $\mu$ for various channel regimes and distinct fronthaul capacities ($0\leq n_{F_1}\leq n_{F_2}\leq n_{F_3}\leq n_{F,\max}(\mathbf{n})$)} 
        \label{fig:results_par}
\end{figure*}
\vspace{.5em}
\begin{remark}[Serial vs. Parallel Tranmission Schemes]
In all channel regimes of Theorem \ref{th:5}--\ref{th:7}, we observe similar performance curves for both serial and parallel fronthaul-edge transmission policies (cf. Figs. \ref{fig:results} and \ref{fig:results_par}). Two main differences are: 
\begin{enumerate} \item First, only for the latter, fractional cache sizes of corner points \circled{$II_a$}, \circled{$II_b$} and \circled{$III$} explicitly depend on the fronthaul capacity $n_{F}$. This dependency causes that increasing $n_{F}$ by some positive $\delta$ will lead to a linear proportional decrease by $\delta$ in these points' fractional cache sizes. This behavior is shown by a left shift of \circled{$II_a$}, \circled{$II_b$} and \circled{$III$} in Figs. \ref{fig:th_5}--\ref{fig:th_7}.
\item Second, only for the latter we require a finite $n_{F}=n_{F,\max}(\mathbf{n})$ to attain the lowest possible DTB $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ (see Fig. \ref{fig:th_8}). In contrast, serial fronthaul-edge schemes needed an infinite fronthaul capacity ($n_{F}=\infty$) to achieve the same DTB. In other words, fronthaul capacities in the range $n_{F}\in(n_{F,\max}(\mathbf{n}),\infty)$ have a latency-reducing effect only under serial fronthaul-edge schemes. The intuition behind this result is that in parallel transmission policies cloud resources are effectively utilized to overcome partial caching while incurring less fronthaul latency than serial transmission schemes. As a consequence, a finite $n_{F}$ suffices to obtain the DTB $\Delta_{\text{LB}}^{\prime}(\mathbf{n})$.     
\end{enumerate}  
\end{remark}
\vspace{.5em}
\begin{remark}[Maximum Fronthaul Capacity $n_{F,\max}(\mathbf{n})$]
One can verify from Equation \eqref{eq:nF_max} that $n_{F,\max}(\mathbf{n})\leq n_{d1}$. This suggests that any full-duplex HeNB is capable to forward any fronthaul message of any time instant, say $t-1$, through the wireless HeNB-to-$U_1$ link in the consecutive channel use $t$. Our achievability schemes (see sub-section \ref{subsec:par_upp_bound}) make implicit use of this observation.     
\end{remark}
\vspace{0.5em}
Throughout the rest of this section we elaborate on lower (cf. \ref{subsec:par_low_bound}) and upper bounds (see \ref{subsec:par_upp_bound}) on the DTB for the case of parallel fronthaul-edge transmissions. We put our focus on the achievability. In the respective sub-section, we introduce transmission schemes which achieve the optimal DTB provided in Theorem \ref{th:5}--\ref{th:8} (cf. Fig. \ref{fig:results_par}). To this end, various schemes are proposed to cover different operating channel regimes of the network under study. Due to the convexity of the DTB, we establish the achievability of corner points in the latency-memory tradeoff curves. In Fig. \ref{fig:results_par}, depending on the operating channel regime, these corner points are denoted by \circled{$I_r$},
$r\in\{a,b\}$, \circled{$II_s$}, $s\in\{a,b\}$, and \circled{$III$}. In this regard, we will show that corner points 
\begin{itemize}
\item \circled{$I_r$}, $r\in\{a,b\}$, involve only fronthauling and do not require edge caching ($\mu=0$); thus, representing cloud-only transmission policies, whereas 
\item \circled{$II_a$}, \circled{$II_b$} and \circled{$III$} involve both edge caching and fronthauling; thus, representing fronthaul-edge transmission policies.
\end{itemize} 
%When showing the achievability of \circled{$II_a$}, \circled{$II_b$} and \circled{$III$}, we will use schemes of these points for the serial  
In general, the DTB at fractional cache size $\mu$ which lies between two neighboring corner points (say \circled{A} and \circled{B}) cache sizes' is achieved through memory sharing between the policies at corner point \circled{A} and \circled{B}. For parallel fronthaul edge transmissions, corner points \circled{A} and \circled{B} are operational at channel regimes $\mathcal{R}_{\circled{A}}$ and $\mathcal{R}_{\circled{B}}$ for non-negative fronthaul capacities below $n_{F,\max}^{\text{\circled{A}}}$ and $n_{F,\max}^{\text{\circled{B}}}$, respectively. Thus, any intermediate point between \circled{A} and \circled{B} is achievable through memory sharing when we restrict the channel regime to be 
$\mathcal{R}_{\circled{A}}\cap\mathcal{R}_{\circled{B}}$ for fronthaul capacities less than $\min\Big\{n_{F,\max}^{\text{\circled{A}}},n_{F,\max}^{\text{\circled{B}}}\Big\}$.
\subsection{Lower Bound (Converse) on the Minimum DTB}
\label{subsec:par_low_bound}

\begin{proposition}[Lower Bound on the Minimum DTB for F-RAN with Parallel Fronthaul-Edge Transmission]\label{prop:3}
For the LDM-based cloud and cache-aided HetNet in Fig. \ref{fig:HetNet} under a parallel fronthaul-edge transmission setting, the optimal DTB $\Delta_{\text{det}}^{*}(\mu,n_F,\mathbf{n})$ is lower bounded as
\begin{equation}
\label{eq:par_lb}
\Delta_{\text{det},P}^{*}(\mu,n_F,\mathbf{n})\geq\Delta_{\text{LB},P}(\mu,\mathbf{n}),
\end{equation}
where \begin{equation}
\label{eq:lb_par}
\Delta_{\text{LB},P}(\mu,n_F,\mathbf{n})=\max\Bigg\{\frac{1}{n_{d3}},\frac{1}{\max\{n_{d1},n_{d2}\}}, \frac{2}{\max\{n_{d1}+n_{d3},n_{d2}\}},\frac{1-\mu}{n_F+n_{d2}},\frac{2-\mu}{n_F+\max\{n_{d2},n_{d3}\}}\Bigg\}.
\end{equation}
\end{proposition}
\noindent\begin{IEEEproof}
The proof of Proposition \ref{prop:3} is presented in Appendix \ref{app:lw_bound_par}.   
\end{IEEEproof}

\subsection{Upper Bound (Achievability) on the Minimum DTB}
\label{subsec:par_upp_bound}

In this sub-section, we propose schemes to cover different operating channel regimes of the network under study for the case of parallel fronthaul-edge transmission. Due to arguments of convexity in the DTB, it suffices to restrict the achievability to corner points \circled{$I_a$}, \circled{$I_b$}, \circled{$II_a$}, \circled{$II_b$} and \circled{$III$}. Remaining intermediate points in the tradeoff curves on the DTB are achievable through file splitting and time sharing of neighboring corner points (see Lemma \ref{lemma:1} for further details). In the following, we will first outline the main ingredients and assumptions of our scheme. This includes the \emph{large block number} assumption and a general signal vector structure that all schemes, irrespective of the channel regime, have in common.
%But before we describe the scheme in detail, we describe the main building blocks.
\vspace{0.5em}
\subsubsection*{Large Block Number}
\begin{figure*}[t]
  \centering
	\begin{tikzpicture}[scale=1]
			\ParBlockMod
	\end{tikzpicture}
\caption{Parallel Fronthaul-Edge Operation}
\label{fig:par_operation}
\end{figure*}  
We recall that in the case of parallel fronthaul-edge transmission, the HeNB operates as a causal \emph{full-duplex} relay endowed with additional cache capabilities. At any time instant $t$, $t=1,2,\ldots,T_P$, the HeNB is thus able to \emph{simultaneously} receive useful \emph{uncached} information through fronthauling and to transmit local information as a function of its its cached content and \emph{past} fronthaul messages from time instants $1,2,\ldots,t-1$. Our transmission scheme operates over $B$ blocks for which we use block-Markov coding. To this end, we split each file in the library into $B$ blocks, so that each block is of finite size $L^{'}=\nicefrac{L}{B}$ bits. We design our scheme in such a way that the wireless delivery time of each block is $T_B$ channel uses; or in other words, the achievable per-block DTB equals $\Delta_{\text{det},B}(\mu,n_F,\mathbf{n})=\nicefrac{T_B}{L^{\prime}}$. This DTB becomes feasible if the fronthaul transmission initiates and terminates by an offset of $T_O$ ($1\leq T_O\leq T_B$) channel uses prior to the wireless transmission (see Fig. \ref{fig:par_operation}). Thus, prior to any per-block wireless transmission just enough a-priori information on each block is made available through fronthauling. The total delivery time to provide both users with their requested files adds up to $T_P=BT_B+T_O$. Hence, the total delivery time per bit for finite $T_O$ that does not scale with $B$ is given by
\begin{equation}\label{eq:tot_DTB_par}
\Delta_{\text{det}}(\mu,n_F,\mathbf{n})=\limsup_{L\rightarrow\infty}\frac{T_P}{L}=\Delta_{\text{det},B}(\mu,n_F,\mathbf{n})+\lim_{B\rightarrow\infty}\frac{T_O}{BL^{\prime}}=\Delta_{\text{det},B}(\mu,n_F,\mathbf{n}).
\end{equation}
One can infer that for arbitrarily large number of blocks $B$, the offset duration $T_O$ becomes negligible and thus the overall DTB converges to the per-block DTB. In the remainder of this sub-section, we will make use of the large block observation and therefore present optimal achievability schemes for a single block that require a finite offset $T_O=1$. For that purpose, we now summarize the main transmit signal vector structure of eNB and HeNB that all block transmissions have in common.
\vspace{0.5em}
\subsubsection*{Building Blocks}
       
% Our achievable scheme deploys a block-Markov encoding scheme in which the HeNB simultaneously receives and transmits distinct fractions of requested file blocks. To this end, we split file into $B$ blocks, each block having a size $L^{'}=\nicefrac{L}{B}$ bits. We design our wireless transmission scheme in such a way that the wireless delivery time of each block is $T_B$ channel uses.   

Similar to sub-section \ref{subsec:ser_upp_bound}, we propose a general signal vector structure that all schemes have in common. Our scheme will use $T_B=2$ channel uses to transmit a single block of the requested file. It requires an offset of $T_O=1$ channel uses between fronthaul and wireless transmission. The general transmission structure for both eNB and HeNB is shown in Fig. \ref{fig:ldm_stack_par}. We note that the transmission structure of the HeNB remains unchanged (Fig. \ref{fig:ldm_stack} vs. Fig. \ref{fig:ldm_stack_par}), whereas the signal vector structure of the eNB is modified as follows:

\begin{figure}[t]
\begin{center}
		\LDMstacktwo
	\caption{Transmitted Signal Vector Structure at $t-$th Channel Use of length $q=\max\{n_{d1},n_{d2},n_{d3}\}$ at (H)eNB for the Parallel Fronthaul-Edge Transmission Setting ($b=1,2,\ldots,B$)}	
	\label{fig:ldm_stack_par}
	\end{center}
\end{figure}

For any block $b=1,\ldots,B$ ($T_O=1$) the eNB reserves fronthaul 
%two main type of resources:
\begin{enumerate}[label=(\alph*)]
\item capacity-\emph{dependent}
\item and capacity-\emph{independent}
\end{enumerate} resources. All resources are transmitted in $T_B=2$ channel instants $t_1=2b$ and $t_2=2b+1$. First type of resource includes private information
\begin{itemize}
\item[--]  $\mathbf{u}_{1,p}[t]$ and $\mathbf{u}_{2,p}[t]$ intended for $U_1$
\item[--] $\mathbf{v}_{1,p}[t]$ and $\mathbf{v}_{2,p}[t]$ intended for $U_2$;
\end{itemize}
all of which are conveyed to $U_1$ and $U_2$ in all two channel uses of a block. Latter resource type\footnote{We call this resource type fronthaul-edge block in Fig. \ref{fig:ldm_stack_par}.} comprises of private information 
\begin{itemize}
\item[--]  $\mathbf{u}_{\text{FE}}[t]$ intended for $U_1$
\item[--] and $\mathbf{v}_{\text{FE}}[t]$ intended for $U_2$
\end{itemize}
sent at the $t_1-$th and $t_2-$th channel use. The signal $\mathbf{w}_{\text{IN}}[t]$ is introduced to neutralize the interference of $\mathbf{v}_{\text{FE}}[t_1]$ and $\mathbf{v}_{\text{FE}}[t_2]$, partially, or even completely. We use the notation of sub-section \ref{subsec:ser_upp_bound} to denote the length of $\mathbf{u}_{i,p}[t]$, $i=1,\ldots,3$, and $\mathbf{v}_{j,p}[t]$, $j=1,2$. $R^{u}_{\text{FE}}[t_1],R^{u}_{\text{FE}}[t_2],R^{v}_{\text{FE}}[t_1]$ and $R^{v}_{\text{FE}}[t_2]$ indicate the rate of the fronthaul-edge block signals at time instant $t_1$ and $t_2$. As we will see, in comparison to $R_{j,p}^{u}[t]$ and $R_{j,p}^{v}[t]$, $j=1,2$, these rates depend on the fronthaul capacity $n_F$. 
% In the sequel, we focus on channel uses $t_1=2$ and $t_2=3$ for $b=1$ to simplify notation.  

The transmission according to the signal structure of Fig. \ref{fig:ldm_stack_par} requires that at the respective receivers interference-decoding and TIN is applied for each block in a successive manner. Hence, the \emph{per-block} achievable rates of $U_1$ and $U_2$ become
\begin{subequations}
\begin{alignat}{2}
R_{U_1}&=\sum_{t\in[t_1:t_2]}\Bigg(R_{\text{FE}}^{u}[t]+R_{\text{IN}}^{w}[t]+\sum_{i=1}^{3}R^{u}_{i,p}[t]\Bigg),\label{eq:ach_rate_U1_par}\\
R_{U_2}&=\sum_{t\in[t_1:t_2]}\Bigg(R_{\text{FE}}^{v}[t]+\sum_{j=1}^{2}R^{v}_{j,p}[t]\Bigg),\label{eq:ach_rate_U2_par}
\end{alignat}   
\end{subequations} respectively. For any block $b=1,\ldots,B$, the HeNB simultaenously receives \begin{equation}
\sum_{t\in[t_1:t_2]}n_F\label{eq:num_bits_HeNB_recept_block}
\end{equation} bits in fronthaul messages and transmits \begin{equation}
\sum_{t\in[t_1:t_2]}R_{3,p}^{u}[t]+R_{\text{IN}}^{w}[t]\label{eq:num_bits_HeNB_transmit_block}
\end{equation}
bits from the cached content and from parallel fronthauling. Thus, the difference between \eqref{eq:num_bits_HeNB_transmit_block} and \eqref{eq:num_bits_HeNB_recept_block} yields the number of cached bits per block which forces the fractional cache size to be \begin{equation}
\label{eq:frac_cache_size_par}
\mu^{\prime}_{\text{Ach}}(n_F,\mathbf{n})=\frac{\sum_{t\in[t_1:t_2]}\Big(R_{3,p}^{u}[t]+R_{\text{IN}}^{w}[t]-n_F\Big)}{R_{U_2}}.
\end{equation} The design parameters are the rate allocation parameters and the respective null vectors $\mathbf{0}_{l_k}$. For all channel regimes at given fractional cache size $\mu\in[0,1]$ and fronthaul capacity $n_{F}\in[0,n_{F,\max}(\mathbf{n})]$, we carefully choose the non-negative rate allocation parameters and the respective null vectors in such a way that  the achievable per-user rates for any block $b$ are identical, i.e.,
\begin{equation}
\label{eq:user_rate_1_and_2_par}
R_{U_1}\stackrel{!}{=}R_{U_2}\triangleq R_{U}\qquad\forall b=1,\ldots,B
\end{equation} and as large as possible while simultaenously equating the achievable fractional cache size with the given cache size $\mu$, i.e., \begin{equation}
\label{eq:cache_size_req_par}
\mu^{\prime}_{\text{Ach}}(n_F,\mathbf{n})\stackrel{!}{=}\mu.
\end{equation}
This design criterion ultimately results in identical delivery times to convey the requested files to $U_1$ and $U_2$ at a given cache size and fronthaul capacity. It is easy to infer that the achievable per-block DTB becomes $\Delta_{\text{det},B}(\mu=\mu^{\prime}_{\text{Ach}},n_F,\mathbf{n})=\nicefrac{T_B}{R_U}=\nicefrac{2}{R_U}$. We recall that for a large block size, $\Delta_{\text{det}}$ converges to $\Delta_{\text{det},B}$. 

%\begin{example}[Regime $\mathcal{R}_1$]\label{example_1}
%In this example, we consider the channel $\mathbf{n}=(2,5,4)^{T}\in\mathcal{R}_1$ for $n_{F}=0$. Theorem \ref{th:1} gives us the corner points \circled{$I_a$}$\:=\Big(\mu=0,\Delta_{\text{det}}^{*}(\mu=0,n_{F}=0,\mathbf{n})=\nicefrac{2}{5}\Big)$ and \circled{$II_b$}$\:=\Big(\mu^{\prime}=\nicefrac{1}{3},\Delta_{\text{det}}^{*}(\mu=\nicefrac{1}{3},n_{F}=0,\mathbf{n})=\nicefrac{1}{3}\Big)$.
%
%At extreme point \circled{$I_a$} neither fronthauling nor edge caching involving the HeNB is performed. Thus, the F-RAN under study reduces to a broadcast channel in which the eNB is responsible for transmitting the requested files while the HeNB remains silent. Thus, the only relevant channel realizations are $n_{d2}=5$ and $n_{d3}=4$. We observe that the stronger of those two channels is $n_{d2}=5$ ($n_{d3}\leq n_{d2}$). The optimal scheme equally distributes the transmission load of $n_{d2}=5$ bits to both users. That is, by sending $\nicefrac{n_{d2}}{2}=\nicefrac{5}{2}$ private information bits in a single channel use; or, alternatively by sending one bit in $\Delta_{\text{det}}^{*}(\mu=0,n_{F}=0,\mathbf{n})=\nicefrac{2}{5}$ channel uses, to $U_1$ and $U_2$, respectively. This scheme is feasible since the weaker channel $n_{d3}$ supports the transmission of $\nicefrac{n_{d2}}{2}$ bits ($\nicefrac{n_{d2}}{2}\leq n_{d3}$). These conditions are equivalent with $\mathbf{n}\in\mathcal{I}_0$. In summary, in the block representation this scheme is given by fixing the rate allocation parameters to $R_{2,p}^{u}=R_{p}^{v}=\nicefrac{n_{d2}}{2}=\nicefrac{5}{2}$, $l_2=n_{d2}=5$ and $R_{1,p}^{u}=R_{3,p}^{u}=R_{\text{IN}}^{w}=l_1=l_3=l_4=0$. We refer to the proof of Lemma \ref{lemma:2} and Remark \ref{remark_bc_conditions} for further details on this scheme.  
%
%The extreme point \circled{$II_b$} is achievable through cache-only transmission schemes in channel regimes $\mathbf{n}\in\mathcal{C}_1\supseteq\mathcal{R}_1$. It requires one channel use and achieves a DTB of $\nicefrac{2}{(n_{d1}+n_{d3})}=\nicefrac{1}{3}$ at fractional cache size $\mu^{\prime}(\mathbf{n})=\nicefrac{(2n_{d1}+2n_{d3}-2n_{d2})}{(n_{d1}+n_{d3})}=\nicefrac{1}{3}$. Fig. \ref{fig:AcScheme} illustrates the scheme for the case when $U_1$ and $U_2$ request $W_{d_1}=(a_1,a_2,a_3)$ and $W_{d_2}=(b_1,b_2,b_3)$, respectively. In this case where the channel of the cross link $n_{d2}$ is the strongest, it is advantageous that the eNB transmits not only private information to $U_2$ but also to $U_1$. This implies that the rates $R_{1,p}^{u}, R_{2,p}^{u}$ are chosen to be non-zero whereas $l_1=0$. From the perspective of $U_2$, the optimal DTB of $\nicefrac{1}{3}$ is then only achievable if we fix $R_{p}^{v}=\nicefrac{(n_{d1}+n_{d3})}{2}=3$ in order to convey bits $b_1,b_2$ and $b_3$. Note that the eNB-$U_2$ link is capable of reliably carrying $R_{p}^{v}=3$ bits to $U_2$ because $R_{p}^{v}=3<n_{d3}=4$ holds in $\mathcal{C}_1$. The unused signal levels at the eNB of rate $R_{1,p}^{u}=\nicefrac{(n_{d3}-n_{d1})}{2}=1$ and $R_{2,p}^{u}=n_{d2}-n_{d3}=1$ are allocated to send private information $a_1$ and $a_3$ to $U_1$.  To retrieve the remaining desired bit of $U_1$ ($a_2$), the interfering bit $b_3$ of $\mathbf{v}_{p}$ is neutralized by sending the single XOR combination ($R_{\text{IN}}^{w}=n_{d1}+n_{d3}-n_{d2}=1$) $a_2\oplus b_3$ at the \emph{highest} signal level of the HeNB. Therefore, the HeNB retains $a_2$ and $b_3$ in its cache during the placement phase. This constitutes a fractional cache size $\mu^{\prime}(\mathbf{n})=\nicefrac{1}{3}$. With this strategy, $U_1$ receives $R_{1,p}^{u}+R_{2,p}^{u}=\nicefrac{(2n_{d2}-n_{d1}-n_{d3})}{2}=2$ bits ($a_1$ and $a_3$) of $W_{d_1}$ from the eNB while the remaining $R_{\text{IN}}^{w}=n_{d1}+n_{d3}-n_{d2}=1$ bits ($a_2$) are received through network coding which involves both HeNB and eNB. Sending additional private information from the HeNB would not increase the achievable rate of $U_2$ any further. For that reason, $R_{3,p}^{u}=l_3=0$ and $l_2=4$. When generalizing the scheme, it is easy to see that the scheme is feasible for arbitrary $\mathbf{n}\in\mathcal{C}_1$. If the achievable per-user rate is a non-integer, two channel uses are required. For further details on this case, we point to our previous work \cite{prev_work}.    
%
%Any point between the two corner points \circled{$I_a$} and \circled{$II_b$} is achieved through file splitting and time sharing between the policies at those two corner points. Such scheme is often termed \emph{memory sharing}. As the transmission at \circled{$I_a$} and \circled{$II_b$} are feasible in $\mathcal{R}_{\text{\circled{$I_a$}}}=\mathcal{I}_0$ and $\mathcal{R}_{\text{\circled{$II_b$}}}=\mathcal{C}_1$, any intermediate point in the memory-latency tradeoff curve is achievable through memory sharing in the channel regime $\mathcal{R}_{1}\triangleq\mathcal{R}_{\text{\circled{$II_b$}}}
%\cap\mathcal{R}_{\text{\circled{$I_a$}}}=\mathcal{C}_1\cap\mathcal{I}_0$. In this particular channel regime, we notice that $\mathcal{R}_{1}=\mathcal{C}_1$ because $\mathcal{C}_1\cap\mathcal{I}_0^{C}=\emptyset$. However, this is not true for all channel regimes under study.  
%\end{example}
%\vspace{0.5em}
In the remainder of sub-section \ref{subsec:par_upp_bound}, we will show the achievability of all relevant corner points. To this end, we specify the rate allocation parameters introduced as part of the generalized signal block structure (see Fig. \ref{fig:ldm_stack_par}).
\begin{table}[h]
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$I_a$} at fractional cache size $\mu^{\prime}=0$ for $n_{F}\in[0,n_{d1}]$ in channel regimes $\mathcal{C}_{1},\mathcal{R}_{2}$ and $\mathcal{R}_{3}$}
\label{tab:rate_alloc_I_a_R1_R3}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
Regime & \multicolumn{2}{c|}{$\mathcal{C}_1$} & \multicolumn{2}{c|}{$\mathcal{R}_2$} & \multicolumn{2}{c|}{$\mathcal{R}_3$}
\\ \hline
Time $t$ & $t_1$ & $t_2$ & $t_1$ & $t_2$ & $t_1$ & $t_2$ 
\\ \hline
$R_{3,p}^{u}$ &  \multicolumn{6}{c|}{$0$} 
\\ \hline
$R_{2,p}^{u}$  & $n_{d3}-n_{d1}$ & \multicolumn{5}{c|}{$0$}
\\ \hline
$R_{1,p}^{u}$  &  \multicolumn{6}{c|}{$n_{d2}-n_{d3}$} 
\\ \hline
%$R_{\text{FE}}^{u}$ & $n_{d1}+n_{d3}-n_{d2}-n_{F}$ & $0$ & $2n_{d3}-n_{d2}-n_{F}$ & $0$ & $2n_{d3}-n_{d2}-n_{F}$ & $0$
%\\ \hline
$R_{\text{FE}}^{u}$ & $\big(n_{F,\max}(\mathbf{n})-n_{F}\big)^{+}$ & $0$ & $\big(n_{F,\max}(\mathbf{n})-n_{F}\big)^{+}$ & $0$ & $\big(n_{F,\max}(\mathbf{n})-n_{F}\big)^{+}$ & $0$
\\ \hline
$R_{\text{IN}}^{w}$ & \multicolumn{6}{c|}{$\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$}
\\ \hline
$R_{\text{FE}}^{v}$  & $\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$  & $n_{F,\max}(\mathbf{n})$ & $\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$  & $n_{F,\max}(\mathbf{n})$ & $\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$ & $n_{F,\max}(\mathbf{n})$
\\ \hline
$R_{2,p}^{v}$ & $n_{d2}-n_{d3}$ & $n_{d2}-n_{d1}$ &  \multicolumn{4}{c|}{$n_{d2}-n_{d3}$}  
\\ \hline
$R_{1,p}^{v}$ & \multicolumn{6}{c|}{$0$}
\\ \hline
$l_4$ & \multicolumn{6}{c|}{$0$}
\\ \hline
$l_3$ &  \multicolumn{2}{c|}{$\big(n_{F,\max}(\mathbf{n})-n_{F}\big)^{+}$} & \multicolumn{4}{c|}{$\max\big\{n_{d1}+n_{d3}-n_{d2}-n_{F},n_{d1}-n_{d3}\big\}$}
\\ \hline
$l_2$  &  \multicolumn{4}{c|}{$2n_{d2}-n_{d1}-n_{d3}$} &  \multicolumn{2}{c|}{$n_{d2}-n_{d3}$}   
\\ \hline
$l_1$ &  \multicolumn{4}{c|}{$0$} &  \multicolumn{2}{c|}{$n_{d1}-n_{d2}$} 
\\ \hline 
\hline
$n_{F,\max}(\mathbf{n})$ & \multicolumn{2}{c|}{$n_{d1}+n_{d3}-n_{d2}$} & \multicolumn{4}{c|}{$2n_{d3}-n_{d2}$} \\ \hline
\end{tabular}
\end{table}
\begin{table}[h]
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$I_a$} at fractional cache size $\mu^{\prime}=0$ for $n_{F}\in[0,n_{d1}]$ in channel regimes $\mathcal{R}_{51}$ and $\mathcal{C}_{52}$}
\label{tab:rate_alloc_I_a_R51_R52}
\begin{tabular}{|c||c|c|c|c|}
\hline
Regime & \multicolumn{2}{c|}{$\mathcal{R}_{51}$} & \multicolumn{2}{c|}{$\mathcal{C}_{52}$} 
\\ \hline
Time $t$ & $t_1$ & $t_2$ & $t_1$ & $t_2$ 
\\ \hline
$R_{3,p}^{u}$ &  \multicolumn{4}{c|}{$0$}
\\ \hline
$R_{2,p}^{u}$  & \multicolumn{3}{c|}{$n_{d3}-n_{d2}$} & $n_{d2}-n_{d1}$
\\ \hline
$R_{1,p}^{u}$  &  \multicolumn{4}{c|}{$0$}
\\ \hline
$R_{\text{FE}}^{u}$ & $\big(n_{F,\max}(\mathbf{n})-n_{F}\big)^{+}$ & $0$ & $\big(n_{F,\max}(\mathbf{n})-n_{F}\big)^{+}$ & $0$
\\ \hline
$R_{\text{IN}}^{w}$ & \multicolumn{4}{c|}{$\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$}
\\ \hline
$R_{\text{FE}}^{v}$  & $\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$  & $n_{F,\max}(\mathbf{n})$ & $\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$  & $n_{F,\max}(\mathbf{n})$ 
\\ \hline
$R_{2,p}^{v}$ & \multicolumn{2}{c|}{$0$} & $2n_{d2}-n_{d1}-n_{d3}$ & $0$  
\\ \hline
$R_{1,p}^{v}$ & \multicolumn{4}{c|}{$n_{d3}-n_{d2}$}
\\ \hline
$l_4$ & \multicolumn{4}{c|}{$0$}
\\ \hline
$l_3$ &  \multicolumn{2}{c|}{$\max\big\{n_{d1}-n_{F},n_{d1}-n_{F,\max}(\mathbf{n})\big\}$} & \multicolumn{2}{c|}{$\big(n_{d1}-n_{F}\big)^{+}$}
\\ \hline
$l_2$  &  \multicolumn{4}{c|}{$n_{d3}-n_{d1}$} 
\\ \hline
$l_1$ &  \multicolumn{4}{c|}{$0$} 
\\ \hline 
\hline
$n_{F,\max}(\mathbf{n})$ & \multicolumn{2}{c|}{$2n_{d2}-n_{d3}$} & \multicolumn{2}{c|}{$n_{d1}$}
\\ \hline
\end{tabular}
\end{table}
\newcolumntype{C}{>{\centering\arraybackslash}p{11.0em}}
\begin{table}[h]
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$I_a$} at fractional cache size $\mu^{\prime}=0$ for $n_{F}\in[(n_{d3}-2n_{d2})^{+},n_{d1}]$ in channel regimes $\mathcal{C}_{4}$ and $\mathcal{C}_{61}$}
\label{tab:rate_alloc_I_a_R4_R62}
\begin{tabular}{|c||C|C|C|C|}
\hline
Regime & \multicolumn{2}{c|}{$\mathcal{C}_{4}$} & \multicolumn{2}{c|}{$\mathcal{C}_{61}$} 
\\ \hline
Time $t$ & $t_1$ & $t_2$ & $t_1$ & $t_2$ 
\\ \hline
$R_{3,p}^{u}$ & $\min\{n_{F,\max}(\mathbf{n})-n_{d2},n_{F}\}$ & $\min\Big\{\big(\max\{n_{d3}-2n_{d2},n_F-n_{d2}\}\big)^{+},n_{F,\max}(\mathbf{n})-n_{d2}\Big\}$ &  $\min\{n_{F},n_{d1}-n_{d2}\}$ & $\min\Big\{\big(\max\{n_{d3}-2n_{d2},n_F-n_{d1}-n_{d2}+n_{d3}\}\big)^{+},n_{d1}-n_{d2}\Big\}$
 \\ \hline
$R_{2,p}^{u}$  & \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$0$}
\\ \hline
$R_{1,p}^{u}$  & \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$0$}
\\ \hline
$R_{\text{FE}}^{u}$ & $\min\big\{n_{d2},\big(n_{F,\max}(\mathbf{n})-n_{F}\big)^{+}\big\}$ & $\big(n_{F,\max}(\mathbf{n})-n_{d2}-n_{F}\big)^{+}$ & $\min\big\{n_{d2},\max\{n_{d1}-n_{F},n_{d1}-n_{F,\max}(\mathbf{n})\}\big\}$ & $\max\{n_{d3}-n_{d2}-n_{F},n_{d3}-n_{d1}\}$ 
\\ \hline
$R_{\text{IN}}^{w}$ & $\big(\min\{n_{d2}+n_F-n_{F,\max}(\mathbf{n}),n_{d2}\}\big)^{+}$ & $\min\{2n_{d2}-n_{d3}+n_{F},n_{d2},n_{F}\}$ & $\big(\min\{n_{d2}+n_F-n_{d1},n_{d2}+n_{F,\max}(\mathbf{n})-n_{d1}\}\big)^{+}$ & $\min\{2n_{d2}-n_{d3}+n_{F},n_{d1}+n_{d2}-n_{d3},n_{F}\}$
\\ \hline
$R_{\text{FE}}^{v}$  & $\max\big\{n_{d3}-n_{d2},\min\{n_{F},n_{F,\max}(\mathbf{n})\}\big\}$ & $\min\{n_{d2}+n_{F},n_{F,\max}(\mathbf{n})\}$ & $\max\big\{n_{d1}-n_{d2},\min\{n_{F},n_{F,\max}(\mathbf{n})\}\big\}$ & $\min\big\{2n_{d2}-n_{d3}+n_{F},n_{d1}+n_{d2}-n_{d3}\big\}$
\\ \hline
$R_{2,p}^{v}$ & \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$0$}
\\ \hline
$R_{1,p}^{v}$ & \multicolumn{2}{c|}{$0$} & $n_{d3}-n_{d1}$ & $n_{d3}-n_{d2}$ 
\\ \hline
$l_4$ & $\max\{n_{d1}-n_{d3},n_{d1}-n_{d2}-n_{F}\}$ & $\max\big\{\min\big\{n_{d1}+n_{d2}-n_{d3},n_{d1}-n_F,n_{d1}-n_{d2}\big\},n_{d1}-n_{F,\max}(\mathbf{n})\big\}$ & $\big(n_{d1}-n_{d2}-n_F\big)^{+}$ & $\big(\min\{n_{d1}+n_{d2}-n_{d3},n_{F,\max}(\mathbf{n})-n_{F},n_{d1}-n_{d2}\}\big)^{+}$
\\ \hline
$l_3$ & $\min\{n_{d2},(n_{F,\max}(\mathbf{n})-n_{F})^{+}\}$ & $\big(\max\{n_{d3}-n_{d2}-n_{F},n_{d2}-n_{F}\}\big)^{+}$ & $\min\big\{n_{d2},\max\{n_{d1}-n_{F},n_{d1}-n_{F,\max}(\mathbf{n})\}\big\}$ & $\max\{n_{d3}-n_{d2}-n_{F},n_{d3}-n_{d1},n_{d2}-n_{F}\}$
\\ \hline
$l_2$  & \multicolumn{2}{c|}{$0$} & \multicolumn{2}{c|}{$n_{d3}-n_{d1}$}
\\ \hline
$l_1$ & \multicolumn{2}{c|}{$n_{d1}-n_{d3}$} & \multicolumn{2}{c|}{$0$}
\\ \hline \hline
$n_{F,\max}(\mathbf{n})$ & \multicolumn{2}{c|}{$n_{d3}$} & \multicolumn{2}{c|}{$2n_{d1}-n_{d3}$}
\\ \hline
\end{tabular}
\end{table}
\vspace{0.5em}
\subsubsection*{Scheme for Corner Point \circled{$I_a$}}
The transmission scheme uses the generalized block structure of Fig. \ref{fig:ldm_stack_par} to convey each receiver with its requested file. At this particular corner point, the HeNB does not have any caching capability ($\mu^{\prime}_{\text{Ach}}=0$). In fact, it retrieves information on the requested files \emph{only} through the cloud-to-HeNB fronthaul link. Thus, the HeNB for this case functions as a standard full-duplex relay being capable of performing standard relaying techniques. In our scheme, the HeNB applies the relaying strategy decode-and-forward (DF) to encode signals $\mathbf{u}_{3,p}[t]$ and $\mathbf{w}_{\text{IN}}[t]$ at the $t-$th channel use from its received fronthaul signal $\mathbf{x}_{F}[t-1]$ at time instant $t-1$. More specifically, at channel use $t-1$ the cloud provides the HeNB with the signals $\mathbf{u}_{3,p}[t]$ and $\mathbf{w}_{\text{IN}}[t]$ that it will transmit to $U_1$ one channel use later at time $t$. Thus, we carefully choose the rate parameters $R_{3,p}^{u}[t]$ and $R_{\text{IN}}^{w}[t]$ for fixed fronthaul capacity $n_F\in[0,n_{F,\max}(\mathbf{n})]$ such that reliable fronthauling and wireless transmission of $\mathbf{u}_{3,p}[t]$ and $\mathbf{w}_{\text{IN}}[t]$ at time instants $t-1$ and $t$ are feasible, i.e.,  
\begin{equation}
\label{eq:rate_HeNB_mu_0}
n_{F}=R_{3,p}^{u}[t]+R_{\text{IN}}^{w}[t]\leq n_{F,\max}(\mathbf{n}) \leq n_{d1}\qquad\forall t\in[t_1:t_2],\:b=1,\ldots,B.
\end{equation} 
%\begin{equation}
%\label{eq:rate_HeNB_mu_0}
%n_{F}=R_{3,p}^{u}[t]+R_{\text{IN}}^{w}[t]\leq n_{F,\max}(\mathbf{n}) \leq n_{d1}\qquad\forall t\in[1:T_P].
%\end{equation} 
We note that condition \eqref{eq:rate_HeNB_mu_0} is in agreement with Equation \eqref{eq:frac_cache_size_par}. In order to fulfill \eqref{eq:user_rate_1_and_2_par}, we choose the remaining rate allocation parameters such that the per-block achievable rates of both users at time instants $t_1$ and $t_2$, $\forall b$, satisfy
\begin{subequations}
\label{eq:rates_t1_t2}
\begin{alignat}{2}
R_{U_1}[t_1]&=R_{U_2}[t_2],\label{eq:ach_rate_users_t1_t2_1}\\ R_{U_1}[t_2]&=R_{U_2}[t_1],\label{eq:ach_rate_users_t1_t2_2}
\end{alignat}
\end{subequations} while the overall rate adds up to 
\begin{equation}
\label{eq:overall_ach_rate_block}
R_{U}=n_{F}+\max\{n_{d2},n_{d3}\}.
\end{equation} Tables \ref{tab:rate_alloc_I_a_R1_R3}--\ref{tab:rate_alloc_I_a_R4_R62} specify the optimal rate allocation parameters for all channel regimes of Theorem \ref{th:5} with fronthaul capacity $n_{F}\in[0,n_{d1}]$. These parameters meet conditions \eqref{eq:rate_HeNB_mu_0},\eqref{eq:rates_t1_t2} and \eqref{eq:overall_ach_rate_block}. On closer inspection of these tables, one can verify that for $n_{F}=n_{F,\max}(\mathbf{n})$ the user rates become
\begin{equation}
\label{eq:behavior_nF_eq_nF_max}
R_{U_k}[t_i]=\nicefrac{1}{\Delta_{\text{LB}}^{\prime}(\mathbf{n})},\qquad i=k=\{1,2\}\quad \forall b,
\end{equation} which constitutes an overall DTB of $\Delta_{\text{det}}(\mu=0,n_{F}=n_{F,\max}(\mathbf{n}),\mathbf{n})=\Delta_{\text{LB}}^{\prime}(\mathbf{n})$ under the large block number assumption. This is the lowest attainable DTB. Increasing the systems fronthaul capacities in the range $n_{F}\in[n_{F,\max}(\mathbf{n}),n_{d1}]$ will therefore not reduce the DTB any further (see Tables \ref{tab:rate_alloc_I_a_R1_R3}--\ref{tab:rate_alloc_I_a_R4_R62}).    
\vspace{0.5em}
\subsubsection*{Scheme for Corner Point \circled{$I_b$}}
The optimal scheme at corner point \circled{$I_b$} is using the signal vector structure specified in Fig. \ref{fig:ldm_stack_par}. The rate allocation that attain the optimal DTB is given in Table \ref{tab:rate_alloc_I_b_R4_R61_prime_C62}.  
\begin{table}[h]
\centering
\caption{Rate allocation parameters for corner point \protect\circled{$I_b$} at fractional cache size $\mu^{\prime}=0$ for $n_{F}\in[0,n_{d1}]$ in channel regimes $\mathcal{R}_4^{\prime},\mathcal{R}_{61}^{\prime}$ and $\mathcal{C}_{62}^{\prime}$}
\label{tab:rate_alloc_I_b_R4_R61_prime_C62}
\begin{tabular}{|c||c|c|c|}
\hline
Regime & \multicolumn{1}{c|}{$\mathcal{R}_4^{\prime}$} & \multicolumn{1}{c|}{$\mathcal{R}_{61}^{\prime}$} & \multicolumn{1}{c|}{$\mathcal{C}_{62}$}
\\ \hline
Time $t$ & $t_1,t_2$ & $t_1,t_2$ & $t_1,t_2$ 
\\ \hline
$R_{3,p}^{u}$ &  \multicolumn{3}{c|}{$\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$} 
\\ \hline
$R_{2,p}^{u}$  & \multicolumn{3}{c|}{$n_{d2}$}
\\ \hline
$R_{1,p}^{u}$  &  \multicolumn{3}{c|}{$0$} 
\\ \hline
$R_{\text{FE}}^{u}$ & \multicolumn{3}{c|}{$0$}
\\ \hline
$R_{\text{IN}}^{w}$ & \multicolumn{3}{c|}{$0$}
\\ \hline
$R_{\text{FE}}^{v}$  & \multicolumn{3}{c|}{$\min\big\{n_F,n_{F,\max}(\mathbf{n})\big\}$}
\\ \hline
$R_{2,p}^{v}$ & \multicolumn{3}{c|}{$0$} 
\\ \hline
$R_{1,p}^{v}$ & \multicolumn{3}{c|}{$n_{d2}$}
\\ \hline
$l_4$ & \multicolumn{2}{c|}{$\max\big\{n_{d1}-n_{d2}-n_F,n_{d1}+n_{d2}-n_{d3}\big\}$} & \multicolumn{1}{c|}{$\big(n_{F,\max}(\mathbf{n})-n_F\big)^{+}$}
\\ \hline
$l_3$ &  \multicolumn{1}{c|}{$n_{d2}$} & \multicolumn{2}{c|}{$n_{d2}+n_{d3}-n_{d1}$}
\\ \hline
$l_2$  & \multicolumn{3}{c|}{$0$}   
\\ \hline
$l_1$ &  \multicolumn{1}{c|}{$\max\big\{n_{d1}-2n_{d2}-n_F,n_{d1}-n_{d3}\big\}$} & \multicolumn{1}{c|}{$\big(n_{F,\max}(\mathbf{n})-n_F\big)^{+}$} & \multicolumn{1}{c|}{$\max\big\{n_{d3}-2n_{d2}-n_{F},n_{d3}-n_{d1}-n_{d2}\}$} 
\\ \hline 
\hline
$n_{F,\max}(\mathbf{n})$ & \multicolumn{2}{c|}{$n_{d3}-2n_{d2}$} & \multicolumn{1}{c|}{$n_{d1}-n_{d2}$} \\ \hline
\end{tabular}
\end{table}
\vspace{0.5em}
\subsubsection*{Scheme for Corner Points \circled{$II_a$}, \circled{$II_b$} and \circled{$III$}}  
The schemes for these three corner points are directly deducible from schemes for corner points \circled{$II_{a,S}$}, \circled{$II_{b,S}$} and \circled{$III_{S}$} of the serial fronthaul-edge transmission (see sub-section \ref{subsec:ser_upp_bound}). In this paragraph, we use the indices $S$ and $P$ to distinguish corner points of serial transmissions from those for parallel transmissions. Through careful comparison of Theorems \ref{th:1}--\ref{th:3} with \ref{th:5}--\ref{th:7}, one can verify that \begin{subequations}
\label{eq:mu_par_vs_mu_ser}
\begin{alignat}{3}
\mu_{S}^{\prime}(\mathbf{n})L&=\mu_{P}^{\prime}(n_F,\mathbf{n})L+n_{F},\label{eq:mu_par_vs_mu_ser_1}\\ \mu_{S}^{\prime\prime}(\mathbf{n})L&=\mu_{P}^{\prime\prime}(n_F,\mathbf{n})L+n_{F},\label{eq:mu_par_vs_mu_ser_2} \\ \mu_{S}^{\prime\prime\prime}(\mathbf{n})L&=\mu_{P}^{\prime\prime\prime}(n_F,\mathbf{n})L+n_{F}.\label{eq:mu_par_vs_mu_ser_3}
\end{alignat}
\end{subequations}
These equations suggest that the HeNB's cached content at corner points \circled{$II_{a,S}$}, \circled{$II_{b,S}$} and \circled{$III_{S}$} are separable into two distinct components attributed to edge caching and fronthauling for the case of parallel transmission. 

In the following, we explicitly account for the cache separability and propose how to map the achievability scheme of serial to parallel fronthaul-edge transmission. The mapping is done as follows:

We keep the signal structure for both cases identical, i.e.,  
\begin{subequations}
\label{eq:decomposing_signals}
\begin{alignat}{3}
\mathbf{u}_{i,p}^{P}[t]&=\mathbf{u}_{i,p}^{S},\qquad i=1,\ldots,3,\label{eq:decomposing_signals_1}\\ \mathbf{v}_{1,p}^{P}[t]&=\mathbf{v}_{p}^{S},\label{eq:decomposing_signals_2} \\ \mathbf{w}_{\text{IN }}^{P}[t]&=\mathbf{w}_{\text{IN }}^{S},\label{eq:decomposing_signals_3}
\end{alignat}
\end{subequations} for $t=[t_1:t_2],\forall b$. These equalities are tantamount to identical rate allocation. Thus, the rates of the remaining signal vectors of the generalized block structure in Fig. \ref{fig:ldm_stack_par}, the fronthaul-edge transmission block and $\mathbf{v}_{2,p}^{P}[t]$, are set to $0$. To account for the separability of the HeNB's cached of serial transmission according to \eqref{eq:mu_par_vs_mu_ser}, we decompose signals $\mathbf{u}_{3,p}[t]$ and $\mathbf{w}_{\text{IN}}[t]$ for the parallel transmission case into sub-signals attributed to edge caching and fronthauling (indices $C$ and $F$) according to
\begin{subequations}
\label{eq:decomposing}
\begin{alignat}{2}
\mathbf{u}_{3,p}[t]&=\Big(\mathbf{u}_{3,p}^{C}[t]),\mathbf{u}_{3,p}^{F}[t]\Big)^{T},\label{eq:decomposing_1}\\ \mathbf{w}_{\text{IN}}[t]&=\Big(\mathbf{w}_{\text{IN}}^{C}[t],\mathbf{w}_{\text{IN}}^{F}[t]\Big)^{T},\label{eq:decomposing_2}
\end{alignat}
\end{subequations} with rate allocation 
\begin{subequations}
\label{eq:decomposing_rate}
\begin{alignat}{2}
R_{3,p}^{F}[t]+R_{\text{IN}}^{F}[t]&=n_{F},
\label{eq:decomposing_rate_1}\\ R_{3,p}^{C}[t]+R_{\text{IN}}^{C}[t]&=\begin{cases}\mu_{P}^{\prime}(n_{F},\mathbf{n})L=\mu_{S}^{\prime}(\mathbf{n})L-n_F\quad&\text{ at \circled{$II_b$}}\\\mu_{P}^{\prime\prime}(n_{F},\mathbf{n})L=\mu_{S}^{\prime\prime}(\mathbf{n})L-n_F\quad&\text{ at \circled{$II_a$}}\\\mu_{P}^{\prime\prime\prime}(n_{F},\mathbf{n})L=\mu_{S}^{\prime\prime\prime}(\mathbf{n})L-n_F\quad&\text{ at \circled{$III$}} \end{cases},\label{eq:decomposing_rate_2}
\end{alignat}
\end{subequations} for $t=[t_1:t_2],\forall b$, and
\begin{equation}\label{eq:nF_max_corner_points_II_III}
n_{F}\leq\begin{cases}\mu_{S}^{\prime}(\mathbf{n})L\quad&\text{ at \circled{$II_b$}}\\\mu_{S}^{\prime\prime}(\mathbf{n})L\quad&\text{ at \circled{$II_a$}}\\\mu_{S}^{\prime\prime\prime}(\mathbf{n})L\quad&\text{ at \circled{$III$}}\end{cases}.
\end{equation} This concludes the achievability at these points for the case of parallel transmission. 

%Thus, the required number of cached bits for parallel transmission reduces by $n_F$ bits through fronthaul.
%Thus, the rate allocation parameters of parallel and serial transmission are identical except of fixing  
%We can therefore map the achievability scheme of serial to parallel fronthaul-edge transmission. The mapping is done by setting the rate allocation parameters of the parallel transmission    
% 




==> content/tikz_ldm.tex <==
%\input{tikzheader}

%name number of pipes; position (x,y);
\newcommand{\ldmnewuser}[3]{
\begin{scope}[pipedot/.style={draw, circle, inner sep=0pt, minimum size=0.3cm}]
\def\username{#1}
\def\numPipes{#2}
\def\distanceDots{0.6}
\coordinate (position\username) at #3;

\foreach \x in {1,...,\numPipes} {
	\pgfmathparse{-(\x-1)*\distanceDots}
	\node[pipedot] (node\x\username) at ($(0, \pgfmathresult)+(position\username)$) {};
}
\node[draw,fit=(node1\username) (node\numPipes\username)] (group\username) {};
\end{scope}
} 

%name of user1, name of user2, no of pipes, shifted levels 
\newcommand{\ldmconnectusers}[4]{
\foreach \x in {1,...,#3} {
	\pgfmathtruncatemacro\mymacro{(\x+#4)}
	\draw[->, thick] (node\x #1)--(node\mymacro #2) ;
}
} 



%\begin{document}

\begin{tikzpicture}

%\ldmnewuser{Alice}{6}{(0,0)}
\ldmnewuser{HeNB}{4}{(0,0)}
%\node[node distance=0.1cm, above=of groupAlice] {Alice};
\node[node distance=0.1cm, above=of groupHeNB] {HeNB};
%\node[node distance=0.2cm, left=of node1Alice] {$a\otimes b$};
\node[node distance=0.2cm, left=of node1HeNB] {$a_1\oplus b_3$};
% \node[node distance=0.2cm, left=of node2Alice] {$a\otimes b\otimes b$};

\ldmnewuser{eNB}{4}{(0,-5)}
\node[node distance=0.1cm, above=of groupeNB] {eNB};
\node[node distance=0.2cm, left=of node1eNB] {$b_1$};
\node[node distance=0.2cm, left=of node2eNB] {$b_2$};
\node[node distance=0.2cm, left=of node3eNB] {$b_3$};
\node[node distance=0.2cm, left=of node4eNB] {$a_2$};

%\ldmnewuser{Bob}{6}{(5,0)}
\ldmnewuser{fU}{4}{(5,0)}
%\node[node distance=0.1cm, above=of groupBob] {Bob};
\node[node distance=0.1cm, above=of groupfU] {$U_1$};
\node[node distance=0.2cm, right=of node3fU] {$a_1$};
\node[node distance=0.2cm, right=of node4fU] {$a_2$};

%\ldmnewuser{Eve}{6}{(5,-5)}
\ldmnewuser{sU}{4}{(5,-5)}
%\node[node distance=0.1cm, above=of groupEve] {Eve};
\node[node distance=0.1cm, above=of groupsU] {$U_2$};
\node[node distance=0.2cm, right=of node2sU] {$b_1$};
\node[node distance=0.2cm, right=of node3sU] {$b_2$};
\node[node distance=0.2cm, right=of node4sU] {$b_3$};

% Connect Tx and Rx

%\ldmconnectusers{Alice}{Bob}{4}{1}
\ldmconnectusers{HeNB}{fU}{1}{2}
%\ldmconnectusers{Alice}{Eve}{2}{3}
\ldmconnectusers{eNB}{fU}{4}{0}
\ldmconnectusers{eNB}{sU}{3}{1}

% Coloring and marking specific areas
\node[right=of node3sU.south, yshift=-0.2cm, xshift=12pt] (sU1) {}; 
\node[right=of node2sU.north, yshift=0.2cm, xshift=12pt] (sU2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(sU1) -- (sU2) node [black,midway,xshift=8pt] {$n_{d2}-n_{d1}$};
\node[right=of node3fU.south, yshift=-0.2cm, xshift=12pt] (fU1) {}; 
\node[right=of node3fU.north, yshift=0.2cm, xshift=12pt] (fU2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU1) -- (fU2) node [black,midway,xshift=20pt] {$n_{d1}+n_{d3}-n_{d2}$};
\node[right=of node4fU.south, yshift=-0.2cm, xshift=12pt] (fU3) {}; 
\node[right=of node4fU.north, yshift=0.2cm, xshift=12pt] (fU4) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU3) -- (fU4) node [black,midway,xshift=6pt] {$n_{d2}-n_{d3}$};

\begin{scope}[on background layer]
%\node[fill=blue!10,fit=(node1fU) (node2fU)] (groupfUd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node1HeNB) (node1HeNB)] (groupHeNBd1) {};
\node[pattern=horizontal lines, pattern color=red!80,fit=(node1HeNB) (node1HeNB)] (groupHeNBd2) {};
\node[pattern=north west lines, pattern color=black,fit=(node1eNB) (node2eNB)] (groupeNBd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node3eNB) (node3eNB)] (groupeNBd3) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node4eNB) (node4eNB)] (groupeNBd3) {};
\node[pattern=north west lines, pattern color=black,fit=(node1fU) (node2fU)] (groupfUd1) {};
\node[pattern=horizontal lines, pattern color=red!80,fit=(node3fU) (node3fU)] (groupfUd3) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node4fU) (node4fU)] (groupfUd3) {};
\node[pattern=north west lines, pattern color=black,fit=(node2sU) (node3sU)] (groupsUd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node4sU) (node4sU)] (groupsUd3) {};
%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
\end{scope}


%\node[right=of node5Bob.south, yshift=-0.2cm] (bobcurly1) {}; 
%\node[right=of node2Bob.north, yshift=0.2cm] (bobcurly2) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(bobcurly1) -- (bobcurly2) node [black,midway] {$n_1$};
%
%\node[right=of node5Eve.south, yshift=-0.2cm] (evecurly1) {}; 
%\node[right=of node4Eve.north, yshift=0.2cm] (evecurly2) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(evecurly1) -- (evecurly2) node [black,midway] {$n_2$};
%
%\node[right=of node3Eve.south, yshift=-0.2cm] (evecurly3) {}; 
%\node[right=of node2Eve.north, yshift=0.2cm] (evecurly4) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(evecurly3) -- (evecurly4) node [black,midway,xshift=0.4cm] {$n_1-n_2$};
%
%
%
%\begin{scope}[on background layer]
%\node[fill=blue!10,fit=(node2Bob) (node5Bob)] (groupBobn1) {};
%\node[fill=blue!50,fit=(node2Eve) (node3Eve)] (groupEven1n2) {};
%%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
%\end{scope}


%\draw[->,red] (node5Bob.south)--(node1Eve.north) ;
\end{tikzpicture}

\begin{tikzpicture}

%\ldmnewuser{Alice}{6}{(0,0)}
\ldmnewuser{HeNB}{4}{(0,0)}
%\node[node distance=0.1cm, above=of groupAlice] {Alice};
\node[node distance=0.1cm, above=of groupHeNB] {HeNB};
%\node[node distance=0.2cm, left=of node1Alice] {$a\otimes b$};
\node[node distance=0.2cm, left=of node1HeNB] {$a_4\oplus b_5$};
% \node[node distance=0.2cm, left=of node2Alice] {$a\otimes b\otimes b$};

\ldmnewuser{eNB}{4}{(0,-5)}
\node[node distance=0.1cm, above=of groupeNB] {eNB};
\node[node distance=0.2cm, left=of node1eNB] {$b_4$};
\node[node distance=0.2cm, left=of node2eNB] {$a_3$};
\node[node distance=0.2cm, left=of node3eNB] {$b_5$};
\node[node distance=0.2cm, left=of node4eNB] {$a_5$};

%\ldmnewuser{Bob}{6}{(5,0)}
\ldmnewuser{fU}{4}{(5,0)}
%\node[node distance=0.1cm, above=of groupBob] {Bob};
\node[node distance=0.1cm, above=of groupfU] {$U_1$};
\node[node distance=0.2cm, right=of node2fU] {$a_3$};
\node[node distance=0.2cm, right=of node3fU] {$a_4$};
\node[node distance=0.2cm, right=of node4fU] {$a_5$};

%\ldmnewuser{Eve}{6}{(5,-5)}
\ldmnewuser{sU}{4}{(5,-5)}
%\node[node distance=0.1cm, above=of groupEve] {Eve};
\node[node distance=0.1cm, above=of groupsU] {$U_2$};
\node[node distance=0.2cm, right=of node2sU] {$b_4$};
\node[node distance=0.2cm, right=of node4sU] {$b_5$};

% Connect Tx and Rx

%\ldmconnectusers{Alice}{Bob}{4}{1}
\ldmconnectusers{HeNB}{fU}{1}{2}
%\ldmconnectusers{Alice}{Eve}{2}{3}
\ldmconnectusers{eNB}{fU}{4}{0}
\ldmconnectusers{eNB}{sU}{3}{1}

% Coloring and marking specific areas
\node[right=of node2sU.south, yshift=-0.2cm, xshift=12pt] (sU1) {}; 
\node[right=of node2sU.north, yshift=0.2cm, xshift=12pt] (sU2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(sU1) -- (sU2) node [black,midway,xshift=6pt] {$n_{d2}-n_{d3}$};

\node[right=of node2fU.south, yshift=-0.2cm, xshift=12pt] (fU5) {}; 
\node[right=of node2fU.north, yshift=0.2cm, xshift=12pt] (fU6) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU5) -- (fU6) node [black,midway,xshift=6pt] {$n_{d3}-n_{d1}$};

\node[right=of node3fU.south, yshift=-0.2cm, xshift=12pt] (fU1) {}; 
\node[right=of node3fU.north, yshift=0.2cm, xshift=12pt] (fU2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU1) -- (fU2) node [black,midway,xshift=20pt] {$n_{d1}+n_{d3}-n_{d2}$};

\node[right=of node4fU.south, yshift=-0.2cm, xshift=12pt] (fU3) {}; 
\node[right=of node4fU.north, yshift=0.2cm, xshift=12pt] (fU4) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU3) -- (fU4) node [black,midway,xshift=6pt] {$n_{d2}-n_{d3}$};


\begin{scope}[on background layer]
%\node[fill=blue!10,fit=(node1fU) (node2fU)] (groupfUd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node1HeNB) (node1HeNB)] (groupHeNBd1) {};
\node[pattern=horizontal lines, pattern color=red!80,fit=(node1HeNB) (node1HeNB)] (groupHeNBd2) {};

\node[pattern=north west lines, pattern color=black,fit=(node1eNB) (node1eNB)] (groupeNBd1) {};
\node[pattern=north east lines, pattern color=red!80,fit=(node2eNB) (node2eNB)] (groupeNBd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node3eNB) (node3eNB)] (groupeNBd3) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node4eNB) (node4eNB)] (groupeNBd3) {};

\node[pattern=north west lines, pattern color=black,fit=(node1fU) (node1fU)] (groupfUd1) {};
\node[pattern=north east lines, pattern color=red!80,fit=(node2fU) (node2fU)] (groupfUd1) {};
\node[pattern=horizontal lines, pattern color=red!80,fit=(node3fU) (node3fU)] (groupfUd3) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node4fU) (node4fU)] (groupfUd3) {};

\node[pattern=north west lines, pattern color=black,fit=(node2sU) (node2sU)] (groupsUd1) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node3sU) (node3sU)] (groupsUd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node4sU) (node4sU)] (groupsUd3) {};
%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
\end{scope}





%\node[right=of node5Bob.south, yshift=-0.2cm] (bobcurly1) {}; 
%\node[right=of node2Bob.north, yshift=0.2cm] (bobcurly2) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(bobcurly1) -- (bobcurly2) node [black,midway] {$n_1$};
%
%\node[right=of node5Eve.south, yshift=-0.2cm] (evecurly1) {}; 
%\node[right=of node4Eve.north, yshift=0.2cm] (evecurly2) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(evecurly1) -- (evecurly2) node [black,midway] {$n_2$};
%
%\node[right=of node3Eve.south, yshift=-0.2cm] (evecurly3) {}; 
%\node[right=of node2Eve.north, yshift=0.2cm] (evecurly4) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(evecurly3) -- (evecurly4) node [black,midway,xshift=0.4cm] {$n_1-n_2$};
%
%
%
%\begin{scope}[on background layer]
%\node[fill=blue!10,fit=(node2Bob) (node5Bob)] (groupBobn1) {};
%\node[fill=blue!50,fit=(node2Eve) (node3Eve)] (groupEven1n2) {};
%%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
%\end{scope}


%\draw[->,red] (node5Bob.south)--(node1Eve.north) ;
\end{tikzpicture}


%\begin{tikzpicture}
%\coordinate (coordSourceupleft1) at (0,0);
%\coordinate (coordChannelupleft1) at (10,0);
%
%\node (reliableSourceBitsLeft) at (coordSourceupleft1) {};
%\node[right=of reliableSourceBitsLeft] (reliableSourceBitsRight) {};
%\node[node distance=1cm, below=of reliableSourceBitsLeft] (secureSourceBitsLeft) {};
%\node[node distance=1cm, below=of reliableSourceBitsRight] (secureSourceBitsRight) {};
%\node[node distance=0.1cm, left=of secureSourceBitsRight] (secureSourceBitsBlack) {};
%\node[node distance=1cm, below=of secureSourceBitsRight] (bottomSourceRight) {};
%\node[node distance=0.1cm, left=of secureSourceBitsLeft] {\parbox{2cm}{Secure source bits}};
%\node[node distance=0.1cm, right=of secureSourceBitsRight] {$m_2-m_1$};
%\node[node distance=0.1cm, left=of reliableSourceBitsLeft] {\parbox{2cm}{Reliable source bits}};
%\node[node distance=0.1cm, right=of reliableSourceBitsRight] {$m_1$};
%
%\draw [fill=yellow!20] (reliableSourceBitsLeft) rectangle (bottomSourceRight);
%\draw [fill=yellow!50] (secureSourceBitsLeft) rectangle (bottomSourceRight);
%\draw [fill=black] (secureSourceBitsBlack) rectangle (bottomSourceRight);
%
%
%\node (reliableChannelBitsLeft) at (coordChannelupleft1) {};
%\node[right=of reliableChannelBitsLeft] (reliableChannelBitsRight) {};
%\node[node distance=1cm, below=of reliableChannelBitsLeft] (secureChannelBitsLeft) {};
%\node[node distance=1cm, below=of reliableChannelBitsRight] (secureChannelBitsRight) {};
%\node[node distance=0.1cm, left=of secureChannelBitsRight] (secureChannelBitsBlack) {};
%\node[node distance=1cm, below=of secureChannelBitsRight] (bottomChannelRight) {};
%\node[node distance=0.1cm, left=of secureChannelBitsLeft] {\parbox{2cm}{Secure source bits}};
%\node[node distance=0.1cm, right=of secureChannelBitsRight] {$m_2-m_1$};
%\node[node distance=0.1cm, left=of reliableChannelBitsLeft] {\parbox{2cm}{Reliable source bits}};
%\node[node distance=0.1cm, right=of reliableChannelBitsRight] {$m_1$};
%
%\draw [fill=yellow!20] (reliableChannelBitsLeft) rectangle (bottomChannelRight);
%\draw [fill=yellow!50] (secureChannelBitsLeft) rectangle (bottomChannelRight);
%\draw [fill=black] (secureChannelBitsBlack) rectangle (bottomChannelRight);
%
%\end{tikzpicture}
%
%
%\tikzstyle{antenna} = [regular polygon,regular polygon sides=3, draw,shape
%border rotate=180,minimum size=0.2pt,scale=0.3]
%\tikzstyle{waves} = [snake=expanding waves, segment amplitude = 1.5cm, segment length = 0.3 cm,draw ]
%\begin{tikzpicture}
%	\coordinate (usercoord) at (0,0);
%	\node[rectangle,draw, minimum width=1cm, minimum height=1cm] (user) at (usercoord) {Tx};
%	\node[antenna] (userant1) at ($(user.west)+(-0.3cm,0.3cm)$) {};
%    \path[waves]  (userant1.west) -- ($(userant1.west)+(-1cm,0)$);
%    \draw (user) -| (userant1);
%          
%\end{tikzpicture}

%\end{document}

==> content/tikz_stacks.tex <==
%\input{tikzheader}

\edef\defaultpgflinewidth{\the\pgflinewidth}
%\newlength{\defaultpgflinewidth}
%\setlength{\defaultpgflinewidth}{0.1cm}

%Previous level name, new level name, level height, level description
\newcommand{\placeLevelOnTop}[4]{
\node[draw, fill=white, line width=\defaultpgflinewidth, rectangle, minimum width=1cm,minimum height=#3,inner sep=0pt] (#2) at ($(#1.north)+(0,#3*0.5-\defaultpgflinewidth*0.5)$) {#4}; 
}

%Previous level name, new level name, level height, level description
\newcommand{\placeLevelBelowBottom}[4]{
\node[draw, color=black!20, fill=white, line width=\defaultpgflinewidth, rectangle, minimum width=1cm,minimum height=#3,inner sep=0pt] (#2) at ($(#1.south)+(0,-#3*0.5+\defaultpgflinewidth*0.5)$) {#4}; 
}

\newlength{\mylabelwidth}
%Base coordinate, Level name, level label 
\newcommand{\addLevelLabel}[3]{
\settowidth{\mylabelwidth}{\pgfinterruptpicture #3 \endpgfinterruptpicture}
\node at ($(#2.north west -| #1)+(-0.2cm,-\defaultpgflinewidth*0.5)+(-\mylabelwidth*0.5,0)$) {#3};
\begin{pgfonlayer}{background}
\draw[dashed] ($(#2.north west -| #1)+(-0.1cm,-\defaultpgflinewidth*0.5)$) -- ($(#2.north west)+(0,-\defaultpgflinewidth*0.5)$);
\end{pgfonlayer}
}

%Lower Level name, Upper level name, brace label
\newcommand{\addBraceRight}[3]{
\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
(#1.south east) -- (#2.north east) node [black,midway,xshift=0.8cm,rotate=90] {\footnotesize
#3};
}

%Level name, dim label
\newcommand{\addDimensioningRight}[2]{
\draw[dashed] ($(#1.north east)+(0,-\defaultpgflinewidth*0.5)$) -- ($(#1.north east)+(0.6cm,-\defaultpgflinewidth*0.5)$);
\draw[dashed] ($(#1.south east)+(0,\defaultpgflinewidth*0.5)$) -- ($(#1.south east)+(0.6cm,\defaultpgflinewidth*0.5)$);
\draw[thick,<->] ($(#1.north east)+(0.3cm,-\defaultpgflinewidth*0.5)$) -- node[right,fill=white,inner sep=0pt,xshift=0.1cm] {#2} ($(#1.south east)+(0.3cm,\defaultpgflinewidth*0.5)$);
}

%Level name, dim label
\newcommand{\addDimensioningLeft}[2]{
\draw[dashed] ($(#1.north west)+(0,-\defaultpgflinewidth*0.5)$) -- ($(#1.north west)+(-0.6cm,-\defaultpgflinewidth*0.5)$);
\draw[dashed] ($(#1.south west)+(0,\defaultpgflinewidth*0.5)$) -- ($(#1.south west)+(-0.6cm,\defaultpgflinewidth*0.5)$);
\draw[thick,<->] ($(#1.north west)+(-0.3cm,-\defaultpgflinewidth*0.5)$) -- node[left,fill=white,inner sep=0pt,xshift=-0.1cm] {#2} ($(#1.south west)+(-0.3cm,\defaultpgflinewidth*0.5)$);
}



%\begin{document}

\begin{tikzpicture}

[
%
]
\coordinate (txOneY) at (0,0);
\coordinate (txTwoY) at ($(txOneY)+(1.5,0)$);
\coordinate (baseLeft) at ($(txOneY)+(-0.75cm,0)$);
\coordinate (txOneZ) at ($(txTwoY)+(2,0)$);
\coordinate (txTwoZ) at ($(txOneZ)+(1.5,0)$);

\node (ytx1) at ($(txOneY)+(0,-0.5)$) {Tx1};
\node (ytx2) at ($(txTwoY)+(0,-0.5)$) {Tx2};
\node  at ($(txOneY)!0.5!(txTwoY) + (0,-1)$) {$\textbf{Rx2}$};
\node (ztx1) at ($(txOneZ)+(0,-0.5)$) {Tx1};
\node (ztx2) at ($(txTwoZ)+(0,-0.5)$) {Tx2};
\node  at ($(txOneZ)!0.5!(txTwoZ) + (0,-1)$) {$\textbf{Rx1}$};

\placeLevelOnTop{txOneY}{d1}{0.5cm}{${D}_1$}
\placeLevelOnTop{d1}{c1}{1cm}{${C}_1$}
\placeLevelOnTop{c1}{b1}{0.5cm}{${B}_1$}

\placeLevelOnTop{txTwoY}{b2}{0.5cm}{${B}_2$}

\placeLevelOnTop{txOneZ}{d1}{0.5cm}{${B}_1$}

\placeLevelOnTop{txTwoZ}{d2z}{0.5cm}{${D}_2$}
\placeLevelOnTop{d2z}{c2z}{1cm}{${C}_2$}
\placeLevelOnTop{c2z}{b2z}{0.5cm}{${B}_2$}
\addLevelLabel{baseLeft}{c2z}{$2n_d-n_c$}
\addLevelLabel{baseLeft}{d2z}{$n_d$}
\addLevelLabel{baseLeft}{b2z}{$n_c$}

\addDimensioningRight{c2z}{$l_1$}


\draw[thick] ($(baseLeft)+(0,-\defaultpgflinewidth*0.5)$) -- ($(txTwoY)+(0.75cm,-\defaultpgflinewidth*0.5)$);
\draw[thick] ($(txOneZ)+(-0.75,-\defaultpgflinewidth*0.5)$) -- ($(txTwoZ)+(0.75cm,-\defaultpgflinewidth*0.5)$);

\end{tikzpicture}




%\end{document}

==> tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
      \pgf@temp
      \fi%
    },
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
        \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{\csname pgfk@/tikz/tikzmark prefix\endcsname#1\csname pgfk@/tikz/tikzmark suffix\endcsname}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname{\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
      \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}\save@orig@pic%
      \pgfsys@getposition{\pgfpictureid}\save@this@pic%
      \pgf@process{\pgfpointorigin\save@this@pic}%
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
      \pgf@process{\pgfpointorigin\save@orig@pic}%
      \advance\pgf@x by -\pgf@xa
      \advance\pgf@y by -\pgf@ya
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
          \advance \pgf@xa by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@x\relax
\advance \pgf@ya by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@y\relax
          \advance \pgf@xa by -\csname save@pg@\pgfpictureid\endcsname\pgf@x\relax
\advance \pgf@ya by -\csname save@pg@\pgfpictureid\endcsname\pgf@y\relax
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }
\begingroup
\catcode`\;=\active
\gdef\tikzmark@active#1#2{%
\tikz[remember picture with id=#2] #1;}
\endgroup
\def\tikzmark@nonactive#1#2{%
\tikz[remember picture with id=#2] #1;}
\newcommand\tikzmark@outside[2][]{%
  \ifnum\catcode`\;=\active
   \let\tikzmark@next=\tikzmark@active
  \else
   \let\tikzmark@next=\tikzmark@nonactive
  \fi
  \tikzmark@next{#1}{#2}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x pt}{\the\pgf@y pt}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark}[2][]{\only#3{\beameroriginal{\tikzmark}[{#1}]{#2}}}
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@#1}{%
      #3%
    }{%
      #2%
    }%
  }%
\newcommand\subnode[3][]{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@shape{rectangle}%
  \def\tikz@anchor{center}%
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
  {\PackageError{pgf}{Unknown shape ``\tikz@shape''}{}}%
  {%
    {%
      \let\pgf@sh@savedmacros=\pgfutil@empty% MW
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \def\pgf@sm@shape@name{\tikz@shape}% CJ % TT added prefix!
      \csname pgf@sh@s@\tikz@shape\endcsname%
      \pgf@sh@savedpoints%
      \pgf@sh@savedmacros% MW
      \pgftransformshift{%
        \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
       \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}% FIXME : this is double work!
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@node@name{\tikz@fig@name}%
      \ifx\pgf@node@name\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{\tikz@shape}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
        \pgfgettransform\pgf@temp
        \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
      \fi%
    }%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}
\def\usetikzmarklibrary{\pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}}%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

%% 
%% Copyright (C) 2011-2016 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.

